Explicit formula of deformation quantization with separation of variables for complex two-dimensional locally symmetric K\"{a}hler manifold

We give a complex two-dimensional noncommutative locally symmetric K\"{a}hler manifold via a deformation quantization with separation of variables. We present an explicit formula of its star product by solving the system of recurrence relations given by Hara-Sako. In the two-dimensional case, this system of recurrence relations gives two types of equations corresponding to the two coordinates. From the two types of recurrence relations, symmetrized and antisymmetrized recurrence relations are obtained. The symmetrized one gives the solution of the recurrence relation. From the antisymmetrized one, the identities satisfied by the solution are obtained. The star products for $\mathbb{C}^{2}$ and $\mathbb{C}P^{2}$ are constructed by the method obtained in this study, and we verify that these star products satisfy the identities.

==> EX/NCK2_C2.tex <==
\subsection{Example %for
of \(\mathbb{C}^{2}\)}
\label{subsec_NR_C2}
\ We shall construct a deformation quantization with separation of variables for \(\mathbb{C}^{2},\) the simplest concrete example via Theorem \ref{main_thm_N2}, and show that it also reproduces the star product with separation of variables by Karabegov \cite{Kara2}. Since \(\mathbb{C}^{2}\) is flat, i.e. \(R_{ABC}^{\quad \ \ \, D}=0,\) each \(X_{k}\left(\infty\right)\) is a constant multiple of the identity matrix, and \(T_{n}\left(\infty\right)\) can be obtained easily.

\begin{prop}
The formula for determining a star product with separation of variables on \(\mathbb{C}^{2}\) is given by
\begin{align}
  T_{n}\left(\infty\right)
  =
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \left(
    \begin{array}{ccccc}
      \tbinom{n}{0}  &  &  &  \text{\huge{0}}  \\
        &  \ddots  &  &  \\
        &    &  \tbinom{n}{n}  &  \\
      \text{\huge{0}}  &  &  &  0  &  \\
        &  &  &  &  \ddots
    \end{array}
  \right).
  \label{Tn_C}
\end{align}
\label{thm_Tn_C2}
\end{prop}

\begin{prf*}
We now take the canonical coordinates 
\(
  z^{1}=x^{1}+iy^{1},
  z^{2}=x^{2}+iy^{2}
\) 
as the local coordinates. Since 
\(
  \left(
    g_{AB}
  \right)
\), 
the component matrix of the K\"{a}hler metric on \(\mathbb{C}^{2}\), is
\begin{align*}
  \left(
    g_{AB}
  \right)
  =
  \left(
    \begin{array}{cccc}
      g_{11}  &  g_{12}
      &  g_{1\overline{1}}  &  g_{1\overline{2}}  \\
      g_{21}  &  g_{22}
      &  g_{2\overline{1}}  &  g_{2\overline{2}}  \\
      g_{\overline{1}1}  &  g_{\overline{1}2}
      &  g_{\overline{1}\,\overline{1}}  &  g_{\overline{1}\,\overline{2}}  \\
      g_{\overline{2}1}  &  g_{\overline{2}2}
      &  g_{\overline{2}\,\overline{1}}  &  g_{\overline{2}\,\overline{2}}
    \end{array}
  \right)
  :=
  \left(
    \begin{array}{cccc}
      g_{z^{1}z^{1}}  &  g_{z^{1}z^{2}}
      &  g_{z^{1}\overline{z}^{1}}  &  g_{z^{1}\overline{z}^{2}}  \\
      g_{z^{2}z^{1}}  &  g_{z^{2}z^{2}}
      &  g_{z^{2}\overline{z}^{1}}  &  g_{z^{2}\overline{z}^{2}}  \\
      g_{\overline{z}^{1}z^{1}}  &  g_{\overline{z}^{1}z^{2}}
      &  g_{\overline{z}^{1}\overline{z}^{1}}  &  g_{\overline{z}^{1}\overline{z}^{2}}  \\
      g_{\overline{z}^{2}z^{1}}  &  g_{\overline{z}^{2}z^{2}}
      &  g_{\overline{z}^{2}\overline{z}^{1}}  &  g_{\overline{z}^{2}\overline{z}^{2}}  \\
    \end{array}
  \right)
  =
  \left(
    \begin{array}{cccc}
      0  &  0  &  \frac{1}{2}  &  0  \\
      0  &  0  &  0  &  \frac{1}{2}  \\
      \frac{1}{2}  &  0  &  0  &  0  \\
      0  &  \frac{1}{2}  &  0  &  0
    \end{array}
  \right),
\end{align*}

\noindent
so the inverse matrix 
\(
  \left(
    g^{AB}
  \right)
\) 
is 
\begin{align*}
  \left(
    g^{AB}
  \right)
  =
  \left(
    \begin{array}{cccc}
      g^{11}  &  g^{12}
      &  g^{1\overline{1}}  &  g^{1\overline{2}}  \\
      g^{21}  &  g^{22}
      &  g^{2\overline{1}}  &  g^{2\overline{2}}  \\
      g^{\overline{1}1}  &  g^{\overline{1}2}
      &  g^{\overline{1}\,\overline{1}}  &  g^{\overline{1}\,\overline{2}}  \\
      g^{\overline{2}1}  &  g^{\overline{2}2}
      &  g^{\overline{2}\,\overline{1}}  &  g^{\overline{2}\,\overline{2}}
    \end{array}
  \right)
  :=
  \left(
    \begin{array}{cccc}
      g^{z^{1}z^{1}}  &  g^{z^{1}z^{2}}
      &  g^{z^{1}\overline{z}^{1}}  &  g^{z^{1}\overline{z}^{2}}  \\
      g^{z^{2}z^{1}}  &  g^{z^{2}z^{2}}
      &  g^{z^{2}\overline{z}^{1}}  &  g^{z^{2}\overline{z}^{2}}  \\
      g^{\overline{z}^{1}z^{1}}  &  g^{\overline{z}^{1}z^{2}}
      &  g^{\overline{z}^{1}\overline{z}^{1}}  &  g^{\overline{z}^{1}\overline{z}^{2}}  \\
      g^{\overline{z}^{2}z^{1}}  &  g^{\overline{z}^{2}z^{2}}
      &  g^{\overline{z}^{2}\overline{z}^{1}}  &  g^{\overline{z}^{2}\overline{z}^{2}}  \\
    \end{array}
  \right)
  =
  \left(
    \begin{array}{cccc}
      0  &  0  &  2  &  0  \\
      0  &  0  &  0  &  2  \\
      2  &  0  &  0  &  0  \\
      0  &  2  &  0  &  0
    \end{array}
  \right).
\end{align*}
Since 
\(
  g_{AB},
  \
  g^{AB}
\) 
are constant matrices, 
\(
  \Gamma_{BC}^{A}=0
  \
  \left(
    A,B,C
    =
    1,\overline{1}
  \right),
\) 
therefore \(R_{ABC}^{\quad \ \ \, D}=0.\) Thus each 
\(
  X_{k}
  \in
  M_{k+1}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
  \
  \left(
    k=1,\cdots,n
  \right)
\) 
is obtained as 
\(
  X_{k}
  =
  k\mathrm{Id}_{k+1},
\) 
and especially
\(
  X_{k}^{-1}
  =
  \frac{1}{k}
  \mathrm{Id}_{k+1}.
\) 
Next, we must determine 
\(
  F_{k}^{i_{k}}
\) 
and 
\(
  B_{k}^{i_{k}}.
\) 
Since the choice of the functions 
\(
  \Theta_{\overline{\mu}}^{i_{k}}
\) 
and 
\(
  \Theta_{\nu}^{i_{k}}
\) 
is not unique, there are many possible 
\(
  F_{k}^{i_{k}}
\) 
and 
\(
  B_{k}^{i_{k}}.
\) 
 So we shall now simply choose 
\(
  \Theta_{\mu}^{i_{k}}
  =
  \Theta_{\overline{\mu}}^{i_{k}}
  =
  \frac{1}{\sqrt{2}}
  \delta^{i_{k}}_{\ \,\mu}
\) 
here. %in this discussions. 
%In fact, we 
We can confirm that these 
\(
  \Theta_{\overline{\mu}}^{i_{k}}
\) 
and 
\(
  \Theta_{\nu}^{i_{k}}
\) 
%chosen in this way 
recover
\(
  g_{\overline{\mu}\nu}
  =
  \sum_{i_{k}=1}^{4}
  \Theta_{\overline{\mu}}^{i_{k}}
  \Theta_{\nu}^{i_{k}}.
\) 
So in this case
\begin{align*}
  F_{k}^{i_{k}}
  =
  \frac{1}{\sqrt{2}}
  \left(
    \delta^{i_{k}}_{\ \,1}
    \mathrm{Id}_{k+1}
    +
    \delta^{i_{k}}_{\ \,2}
    F_{d,k+1}
  \right),
  \
  B_{k}^{i_{k}}
  =
  \frac{1}{\sqrt{2}}
  \left(
    \delta^{i_{k}}_{\ \,1}
    \mathrm{Id}_{k+1}
    +
    \delta^{i_{k}}_{\ \,2}
    F_{d,k+1}
  \right).
\end{align*}

\noindent
By 
\(
  X^{-1}_{k}
  =
  \frac{1}{k}
  \mathrm{Id}_{k}
%  \
%  B^{i_{k}}_{k},
\), 
%and 
%\(
%  F^{i_{k}}_{k}
%\)
%correspond to the infinite dimensional matrix
%\begin{align*}
%  X^{-1}_{k}\left(\infty\right)
%  =
%  \left(
%    \begin{array}{c|ccc}
%      X^{-1}_{k} &  &  \text{\huge{0}}  &  \\  \hline
%        &  &  &  \\
%      \text{\huge{0}}  &  & \text{\huge{0}} &  
%    \end{array}
%  \right),
%\end{align*}
%
%\noindent
%\(
%  X^{-1}_{k}\left(\infty\right)
%  =
%  \frac{1}{k}
%  \mathrm{Id}\left(\infty\right),
%  \
%  B^{i_{k}}_{k}\left(\infty\right),
%\) 
%and 
%\(
%  F^{i_{k}}_{k}\left(\infty\right)
%\) 
%respectively, 
we obtain
\begin{align*}
  T_{n}\left(\infty\right)
  =&
  \hbar^{n}
  \sum_{i_{1},\cdots,i_{n}=1}^{4}
  F^{i_{n}}_{n}\left(\infty\right)
  \cdots
  F^{i_{1}}_{1}\left(\infty\right)
  T_{0}\left(\infty\right)
  \left(
    B^{i_{1}}_{1}\left(\infty\right)
    X^{-1}_{1}\left(\infty\right)
  \right)
  \cdots
  \left(
    B^{i_{n}}_{n}\left(\infty\right)
    X^{-1}_{n}\left(\infty\right)
  \right).
  \\
  =&
  \frac{\hbar^{n}}{n!}
  \left(
    \frac{1}{\sqrt{2}}
  \right)^{2n}
  \sum_{i_{1},\cdots,i_{n}=1}^{4}
  \left(
    \delta^{i_{n}}_{\ \,1}
    \mathrm{Id}\left(\infty\right)
    +
    \delta^{i_{n}}_{\ \,2}
    F_{d}\left(\infty\right)
  \right)
  \cdots
  \left(
    \delta^{i_{1}}_{\ \,1}
    \mathrm{Id}\left(\infty\right)
    +
    \delta^{i_{1}}_{\ \,2}
    F_{d}\left(\infty\right)
  \right)
  T_{0}\left(\infty\right)
  \\
  &
  \cdot
  \left(
    \delta^{i_{1}}_{\ \,1}
    \mathrm{Id}\left(\infty\right)
    +
    \delta^{i_{1}}_{\ \,2}
    F_{r}\left(\infty\right)
  \right)
  \cdots
  \left(
    \delta^{i_{n}}_{\ \,1}
    \mathrm{Id}\left(\infty\right)
    +
    \delta^{i_{n}}_{\ \,2}
    F_{r}\left(\infty\right)
  \right).
\end{align*}

\noindent
By using
%Here we use the property that
\begin{align*}
  \left(
    \begin{array}{c|c}
      A_{k+1} &  0  \\  \hline
      0  &  0
    \end{array}
  \right)
  \left(
    \begin{array}{c|c}
      X^{-1}_{k} &  0  \\  \hline
      0  &  0
    \end{array}
  \right)
  =
  \left(
    \begin{array}{c|c}
      A_{k+1} &  0  \\  \hline
      0  &  0
    \end{array}
  \right)
  \left(
    \begin{array}{c|c}
      X^{-1}_{k} &  0  \\  \hline
      0  &  B
    \end{array}
  \right)
\end{align*}

\noindent
for any 
\(
  A_{k+1}
  \in
  M_{k+1}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\)
and 
\(
  B
  \in
  M_{\infty}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\). 
%By using this property, the right-hand side of 
The above equation can be written as
%by
\begin{flalign*}
  T_{n}\left(\infty\right)
  =&
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \delta_{\mu_{1}\nu_{1}}
  \cdots
  \delta_{\mu_{n}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  \\
  =&
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \sum_{\mu_{1},\cdots,\mu_{n}=1}^{2}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  },
\end{flalign*}

\noindent
where 
\(
  \gamma\left(\cdot\right)
  :
  \left\{
    1,2
  \right\}^{n}
  \to
  \mathbb{Z}_{\geq0}
\) 
is defined by 
\begin{align*}
  \gamma
  \left(
    \mu^{\left(n\right)}
  \right)
  :=
  \sum_{k=1}^{n}
  \left[
    \frac{\mu_{k}}{2}
  \right]
  =
  \sum_{k=1}^{n}
  \delta_{\mu_{k}2}
\end{align*}

\noindent
for multi-indices 
\(
  \mu^{\left(n\right)}
  =
  \left(
    \mu_{1},
    \cdots,
    \mu_{n}
  \right),
\) 
and 
\(
  \left[
    \cdot
  \right]
  :
  \mathbb{R}
  \to
  \mathbb{Z}
\) 
is Gauss symbol. We define 
\(
  \gamma
  \left(
    \nu^{\left(n\right)}
  \right)
\) 
in the same way. In other words, 
\(
  \gamma\left(\cdot\right)
  :
  \left\{
    1,2
  \right\}^{n}
  \to
  \mathbb{Z}_{\geq0}
\) 
gives the number of each 
\(
  \mu_{k}
\) 
(or 
\(
  \nu_{k}
\)
) 
that is 2. We can rewrite
\begin{align*}
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \sum_{\mu_{1},\cdots,\mu_{n}=1}^{2}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  =&
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \sum_{j=0}^{n}
  \binom{n}{j}
  \left(
    F_{d}\left(\infty\right)
  \right)^{j}
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{j}
\end{align*}

\noindent
since there are \(\tbinom{n}{j}\) combinations of each \(\mu_{k}\) such that 
\(
  \gamma
  \left(
    \mu^{\left(n\right)}
  \right)
  =
  j.
\) 
After summing over 
\(
  j
  \in
  \left\{1,\cdots,n\right\},
\) 
this is concretely expressed as 
\begin{align*}
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \sum_{j=0}^{n}
  \binom{n}{j}
  \left(
    F_{d}\left(\infty\right)
  \right)^{j}
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{j}
  =
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \left(
    \begin{array}{ccccc}
      \binom{n}{0}  &  &  &  \text{\huge{0}}  \\
        &  \ddots  &  &  \\
        &    &  \binom{n}{n}  &  \\
      \text{\huge{0}}  &  &  &  0  &  \\
        &  &  &  &  \ddots
    \end{array}
  \right)
\end{align*}

\noindent
by matrix representations. This proof was completed.\(_\blacksquare\)
\end{prf*}

\noindent
By Theorem \ref{thm_Tn_C2}, the coefficients
\(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
\) 
(or 
\(
  T_{ij}^{n}
\)
) 
is determined as
\begin{align}
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  =
  T_{ij}^{n}
  =
  \begin{cases}
    \displaystyle
    \frac{
      \binom{n}{i-1}
      \hbar^{n}
    }{
      2^{n}
      \cdot
      n!
    }
    &
    \
    \left(
      i
      =
      j
    \right)
    \\
    0
    &
    \
    \left(
      i
      \neq
      j
    \right)
  \end{cases},
  \label{coeff_Tn_C}
\end{align}

\noindent
where 
\(
  \alpha_{2}^{n}
  =
  i-1
\) 
and 
\(
  \beta_{2}^{n}
  =
  j-1.
\) 
Hence, the star product with separation of variables on \(\mathbb{C}^{2}\) is obtained as follows :
\begin{align}
  f
  \ast
  g
  =&
  \sum_{n=0}^{\infty}
  \sum_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  \left(
    D^{\overrightarrow{\alpha_{n}}}f
  \right)
  \left(
    D^{\overrightarrow{\beta_{n}^{\ast}}}g
  \right)
  \nonumber
  \\
  =&
  \sum_{n=0}^{\infty}
  \sum_{i=1}^{n+1}
  T_{ii}^{n}
  \left\{
    \left(
      D^{1}
    \right)^{
      n
      -
      \left(
        i-1
      \right)
    }
    \left(
      D^{2}
    \right)^{i-1}
    f
  \right\}
  \left\{
    \left(
      D^{\overline{1}}
    \right)^{
      n
      -
      \left(
        i-1
      \right)
    }
    \left(
      D^{\overline{2}}
    \right)^{i-1}
    g
  \right\}.
  \label{star_C_1}
\end{align}

\noindent
Substituting \eqref{coeff_Tn_C} into the right-hand side of \eqref{star_C_1},

\begin{flalign}
  &
  \sum_{n=0}^{\infty}
  \sum_{i=1}^{n+1}
  T_{ii}^{n}
  \left\{
    \left(
      D^{1}
    \right)^{
      n
      -
      \left(
        i-1
      \right)
    }
    \left(
      D^{2}
    \right)^{i-1}
    f
  \right\}
  \left\{
    \left(
      D^{\overline{1}}
    \right)^{
      n
      -
      \left(
        i-1
      \right)
    }
    \left(
      D^{\overline{2}}
    \right)^{i-1}
    g
  \right\}
  &
  \nonumber
  \\
  &=
  \sum_{n=0}^{\infty}
  \sum_{i=1}^{n+1}
  \left(
    \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \binom{n}{i-1}
  \left\{
    \left(
      g^{1\overline{1}}
      \partial_{\overline{1}}
    \right)^{
      n
      -
      \left(
        i-1
      \right)
    }
    \left(
      g^{2\overline{2}}
      \partial_{\overline{2}}
    \right)^{
      i-1
    }
    f
  \right\}
  \left\{
    \left(
      g^{\overline{1}1}
      \partial_{1}
    \right)^{
      n
      -
      \left(
        i-1
      \right)
    }
    \left(
      g^{\overline{2}2}
      \partial_{2}
    \right)^{
      i-1
    }
    g
  \right\}
  &
  \nonumber
  \\
  &=
  \sum_{n=0}^{\infty}
  \frac{
    \left(
      2\hbar
    \right)^{n}
  }{n!}
  \sum_{j=0}^{n}
  \binom{n}{j}
  \left(
    \partial_{\overline{z}^{1}}^{
      n
      -
      j
    }
    \partial_{\overline{z}^{2}}^{
      j
    }
    f
  \right)
  \left(
    \partial_{z^{1}}^{
      n
      -
      j
    }
    \partial_{z^{2}}^{
      j
    }
    g
  \right),
  &
  \label{star_C_2}
\end{flalign}

\noindent
where we rewrite \(i-1\) as \(j\) in the last line in \eqref{star_C_2}. Here, using the left (right) differential operator

\begin{align*}
  f
  \overleftarrow{
    \partial_{z^{A}}
  }
  :=
  \partial_{z^{A}}
  f,
  \
  \overrightarrow{
    \partial_{z^{A}}
  }
  g
  :=
  \partial_{z^{A}}
  g
  \
  \left(
    A
    \in
    \left\{
      1,2,\bar{1},\bar{2}
    \right\}
  \right),
\end{align*}

\noindent
%then
we obtain the star product on \(\mathbb{C}^{2}\) as
\begin{align}
  f
  \ast
  g
  &
  =
  \sum_{n=0}^{\infty}
  \frac{
    \left(
      2\hbar
    \right)^{n}
  }{n!}
  \sum_{j=0}^{n}
  \binom{n}{j}
  \left(
    \partial_{\overline{z}^{1}}^{
      n
      -
      j
    }
    \partial_{\overline{z}^{2}}^{
      j
    }
    f
  \right)
  \left(
    \partial_{z^{1}}^{
      n
      -
      j
    }
    \partial_{z^{2}}^{
      j
    }
    g
  \right)
  \nonumber
  \\
  &=
  \sum_{n=0}^{\infty}
  \frac{
    \left(
      2\hbar
    \right)^{n}
  }{n!}
  f
  \left\{
    \sum_{j=0}^{n}
    \binom{n}{j}
    \left(
      \overleftarrow{
        \partial_{\overline{z}^{1}}
      }
      \overrightarrow{
        \partial_{z^{1}}
      }
    \right)^{
      n-j
    }
    \left(
      \overleftarrow{
        \partial_{\overline{z}^{2}}
      }
      \overrightarrow{
        \partial_{z^{2}}
      }
    \right)^{j}
  \right\}
  g.
  \label{star_C_3}
\end{align}
\noindent
Let us compare the previous result \eqref{star_prd_C2_Kara_Voro_sol} to verify that Theorem \ref{main_thm_N2} works well. By using the binomial theorem for the left and right differential operators in \eqref{star_C_3}, we have
\begin{align}
  \sum_{n=0}^{\infty}
  \frac{
    \left(
      2\hbar
    \right)^{n}
  }{n!}
  f
  \left\{
    \sum_{j=0}^{n}
    \binom{n}{j}
    \left(
      \overleftarrow{
        \partial_{\overline{z}^{1}}
      }
      \overrightarrow{
        \partial_{z^{1}}
      }
    \right)^{
      n-j
    }
    \left(
      \overleftarrow{
        \partial_{\overline{z}^{2}}
      }
      \overrightarrow{
        \partial_{z^{2}}
      }
    \right)^{j}
  \right\}
  g
  =&
  \sum_{n=0}^{\infty}
  \frac{
    \left(
      2\hbar
    \right)^{n}
  }{n!}
  f
  \left(
    \overleftarrow{
      \partial_{\overline{z}^{1}}
    }
    \overrightarrow{
      \partial_{z^{1}}
    }
    +
    \overleftarrow{
      \partial_{\overline{z}^{2}}
    }
    \overrightarrow{
      \partial_{z^{2}}
    }
  \right)^{n}
  g
  \nonumber
  \\
  =&
  f
  \mathrm{exp}
  2\hbar
  \left(
    \overleftarrow{
      \partial_{\overline{z}^{1}}
    }
    \overrightarrow{
      \partial_{z^{1}}
    }
    +
    \overleftarrow{
      \partial_{\overline{z}^{2}}
    }
    \overrightarrow{
      \partial_{z^{2}}
    }
  \right)
  g.
  \label{star_C_4}
\end{align}
\noindent
Here, if we put the formal parameter \(\nu\) as \(\nu:=2\hbar\), we obtain
\(
  f
  \ast
  g
  =
  f
  \mathrm{exp}
  \nu
  \left(
    \overleftarrow{
      \partial_{\overline{z}^{1}}
    }
    \overrightarrow{
      \partial_{z^{1}}
    }
    +
    \overleftarrow{
      \partial_{\overline{z}^{2}}
    }
    \overrightarrow{
      \partial_{z^{2}}
    }
  \right)
  g,
\) 
which is the star product with separation of variables by Karabegov %\cite{Kara2}.
\eqref{star_prd_C2_Kara_Voro_sol}.
\bigskip
\\
\ We stated in Subsection \ref{NR_plus} that \(T_{n}\left(\infty\right)\) given in \eqref{main_them_N2_Tinf} solved via Theorem \ref{main_thm_N2} satisfies the formula \eqref{minus_thm_N2_eq_rsz} in Theorem \ref{minus_thm_N2}. So we shall directly verify that \(T_{n}\left(\infty\right)\) obtained via Theorem \ref{main_thm_N2} actually satisfies the formula \eqref{minus_thm_N2_eq_rsz} in Theorem \ref{minus_thm_N2} in 
%. In 
the case of \(\mathbb{C}^{2}\). 
% by direct calculation.
By Theorem \ref{minus_thm_N2}, \(Y_{n}\) is obtained as
\begin{align*}
  Y_{n}
  =
  \left(
    \begin{array}{ccccc}
      n  &  &  &  &  \text{\huge{0}} \\
        &  n-2  &  &  &  \\
        &  &  \ddots  &  &  \\
        &    &  &  -(n-2)  &  \\
      \text{\huge{0}}  &  &  &  &  -n
    \end{array}
  \right).
\end{align*}

\noindent
The embedding \(Y_{n}\left(\infty\right)\) for \(Y_{n}\) is as in the way of \eqref{emb_gene}. 
%\begin{align*}
%  Y_{n}\left(\infty\right)
%  =
%  \left(
%    \begin{array}{ccccccc}
%      n  &  &  &  &  \text{\huge{0}}  &  &  \\
%        &  n-2  &  &  &  &  &  \\
%        &  &  \ddots  &  &  &  &  \\
%        &    &  &  -(n-2)  &  &  &  \\
%      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
%        &  &  &  &  &  0  &  \\
%        &  &  &  &  &  &  \ddots  
%    \end{array}
%  \right).
%\end{align*}
%
%\noindent
Thus,
\begin{align*}
  T_{n}\left(\infty\right)
  Y_{n}\left(\infty\right)
  =&
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \left(
    \begin{array}{ccccccc}
      n \binom{n}{0}
      &  &  &  &  \text{\huge{0}}  &  &  \\
        &  (n-2) \binom{n}{1}  &  &  &  &  &  \\
        &  &  \ddots  &  &  &  &  \\
        &    &  &  -(n-2) \binom{n}{n-1}  &  &  &  \\
      \text{\huge{0}}  &  &  &  &  -n \binom{n}{n}  &  &  \\
        &  &  &  &  &  0  &  \\
        &  &  &  &  &  &  \ddots  
    \end{array}
  \right).
\end{align*}

\noindent
On the other hand, 
\(
  \hbar
  C_{n}^{'}
  \left(\infty\right)
\) 
is calculated as

\begin{align*}
  \hbar
  C_{n}^{'}\left(\infty\right)
  =&
  \hbar
  \left(
    \frac{1}{2}
    T_{n-1}\left(\infty\right)
    -
    \frac{1}{2}
    F_{d}\left(\infty\right)
    T_{n-1}\left(\infty\right)
    F_{r}\left(\infty\right)
  \right).
\end{align*}

\noindent
We substitute \eqref{Tn_C} for \(n-1\), \eqref{emb_Fd}, and \eqref{emb_Fr} into the the right-hand side of the above. Then,

\begin{align*}
  &
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{\left(n-1\right)!}
  \left\{
    \left(
      \begin{array}{cccccc}
        \binom{n-1}{0}  &  &  &  \text{\huge{0}}  &  &  \\
          &  \ddots  &  &  &  &  \\
          &    &  \binom{n-1}{n-1}  &  &  &  \\
        \text{\huge{0}}  &  &  &  0  &  &  \\
          &  &  &  &  0  &  \\
          &  &  &  &  &  \ddots  
      \end{array}
    \right)
    -
    \left(
      \begin{array}{cccccc}
        0  &  &  &  \text{\huge{0}}  &  &  \\
          &  \binom{n-1}{0}  &  &  &  &  \\
          &    &  \ddots  &  &  &  \\
        \text{\huge{0}}  &  &  &  \binom{n-1}{n-1}  &  &  \\
          &  &  &  &  0  &  \\
          &  &  &  &  &  \ddots  
      \end{array}
    \right)
  \right\}
  \\
  &=
  \left(
  \frac{\hbar}{2}
  \right)^{n}
  \frac{1}{n!}
  \left(
    \begin{array}{ccccccc}
      n \binom{n}{0}
      &  &  &  &  \text{\huge{0}}  &  &  \\
        &  (n-2) \binom{n}{1}  &  &  &  &  &  \\
        &  &  \ddots  &  &  &  &  \\
        &    &  &  -(n-2) \binom{n}{n-1}  &  &  &  \\
      \text{\huge{0}}  &  &  &  &  -n \binom{n}{n}  &  &  \\
        &  &  &  &  &  0  &  \\
        &  &  &  &  &  &  \ddots  
    \end{array}
  \right).
\end{align*}

\noindent
Hence, for any 
\(
  n
  \in
  \mathbb{Z}_{\geq0},
\) 
the matrix 
\(
  T_{n}\left(\infty\right)
\) for \(\mathbb{C}^{2}\) satisfies \eqref{minus_thm_N2_eq_another_rsz}.


==> EX/NCK2_CP2_Varna.tex <==
\subsection{%Example for \(\mathbb{C}P^{2}\)
Example of \(\mathbb{C}P^{2}\)
}
\label{subsec_NR_CP2}
\ %As another concrete example, we shall consider a deformation quantization with separation of variables for \(\mathbb{C}P^{2}.\) Previous works related to deformation quantizations for \(\mathbb{C}P^{N}\) are known, for example Omori-Maeda-Yoshioka \cite{OMY2}, Bordemann et al. \cite{BBEW}, Balachandran et al. \cite{BDMLO}, Hayasaka-Nakayama-Takaya \cite{HNT}, Sako-Suzuki-Umetsu \cite{SSU1,SSU2,SU1,SU2,SU3}, and Hara-Sako \cite{HS1,HS2}. 
%（ここはjournal用）We present the formula for \(T_{n}\left(\infty\right)\) such that it gives a star product with separation of variables for \(\mathbb{C}P^{2}.\)
In this subsection, we confirm that the deformation quantization with separation of variables for \(\mathbb{C}P^{2}\) obtained via our main result (Theorem \ref{main_thm_N2}) satisfies the identities in Theorem \ref{minus_thm_N2} or equivalently \eqref{minus_thm_N2_eq_rsz} in Subsection \ref{NR_minus}.
%reproduces the result by Sako-Suzuki-Umetsu \cite{SSU1,SSU2}.
\begin{prop}
The formula for determining a star product with separation of variables on \(\mathbb{C}P^{2}\) is given by
\begin{align}
  T_{n}\left(\infty\right)
  =
  \frac{
    \Gamma
    \left(
      1
      -
      n
      +
      \frac{1}{\hbar}
    \right)
  }{
    n!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  },
  \label{formula_CP2}
\end{align}
where each \(g_{\overline{\mu_{k}}\nu_{k}}\) is Fubini-Study metric and 
\(
  \gamma\left(\cdot\right)
  :
  \left\{
    1,2
  \right\}^{n}
  \to
  \mathbb{Z}_{\geq0}
\) 
is defined by
\begin{align}
  \gamma
  \left(
    \mu^{\left(n\right)}
  \right)
  :=
  \sum_{k=1}^{2}
  \left[
    \frac{\mu_{k}}{2}
  \right]
  =
  \sum_{k=1}^{2}
  \delta_{\mu_{k}2},
  \qquad
  \gamma
  \left(
    \nu^{\left(n\right)}
  \right)
  :=
  \sum_{k=1}^{2}
  \left[
    \frac{\nu_{k}}{2}
  \right]
  =
  \sum_{k=1}^{2}
  \delta_{\nu_{k}2}
  \label{gamma_gauss}
\end{align}

\noindent
for multi-indices
\(
  \mu^{\left(n\right)}
  =
  \left(
    \mu_{1},
    \cdots,
    \mu_{n}
  \right),
  \nu^{\left(n\right)}
  =
  \left(
    \nu_{1},
    \cdots,
    \nu_{n}
  \right).
\)
\label{thm_Tn_CP2}
\end{prop}

\noindent
We can prove this proposition by direct calculations of \eqref{main_them_N2_Tinf} in Theorem \ref{main_thm_N2}. See \cite{OS_Varna} for %the 
detailed proof of it. By Proposition \ref{thm_Tn_CP2}, the star product with separation of variables on \(\mathbb{C}P^{2}\) is obtained by
\begin{align}
  f
  \ast
  g
  =
  \sum_{n=0}^{\infty}
  \frac{
    \Gamma
    \left(
      1
      -
      n
      +
      \frac{1}{\hbar}
    \right)
    g_{\overline{\mu_{1}}\nu_{1}}
    \cdots
    g_{\overline{\mu_{n}}\nu_{n}}
  }{
    n!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \left(
    D^{\nu_{1}}
    \cdots
    D^{\nu_{n}}
    f
  \right)
  \left(
    D^{\overline{\mu_{1}}}
    \cdots
    D^{\overline{\mu_{n}}}
    g
  \right).
  \label{star_CP2}
\end{align}

\noindent
Detailed calculations for deriving equation \eqref{star_CP2} from \eqref{formula_CP2} are also given in \cite{OS_Varna}. This star product coincides with %the result 
\eqref{star_prd_C2_SSU_sol} by Sako-Suzuki-Umetsu %\cite{SSU1,SSU2}
. This result implies that Theorem \ref{main_thm_N2} works well.
\bigskip
\\
\ As in the case of \(\mathbb{C}^{2},\) we shall see that \eqref{formula_CP2} satisfies \eqref{minus_thm_N2_eq_rsz} in Theorem \ref{minus_thm_N2}. %for \(N=2.\) 
By Theorem \ref{minus_thm_N2}, the components of \(Y_{n}\) for \(\mathbb{C}P^{2}\) are calculated as
\begin{align*}
  Y_{i,j}^{n}
  =
  \begin{cases}
    \hbar
    \left\{
      n
      -
      2
      \left(
        i-1
      \right)
    \right\}
    \left(
      1
      -
      n
      -
      \frac{1}{\hbar}
    \right)
    &
    \left(
      i=j
    \right)
    \\
    0
    &
    \left(
      i
      \neq
      j
    \right)
  \end{cases}.
\end{align*}

%\noindent
%and then
%\begin{align*}
%  Y_{n}
%  =
%  \hbar
%  \left(
%    1
%    -
%    n
%    -
%    \frac{1}{\hbar}
%  \right)
%  \left(
%    \begin{array}{ccccc}
%      n  &  &  &  &  \text{\huge{0}} \\
%        &  n-2  &  &  &  \\
%        &  &  \ddots  &  &  \\
%        &    &  &  -(n-2)  &  \\
%      \text{\huge{0}}  &  &  &  &  -n
%    \end{array}
%  \right).
%\end{align*}
%
%\noindent
%Here the matrix 
%\begin{align*}
%  \left(
%    \begin{array}{ccccc}
%      n  &  &  &  &  \text{\huge{0}} \\
%        &  n-2  &  &  &  \\
%        &  &  \ddots  &  &  \\
%        &    &  &  -(n-2)  &  \\
%      \text{\huge{0}}  &  &  &  &  -n
%    \end{array}
%  \right),
%\end{align*}
%
%\noindent
%which is \(Y_{n}\) without the coefficient, is the matrix of the \(k\)-th column of the matrix multiplied by
%
%\begin{align*}
%  n
%  -
%  2
%  \left(
%    k-1
%  \right)
%  =
%  n
%  \left\{
%    1
%    -
%    \frac{
%      2\left(k-1\right)
%    }{n}
%  \right\}.
%\end{align*}

\noindent
\(Y_{n}\left(\infty\right)\) is written as
\begin{align}
  Y_{n}\left(\infty\right)
  =
  \hbar
  \left(
    1
    -
    n
    -
    \frac{1}{\hbar}
  \right)
  \left(
    \begin{array}{ccccccc}
      n  &  &  &  &  \text{\huge{0}}  &  &  \\
        &  n-2  &  &  &  &  &  \\
        &  &  \ddots  &  &  &  &  \\
        &    &  &  -(n-2)  &  &  &  \\
      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
        &  &  &  &  &  0  &  \\
        &  &  &  &  &  &  \ddots  
    \end{array}
  \right).
  \label{Yn_CP2}
\end{align}

\noindent
%So the left-hand side of \eqref{minus_thm_N2_eq_rsz} is obtained by
%\begin{align}
%  T_{n}\left(\infty\right)
%  Y_{n}\left(\infty\right)
%  =&
%  \frac{
%    \hbar
%    \left(
%      1
%      -
%      n
%      -
%      \frac{1}{\hbar}
%    \right)
%    \Gamma
%    \left(
%      1
%      -
%      n
%      +
%      \frac{1}{\hbar}
%    \right)
%  }{
%    n!
%    \Gamma
%    \left(
%      1
%      +
%      \frac{1}{\hbar}
%    \right)
%  }
%  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
%  g_{\overline{\mu_{1}}\nu_{1}}
%  \cdots
%  g_{\overline{\mu_{n}}\nu_{n}}
%  \nonumber
%  \\
%  &
%  \cdot
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n\right)}
%    \right)
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
%  }
%  \left(
%    \begin{array}{ccccccc}
%      n  &  &  &  &  \text{\huge{0}}  &  &  \\
%        &  n-2  &  &  &  &  &  \\
%        &  &  \ddots  &  &  &  &  \\
%        &    &  &  -(n-2)  &  &  &  \\
%      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
%        &  &  &  &  &  0  &  \\
%        &  &  &  &  &  &  \ddots  
%    \end{array}
%  \right).
%  \label{another_lhs_CP2}
%\end{align}

\noindent
To calculate 
\(
  T_{n}\left(\infty\right)
  Y_{n}\left(\infty\right)
\) 
we use the following proposition.

\begin{prop}
\begin{align*}
  &
  \left(
    F_{d}\left(\infty\right)
  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n\right)}
%    \right)
  k
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
    l
  }
  \left(
    \begin{array}{ccccccc}
      n  &  &  &  &  \text{\huge{0}}  &  &  \\
        &  n-2  &  &  &  &  &  \\
        &  &  \ddots  &  &  &  &  \\
        &    &  &  -(n-2)  &  &  &  \\
      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
        &  &  &  &  &  0  &  \\
        &  &  &  &  &  &  \ddots  
    \end{array}
  \right)
  \\
  &=
  \left(
    n
    -
    2
    l
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
  \right)
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    k
%    \gamma
%    \left(
%      \nu^{\left(n\right)}
%    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    l
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
  },
  \qquad
  \left(
    k,
    l
    =
    0,
    \cdots,
    n
  \right).
\end{align*}
%where 
%\(
%  k,
%  l
%  =
%  0,
%  \cdots,
%  n
%\) 
%and these are fixed.
\label{Prop_Fd_Fr}
\end{prop}

\begin{prf*}
Since the properties of \(F_{d}\left(\infty\right)\) and \(F_{r}\left(\infty\right)\) in Remark \ref{rem_Fd_Fr},
\begin{align}
  \left(
    F_{d}\left(\infty\right)
  \right)^{k}
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{l}
  =
  \left(
    \begin{array}{c|c}
      \left(
        \delta_{i,k}
        \delta_{j,l}
      \right)
      &
      0
      \\ \hline
      0
      &
      0
    \end{array}
  \right),
  \label{calc_Fd_T_Fr}
\end{align}

\noindent
where 
\(
  \left(
    \delta_{i,k}
    \delta_{j,l}
  \right)
  \in
  M_{n+1}
  \left(
  \mathbb{C}
  \left[\!
    \left[
      \hbar
    \right]\!
  \right]
  \right)
\) 
is the square matrix of order \(n+1\) such that the 
%diagonal 
\(\left(k,l\right)\) component
%elements 
%\(
%  \left(
%    k,l
%  \right)
%\) 
%component 
is 1 and the others are 0. And note that the indices \(k\) and \(l\) are fixed. Then we get the equation. \(_{\blacksquare}\)
%By direct calculations, we have
%\begin{align}
%  &
%  \left(
%    \begin{array}{ccc}
%      \delta_{
%        \left(
%          \nu^{\left(n\right)}
%        \right),
%        \left(
%          \mu^{\left(n\right)}
%        \right)
%      }
%      &
%      &
%      \text{\huge{0}}
%      \\
%      &
%      0
%      &
%      \\
%      \text{\huge{0}}
%      &
%      &
%      \ddots
%    \end{array}
%  \right)
%  \left(
%    \begin{array}{ccccccc}
%      n  &  &  &  &  \text{\huge{0}}  &  &  \\
%        &  n-2  &  &  &  &  &  \\
%        &  &  \ddots  &  &  &  &  \\
%        &    &  &  -(n-2)  &  &  &  \\
%      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
%        &  &  &  &  &  0  &  \\
%        &  &  &  &  &  &  \ddots  
%    \end{array}
%  \right)
%  \nonumber
%  \\
%  =&
%  \left(
%    \begin{array}{ccc}
%      \left(
%        n
%        -
%        2
%        \left(
%          \mu^{\left(n\right)}
%        \right)
%      \right)
%      \delta_{
%        \left(
%          \nu^{\left(n\right)}
%        \right),
%        \left(
%          \mu^{\left(n\right)}
%        \right)
%      }
%      &
%      &
%      \text{\huge{0}}
%      \\
%      &
%      0
%      &
%      \\
%      \text{\huge{0}}
%      &
%      &
%      \ddots
%    \end{array}
%  \right)
%  \nonumber
%  \\
%  =&
%  \left(
%     n
%     -
%     2
%     \left(
%       \mu^{\left(n\right)}
%     \right)
%   \right)
%   \left(
%    \begin{array}{ccc}
%      \delta_{
%        \left(
%          \nu^{\left(n\right)}
%        \right),
%        \left(
%          \mu^{\left(n\right)}
%        \right)
%      }
%      &
%      &
%      \text{\huge{0}}
%      \\
%      &
%      0
%      &
%      \\
%      \text{\huge{0}}
%      &
%      &
%      \ddots
%    \end{array}
%  \right).
%  \label{calc_Fd_T_Fr_Y}
%\end{align}
%
%\noindent
%Note that Einstein summation convention is not used in the right-hand side of \eqref{calc_Fd_T_Fr_Y} since 
%\(
%  \left(
%    \mu^{\left(n\right)}
%  \right)
%\) 
%and 
%\(
%  \left(
%    \nu^{\left(n\right)}
%  \right)
%\) 
%are fixed. Substituting \eqref{calc_Fd_T_Fr} into both sides of \eqref{calc_Fd_T_Fr_Y}, we have
%\begin{align*}
%  &
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n\right)}
%    \right)
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
%  }
%  \left(
%    \begin{array}{ccccccc}
%      n  &  &  &  &  \text{\huge{0}}  &  &  \\
%        &  n-2  &  &  &  &  &  \\
%        &  &  \ddots  &  &  &  &  \\
%        &    &  &  -(n-2)  &  &  &  \\
%      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
%        &  &  &  &  &  0  &  \\
%        &  &  &  &  &  &  \ddots  
%    \end{array}
%  \right)
%  \\
%  =&
%  \left(
%    n
%    -
%    2
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
%  \right)
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n\right)}
%    \right)
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n\right)}
%    \right)
%  }.
%  _{\blacksquare}
%\end{align*}
\end{prf*}

\noindent
By Proposition \ref{Prop_Fd_Fr}, %the left-hand side of \eqref{another_lhs_CP2} 
\(
  T_{n}\left(\infty\right)
  Y_{n}\left(\infty\right)
\) 
is calculated as
%can be rewritten as
\begin{flalign}
  &
  T_{n}\left(\infty\right)
  Y_{n}\left(\infty\right)
  &
  \nonumber
  \\
  &=
  \frac{
    \hbar
    \left(
      1
      -
      n
      -
      \frac{1}{\hbar}
    \right)
    \Gamma
    \left(
      1
      -
      n
      +
      \frac{1}{\hbar}
    \right)
  }{
    n!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  &
  \nonumber
  \\
  &
  \mbox{}
  \quad
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  \left(
    \begin{array}{ccccccc}
      n  &  &  &  &  \text{\huge{0}}  &  &  \\
        &  n-2  &  &  &  &  &  \\
        &  &  \ddots  &  &  &  &  \\
        &    &  &  -(n-2)  &  &  &  \\
      \text{\huge{0}}  &  &  &  &  -n  &  &  \\
        &  &  &  &  &  0  &  \\
        &  &  &  &  &  &  \ddots  
    \end{array}
  \right)
  &
  \nonumber
  \\
  &=
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \!\!
  \sum_{
    \substack{
      \mu_{1},\cdots,\mu_{n}=1
      \\
      \nu_{1},\cdots,\nu_{n}=1
    }
  }^{2}
  \!\!\!\!\!
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    1
    -
    \frac{2}{n}
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  \right)
  %&
  %\nonumber\\
  %&
  %\mbox{}
  %\quad
  %\cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }.
  \label{another_lhs_CP2_calc}
\end{flalign}

\noindent
%where we used that 
%\(
%  1
%  -
%  \frac{
%    2\left(k-1\right)
%  }{n}
%\) 
%can be rewritten as 
%\begin{align*}
%  1
%  -
%  \frac{
%    2\left(k-1\right)
%  }{n}
%  =
%  1
%  -
%  \frac{2}{n}
%  \gamma
%  \left(
%    \mu^{\left(n\right)}
%  \right),
%\end{align*}
%
%\noindent
%since 
%\(
%  1
%  -
%  \frac{
%    2\left(k-1\right)
%  }{n}
%\) 
%is multiplied by the \(k\)-th column and 
%\(
%  \gamma
%  \left(
%    \mu^{\left(n\right)}
%  \right)
%\) 
%corresponds to the number of columns.

Next, we calculate the right-hand side of \eqref{minus_thm_N2_eq_rsz}. By Theorem \ref{minus_thm_N2},

\begin{comment}
\begin{align}
  \hbar
  g_{\bar{1}1}
  T_{n-1}\left(\infty\right)
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{1}1}
  \nonumber
  \\
  &
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
  }
  \nonumber
  \\
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{1}1}
  \nonumber
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{1}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{1}{2}
    \right]
  }.
  \label{hg11_calc}
\end{align}

\noindent
where 
\(
  \left[
    \cdot
  \right]
  :
  \mathbb{R}
  \to
  \mathbb{Z}
\) 
is Gauss symbol. Similarly for 
\(
  \hbar
  g_{\bar{1}2}
  F_{d}\left(\infty\right)
  T_{n-1}\left(\infty\right),
\) 
\(
  \hbar
  g_{\bar{2}1}
  T_{n-1}\left(\infty\right)
  F_{r}\left(\infty\right)
\) 
and 
\(
  \hbar
  g_{\bar{2}2}
  F_{d}\left(\infty\right)
  T_{n-1}\left(\infty\right)
  F_{r}\left(\infty\right),
\) we obtain

\begin{align}
  %12
  \hbar
  g_{\bar{1}2}
  F_{d}\left(\infty\right)
  T_{n-1}\left(\infty\right)
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{1}2}
  \nonumber
  \\
  &
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
    +
    1
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
  }
  \nonumber
  \\
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{1}2}
  \nonumber
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{2}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{1}{2}
    \right]
  },
  \label{hg12_calc}
  \\
  %21
  \hbar
  g_{\bar{2}1}
  T_{n-1}\left(\infty\right)
  F_{r}\left(\infty\right)
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{2}1}
  \nonumber
  \\
  &
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
    +
    1
  }
  \nonumber
  \\
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{2}1}
  \nonumber
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{1}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{2}{2}
    \right]
  },
  \label{hg21_calc}
  \\
  %22
  \hbar
  g_{\bar{2}2}
  F_{d}\left(\infty\right)
  T_{n-1}\left(\infty\right)
  F_{r}\left(\infty\right)
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{2}2}
  \nonumber
  \\
  &
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
    +
    1
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
    +
    1
  }
  \nonumber
  \\
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\bar{2}2}
  \nonumber
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{2}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
    +
    \left[
      \frac{2}{2}
    \right]
  }.
  \label{hg22_calc}
\end{align}
\end{comment}

\begin{align}
  \hbar
  C_{n}^{'}\left(\infty\right)
  =&
  \hbar
  \left(
    g_{\bar{1}1}
    T_{n-1}\left(\infty\right)
    +
    g_{\bar{1}2}
    F_{d}\left(\infty\right)
    T_{n-1}\left(\infty\right)
    -
    g_{\bar{2}1}
    T_{n-1}\left(\infty\right)
    F_{r}\left(\infty\right)
    -
    g_{\bar{2}2}
    F_{d}\left(\infty\right)
    T_{n-1}\left(\infty\right)
    F_{r}\left(\infty\right)
  \right),
  \nonumber
  \\
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{p_{n}=1}^{4}
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  \left(
    \Theta_{1}^{p_{n}}
    \mathrm{Id}\left(\infty\right)
    +
    \Theta_{2}^{p_{n}}
    F_{d}\left(\infty\right)
  \right)
  \nonumber
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
  }
  \left(
    \Theta_{\bar{1}}^{p_{n}}
    \mathrm{Id}\left(\infty\right)
    -
    \Theta_{\bar{2}}^{p_{n}}
    F_{r}\left(\infty\right)
  \right)
  .
  \label{Cn_CP2_mid}
\end{align}

\noindent
Here 
\(
  \Theta_{\bar{\mu}}^{i_{k}},
  \Theta_{\nu}^{i_{k}}
  \in
  C^{\infty}
  \left(
    U
  \right)
\) 
are the \(C^\infty\) functions such that 
\(
  g_{\overline{\mu}\nu}
  =
  \sum_{i_{k}=1}^{4}
  \Theta_{\bar{\mu}}^{i_{k}}
  \Theta_{\nu}^{i_{k}}
\). 
We can choose 
\(
  \Theta_{\bar{\mu}}^{i_{k}}
\) 
and 
\(
  \Theta_{\nu}^{i_{k}}
\) 
concretely %(See \cite{OS_Varna})
\cite{OS_Varna}, but we do not have to. This is because we can carry out the following calculations without using concrete expressions. The right-hand side of \eqref{Cn_CP2_mid} can be rewritten as
\begin{align}
  &
  \sum_{p_{n}=1}^{4}
  \left(
    \Theta_{1}^{p_{n}}
    \mathrm{Id}\left(\infty\right)
    +
    \Theta_{2}^{p_{n}}
    F_{d}\left(\infty\right)
  \right)
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n-1\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n-1\right)}
    \right)
  }
  \left(
    \Theta_{\bar{1}}^{p_{n}}
    \mathrm{Id}\left(\infty\right)
    -
    \Theta_{\bar{2}}^{p_{n}}
    F_{r}\left(\infty\right)
  \right)
  &
  \nonumber
  \\
  &=
  \sum_{\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    2
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \left(
      \sum_{k=1}^{n-1}
      \left[
        \frac{\nu_{k}}{2}
      \right]
    \right)
    +
    \left[
      \frac{\nu_{n}}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \left(
      \sum_{k=1}^{n-1}
      \left[
        \frac{\mu_{k}}{2}
      \right]
    \right)
    +
    \left[
      \frac{\mu_{n}}{2}
    \right]
  },
  \label{Cn_rhs_mtx}
\end{align}
\noindent
%By using 
where we use 
\(
  \gamma
  \left(
    \mu^{\left(n-1\right)}
  \right)
  =
  \sum_{k=1}^{n-1}
  \left[
    \frac{\mu_{k}}{2}
  \right]
\), 
\(
  \gamma
  \left(
    \nu^{\left(n-1\right)}
  \right)
  =
  \sum_{k=1}^{n-1}
  \left[
    \frac{\nu_{k}}{2}
  \right]
\) 
and also introduce a new indices \(\mu_{n}\) and \(\nu_{n}\). 
\(
  \left(
    1
    -
    2
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
\) 
in the right-hand side of \eqref{Cn_rhs_mtx} is sign \(\pm1\) using the Gauss symbol and \(-1\) when \(\mu_{n}=2\). Then we obtain
\begin{flalign*}
%  \frac{
%    \hbar
%    \Gamma
%    \left(
%      1
%      -
%      \left(
%        n-1
%      \right)
%      +
%      \frac{1}{\hbar}
%    \right)
%  }{
%    \left(
%      n-1
%    \right)!
%    \Gamma
%    \left(
%      1
%      +
%      \frac{1}{\hbar}
%    \right)
%  }
%  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
%  g_{\overline{\mu_{1}}\nu_{1}}
%  \cdots
%  g_{\overline{\mu_{n-1}}\nu_{n-1}}
%  g_{\bar{1}1}
%  \\
%  &
%  \cdot
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{1}{2}
%    \right]
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{1}{2}
%    \right]
%  }
%  \\
%  &
%  +
%  \frac{
%    \hbar
%    \Gamma
%    \left(
%      1
%      -
%      \left(
%        n-1
%      \right)
%      +
%      \frac{1}{\hbar}
%    \right)
%  }{
%    \left(
%      n-1
%    \right)!
%    \Gamma
%    \left(
%      1
%      +
%      \frac{1}{\hbar}
%    \right)
%  }
%  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
%  g_{\overline{\mu_{1}}\nu_{1}}
%  \cdots
%  g_{\overline{\mu_{n-1}}\nu_{n-1}}
%  g_{\bar{1}2}
%  \\
%  &
%  \cdot
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{2}{2}
%    \right]
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{1}{2}
%    \right]
%  }
%  \\
%  &
%  -
%  \frac{
%    \hbar
%    \Gamma
%    \left(
%      1
%      -
%      \left(
%        n-1
%      \right)
%      +
%      \frac{1}{\hbar}
%    \right)
%  }{
%    \left(
%      n-1
%    \right)!
%    \Gamma
%    \left(
%      1
%      +
%      \frac{1}{\hbar}
%    \right)
%  }
%  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
%  g_{\overline{\mu_{1}}\nu_{1}}
%  \cdots
%  g_{\overline{\mu_{n-1}}\nu_{n-1}}
%  g_{\bar{2}1}
%  \\
%  &
%  \cdot
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{1}{2}
%    \right]
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{2}{2}
%    \right]
%  }
%  \\
%  &
%  -
%  \frac{
%    \hbar
%    \Gamma
%    \left(
%      1
%      -
%      \left(
%        n-1
%      \right)
%      +
%      \frac{1}{\hbar}
%    \right)
%  }{
%    \left(
%      n-1
%    \right)!
%    \Gamma
%    \left(
%      1
%      +
%      \frac{1}{\hbar}
%    \right)
%  }
%  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n-1},\nu_{n-1}=1}^{2}
%  g_{\overline{\mu_{1}}\nu_{1}}
%  \cdots
%  g_{\overline{\mu_{n-1}}\nu_{n-1}}
%  g_{\bar{2}2}
%  \\
%  &
%  \cdot
%  \left(
%    F_{d}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \nu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{2}{2}
%    \right]
%  }
%  T_{0}\left(\infty\right)
%  \left(
%    F_{r}\left(\infty\right)
%  \right)^{
%    \gamma
%    \left(
%      \mu^{\left(n-1\right)}
%    \right)
%    +
%    \left[
%      \frac{2}{2}
%    \right]
%  }
  \hbar
  C_{n}^{'}\left(\infty\right)
  =&
%  \hbar
%  \left(
%    g_{\bar{1}1}
%    T_{n-1}\left(\infty\right)
%    +
%    g_{\bar{1}2}
%    F_{d}\left(\infty\right)
%    T_{n-1}\left(\infty\right)
%    -
%    g_{\bar{2}1}
%    T_{n-1}\left(\infty\right)
%    F_{r}\left(\infty\right)
%    -
%    g_{\bar{2}2}
%    F_{d}\left(\infty\right)
%    T_{n-1}\left(\infty\right)
%    F_{r}\left(\infty\right)
%  \right)
%  \\
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \left(
    1
    -
    2
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
%  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\overline{\mu_{n}}\nu_{n}}
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \sum_{k=1}^{n-1}
    \left(
    \left[
      \frac{\nu_{k}}{2}
    \right]
    \right)
    +
    \left[
      \frac{\nu_{n}}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \sum_{k=1}^{n-1}
    \left(
    \left[
      \frac{\mu_{k}}{2}
    \right]
    \right)
    +
    \left[
      \frac{\mu_{n}}{2}
    \right]
  }.
\end{flalign*}
\noindent
Using
\begin{align*}
  \gamma
  \left(
    \mu^{\left(n\right)}
  \right)
  =
  \left(
    \sum_{k=1}^{n-1}
    \left[
      \frac{\mu_{k}}{2}
    \right]
  \right)
  +
  \left[
    \frac{\mu_{n}}{2}
  \right],
  \qquad
  \gamma
  \left(
    \nu^{\left(n\right)}
  \right)
  =
  \left(
    \sum_{k=1}^{n-1}
    \left[
      \frac{\nu_{k}}{2}
    \right]
  \right)
  +
  \left[
    \frac{\nu_{n}}{2}
  \right],
\end{align*}

\noindent
we have
\begin{align}
  &
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
%  \sum_{\mu_{n},\nu_{n}=1}^{2}
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    2
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n-1}}\nu_{n-1}}
  g_{\overline{\mu_{n}}\nu_{n}}
  \nonumber
  \\
  &
  \mbox{}
  \quad
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \left(
      \sum_{k=1}^{n-1}
      \left[
        \frac{\nu_{k}}{2}
      \right]
    \right)
    +
    \left[
      \frac{\nu_{n}}{2}
    \right]
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \left(
      \sum_{k=1}^{n-1}
      \left[
        \frac{\mu_{k}}{2}
      \right]
    \right)
    +
    \left[
      \frac{\mu_{n}}{2}
    \right]
  }
  \nonumber
  \\
  &=
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    2
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  \nonumber
  \\
  &=
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \cdot
    n
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \nonumber
  \\
  &
  \mbox{}
  \quad
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }.
  \label{another_CP2_before}
\end{align}

\noindent
%Here, by 
By replacing the indices, 
%it can be
the above is expressed as
\begin{align}
  &
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \cdot
    n
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  \nonumber
  \\
  &=
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \underbrace{
      \frac{2}{n}
      \left[
        \frac{\mu_{n}}{2}
      \right]
      -
      \cdots
      -
      \frac{2}{n}
      \left[
        \frac{\mu_{n}}{2}
      \right]
    }_{n}
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  \nonumber
  \\
  &=
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \left[
      \frac{\mu_{1}}{2}
    \right]
    -
    \cdots
    -
    \frac{2}{n}
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }.
  \label{gamma_trans_CP2}
\end{align}

\noindent
Substituting \eqref{gamma_trans_CP2} into \eqref{another_CP2_before}, we have
\begin{flalign*}
  &
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \cdot
    n
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  &
  \\
  &
  \mbox{}
  \quad
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  &
  \\
  &=
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \left[
      \frac{\mu_{1}}{2}
    \right]
    -
    \cdots
    -
    \frac{2}{n}
    \left[
      \frac{\mu_{n}}{2}
    \right]
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  &
  \\
  &
  \mbox{}
  \quad
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }
  \\
  &=
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  &
  \\
  &
  \mbox{}
  \quad
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }.
  &
\end{flalign*}

\noindent
Hence,
\begin{align}
  \hbar
  C_{n}^{'}\left(\infty\right)
  =&
  \frac{
    \hbar
    \Gamma
    \left(
      1
      -
      \left(
        n-1
      \right)
      +
      \frac{1}{\hbar}
    \right)
  }{
    \left(
      n-1
    \right)!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  \left(
    1
    -
    \frac{2}{n}
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  \right)
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \nonumber
  \\
  &
  \cdot
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  }.
  \label{another_rhs_CP2}
\end{align}

\noindent
From \eqref{another_lhs_CP2_calc} and \eqref{another_rhs_CP2} it is shown 
%can be verified 
that \eqref{formula_CP2} satisfies \eqref{minus_thm_N2_eq_rsz} in Subsection \ref{NR_minus} for the \(\mathbb{C}P^{2}\) case.


==> EX/NCK2_CP2_journal.tex <==
\subsection{Example for \(\mathbb{C}P^{2}\)}
\label{subsec_NR_CP2}
\ As another concrete example, we shall consider a deformation quantization with separation of variables for \(\mathbb{C}P^{2}.\) Previous works related to deformation quantizations for \(\mathbb{C}P^{N}\) are known so far, such as the results of Omori-Maeda-Yoshioka \cite{OMY2}, Bordemann et al. \cite{BBEW}, Hayasaka-Nakayama-Takaya \cite{HNT}, Sako-Suzuki-Umetsu \cite{SSU1}, and Hara-Sako \cite{HS}. We present the formula for \(T_{n}\left(\infty\right)\) such that it gives a star product with separation of variables for \(\mathbb{C}P^{2}.\)

\begin{theorem}
The formula for determining a star product with separation of variables on \(\mathbb{C}P^{2}\) is given by
\begin{align}
  T_{n}\left(\infty\right)
  =
  \frac{
    \Gamma
    \left(
      1
      -
      n
      +
      \frac{1}{\hbar}
    \right)
  }{
    n!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \sum_{\mu_{1},\nu_{1},\cdots,\mu_{n},\nu_{n}=1}^{2}
  g_{\overline{\mu_{1}}\nu_{1}}
  \cdots
  g_{\overline{\mu_{n}}\nu_{n}}
  \left(
    F_{d}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \nu^{\left(n\right)}
    \right)
  }
  T_{0}\left(\infty\right)
  \left(
    F_{r}\left(\infty\right)
  \right)^{
    \gamma
    \left(
      \mu^{\left(n\right)}
    \right)
  },
  \label{formula_CP2}
\end{align}
where
\(
  \gamma\left(\cdot\right)
  :
  \left\{
    1,2
  \right\}^{n}
  \to
  \mathbb{Z}_{\geq0}
\) 
is defined by
\begin{align*}
  \gamma
  \left(
    \mu^{\left(n\right)}
  \right)
  :=
  \sum_{k=1}^{2}
  \left[
    \frac{\mu_{k}}{2}
  \right],
  \
  \gamma
  \left(
    \nu^{\left(n\right)}
  \right)
  :=
  \sum_{k=1}^{2}
  \left[
    \frac{\nu_{k}}{2}
  \right]
\end{align*}

\noindent
for multi-indices
\(
  \mu^{\left(n\right)}
  =
  \left(
    \mu_{1},
    \cdots,
    \mu_{n}
  \right),
  \nu^{\left(n\right)}
  =
  \left(
    \nu_{1},
    \cdots,
    \nu_{n}
  \right).
\)
\label{thm_Tn_CP2}
\end{theorem}

\noindent
By Theorem \ref{thm_Tn_CP2}, we have
\begin{align*}
  f
  \ast
  g
  =
  \sum_{n=0}^{\infty}
  \frac{
    \Gamma
    \left(
      1
      -
      n
      +
      \frac{1}{\hbar}
    \right)
    g_{\overline{\mu_{1}}\nu_{1}}
    \cdots
    g_{\overline{\mu_{n}}\nu_{n}}
  }{
    n!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \left(
    D^{\nu_{1}}
    \cdots
    D^{\nu_{n}}
    f
  \right)
  \left(
    D^{\overline{\mu_{1}}}
    \cdots
    D^{\overline{\mu_{n}}}
    g
  \right).
\end{align*}

\noindent
This implies that \eqref{formula_CP2} reproduces the results by Sako-Suzuki-Umetsu \cite{SSU1}. As in the case of \(\mathbb{C}^{2},\) \eqref{formula_CP2} satisfies \eqref{minus_thm_N2_eq} in Thm.\ref{minus_thm_N2} for \(n=2.\)


==> EX/NCK2_Previous.tex <==
\subsection{Previous results for \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\)}
\label{subsec_prev_C_CP}

%\ Karabegov proposed the deformation quantization with separation of variables for K\"{a}hler manifolds and denoted noncommutative \(\mathbb{C}^{N}\) as the concrete example. %And previous results of Noncommutative \(\mathbb{C}P^{N}\) are known as some results \cite{BDMLO,BBEW,HNT,HS1,HS2,OMY2,SSU1,SSU2,SU1,SU2,SU3}. 
%It is known that noncommutative \(\mathbb{R}^{2N}\) is the most trivial noncommutative manifold. We can say that noncommutative \(\mathbb{R}^{2N}\) is first obtained by Dirac \cite{Dirac} because canonical quantization is the quantization of phase space \(\mathbb{R}^{2N}\).
%It is known that noncommutative \(\mathbb{R}^{2N}\) is the most trivial noncommutative manifold. We can say that the quantization map from \(\mathbb{R}^{2N}\) to noncommutative \(\mathbb{R}^{2N}\) is introduced by Dirac \cite{Dirac} because canonical quantization is the quantization of phase space \(\mathbb{R}^{2N}\). 
\ It is known that noncommutative \(\mathbb{R}^{2N}\) is the most trivial noncommutative manifold. We can say that the quantization map from \(\mathbb{R}^{2N}\) to noncommutative \(\mathbb{R}^{2N}\) is introduced by Dirac \cite{Dirac} because the canonical quantization is the quantization of phase space \(\mathbb{R}^{2N}\). 
%In the strict case, Noncommutative plane has also proposed by Rieffel from the perspective of \(C^{\ast}\)-algebra \cite{Rief2}. On the other hand, the deformation quantization of \(\mathbb{R}^{2N}\) is also the most trivial example in the formal case.
In the strict deformation quantization case, the noncommutative plane has also been proposed by Rieffel from the perspective of \(C^{\ast}\)-algebra \cite{Rief2}. On the other hand, the deformation quantization of \(\mathbb{R}^{2N}\) is also the most trivial example in the formal deformation quantization case. In particular, the Moyal product \cite{Moya} and the Voros product \cite{Voro} are well-known examples of star products on \(\mathbb{R}^{2N}\). %Here, a noncommutative \(\mathbb{R}^{2N}\) can be regarded as a noncommutative \(\mathbb{C}^{N}\)%, since \(\mathbb{C}^{N}\) is homeomorphic to \(\mathbb{R}^{2N}\)
%. For noncommutative \(\mathbb{C}^{N}\), it is provided the concrete construction by using the deformation quantization with separation of variables by Karabegov as the concrete example \cite{Kara1}.
Here, a noncommutative \(\mathbb{R}^{2N}\) can be regarded as a noncommutative \(\mathbb{C}^{N}\). 
%For noncommutative \(\mathbb{C}^{N}\), the concrete construction is provided by using the deformation quantization with separation of variables by Karabegov as the concrete example \cite{Kara1}. 
For noncommutative \(\mathbb{C}^{N}\), the concrete construction is provided by using the deformation quantization with separation of variables by Karabegov as an example \cite{Kara1}. 
%As another concrete example, we shall consider a deformation quantization with separation of variables for %\(\mathbb{C}P^{2}.\)
%\(\mathbb{C}P^{2}\). 
%Previous works related to deformation quantizations for \(\mathbb{C}P^{N}\) are known, for example Omori-Maeda-Yoshioka \cite{OMY2}, Bordemann et al. \cite{BBEW}, Balachandran et al. \cite{BDMLO}, Hayasaka-Nakayama-Takaya \cite{HNT}, Sako-Suzuki-Umetsu \cite{SSU1,SSU2,SU1,SU2,SU3}, and Hara-Sako \cite{HS1,HS2}.
%Previous works related to noncommutative \(\mathbb{C}P^{N}\) are known approaches from deformation quantizations and fuzzy physics. Noncommutative \(\mathbb{C}P^{N}\) via a deformation quantizations had constructed by Omori-Maeda-Yoshioka \cite{OMY2}, Bordemann et al. \cite{BBEW}, Sako-Suzuki-Umetsu \cite{SSU1,SSU2,SSU3}, and Hara-Sako \cite{HS1,HS2}. 
%Previous works related to noncommutative \(\mathbb{C}P^{N}\) are known approaches from deformation quantizations and fuzzy physics.
As another concrete example, we shall consider here a deformation quantization with separation of variables for \(\mathbb{C}P^{2}\). Previous works related to noncommutative \(\mathbb{C}P^{N}\) are known from deformation quantizations and fuzzy geometry. Noncommutative \(\mathbb{C}P^{N}\) via a deformation quantizations had constructed by Omori-Maeda-Yoshioka \cite{OMY2}, Bordemann et al. \cite{BBEW}, Sako-Suzuki-Umetsu \cite{SSU1,SSU2}, and Hara-Sako \cite{HS1,HS2}. 
%In addition, the (twisted) Fock representation of noncommutative \(\mathbb{C}P^{N}\) was first given by Sako-Suzuki-Umetsu \cite{SSU1,SSU2,SSU3}.
In addition, the (twisted) Fock representation of noncommutative \(\mathbb{C}P^{N}\) was given by Sako-Suzuki-Umetsu \cite{SSU1,SSU2} and Sako-Umetsu \cite{SU1,SU2,SU3}. It is known that this representation is 
%essencially 
essentially equivalent to ordinary Fock representation. 
%In fuzzy physics, noncommutative \(\mathbb{C}P^{N}\), called fuzzy \(\mathbb{C}P^{N}\), had constructed via a matrix algebra. The construction methods of fuzzy sphere, i.e. fuzzy \(\mathbb{C}P^{1}\), had proposed by Hoppe \cite{Hop} and Madore \cite{Mad1}. Furthermore, more general works were later proposed by Grosse-Strohmaier \cite{GS} and Alexanian et al. \cite{ABIY} for fuzzy \(\mathbb{C}P^{2}\), and by Carow-Watamura-Steinacker-Watamura \cite{CSW} for \(\mathbb{C}P^{N}\). See \cite{Mad2} for other references. 
On the other hand, in fuzzy physics, noncommutative \(\mathbb{C}P^{N}\), called fuzzy \(\mathbb{C}P^{N}\), had constructed via a matrix algebra. 
%The construction methods of fuzzy \(S^{2}\), i.e. fuzzy \(\mathbb{C}P^{1}\), had proposed by Hoppe \cite{Hop} and Madore \cite{Mad1}. Furthermore, more general works were later proposed by Grosse-Strohmaier \cite{GS} and Alexanian et al. \cite{ABIY} for fuzzy \(\mathbb{C}P^{2}\), and by Carow-Watamura-Steinacker-Watamura \cite{CSW} for \(\mathbb{C}P^{N}\). 
%The construction methods of fuzzy \(S^{2}\), i.e. fuzzy \(\mathbb{C}P^{1}\), had proposed by Hoppe \cite{Hop}, Madore \cite{Mad1} and Hayasaka-Nakayama-Takaya \cite{HNT}.
The construction methods of fuzzy \(S^{2}\), i.e. fuzzy \(\mathbb{C}P^{1}\), had proposed by Hoppe \cite{Hop} and Madore \cite{Mad1}. Hayasaka-Nakayama-Takaya constructed a star product on \(S^{2}\) from their fuzzy \(S^{2}\) \cite{HNT}. %Furthermore, more general works were later proposed by Grosse-Strohmaier \cite{GS}, Alexanian et al. \cite{ABIY} for fuzzy \(\mathbb{C}P^{2}\), and by Balachandran et al. \cite{BDMLO}, Carow-Watamura-Steinacker-Watamura \cite{CSW} for \(\mathbb{C}P^{N}\). See \cite{Mad2} for other references.
Furthermore, more general works were proposed by Grosse-Strohmaier \cite{GS}, Alexanian et al. \cite{ABIY} for fuzzy \(\mathbb{C}P^{2}\), and by Balachandran et al. \cite{BDMLO}, Carow-Watamura-Steinacker-Watamura \cite{CSW} for \(\mathbb{C}P^{N}\). See \cite{Mad2} for other references. In particular, the Fock representation on fuzzy \(\mathbb{C}P^{N}\) was also discussed by Alexanian-Pinzul-Stern \cite{APS} and them. 
%In %Section \ref{subsec_prev_C_CP}
%this subsection, we introduce the %result
%results of noncommutative \(\mathbb{C}^{2}\) by Karabegov and Voros, and noncommutative \(\mathbb{C}P^{2}\) by Sako-Suzuki-Umetsu to compare %later discussions.
%them with results given in the following sections.
In this subsection, we introduce the results of noncommutative \(\mathbb{C}^{2}\) by Karabegov and Voros, and noncommutative \(\mathbb{C}P^{2}\) by Sako-Suzuki-Umetsu to compare them with results given by Theorem \ref{main_thm_N2} in the following sections.
\begin{theorem}[Karabegov\cite{Kara2}]
For any 
\(
  f,g
  \in
  C^{\infty}
  \left(\mathbb{C}^{2}\right)
\), 
the star product with separation of variables on \(\mathbb{C}^{2}\) is locally given by
\begin{align}
  f
  \ast
  g
  =
  f
  \mathrm{exp}
  \nu
  \left(
    \overleftarrow{
      \partial_{\overline{z}^{1}}
    }
    \overrightarrow{
      \partial_{z^{1}}
    }
    +
    \overleftarrow{
      \partial_{\overline{z}^{2}}
    }
    \overrightarrow{
      \partial_{z^{2}}
    }
  \right)
  g.
  \label{star_prd_C2_Kara_Voro_sol}
\end{align}
\label{star_prd_C2_Kara_Voro}
\end{theorem}
\noindent
It is known as the star product which is called ``Voros product" \cite{Voro} and %equivalent to 
isomorphic to Moyal product \cite{Moya}. %A simple proof is given by, for example, Section 2.2 in \cite{APS}.
A simple proof for the isomorphism of them is given by, for example, Section 2.2 in \cite{APS}. %This star product is called the Wick type \cite{BBEW,BW1,BW2}. 
The star product \eqref{star_prd_C2_Kara_Voro_sol} is sometimes called the ``Wick product" \cite{BBEW,BW1,BW2}. For \(\mathbb{C}P^{N}\), the noncommutative one had been constructed by several previous works. In Section \ref{subsec_NR_CP2}, we compare the star product on \(\mathbb{C}P^{2}\) obtained by Theorem \ref{main_thm_N2} with the previous work by Sako-Suzuki-Umetsu. So we denote the result for \(\mathbb{C}P^{2}\) by them.
\begin{theorem}[Sako-Suzuki-Umetsu\cite{SSU1,SSU2}]
For any 
\(
  f,g
  \in
  C^{\infty}
  \left(\mathbb{C}P^{2}\right)
\), 
the star product with separation of variables on \(\mathbb{C}P^{2}\) is locally given by
\begin{align}
  f
  \ast
  g
  =
  \sum_{n=0}^{\infty}
  \frac{
    \Gamma
    \left(
      1
      -
      n
      +
      \frac{1}{\hbar}
    \right)
    g_{\overline{\mu_{1}}\nu_{1}}
    \cdots
    g_{\overline{\mu_{n}}\nu_{n}}
  }{
    n!
    \Gamma
    \left(
      1
      +
      \frac{1}{\hbar}
    \right)
  }
  \left(
    D^{\nu_{1}}
    \cdots
    D^{\nu_{n}}
    f
  \right)
  \left(
    D^{\overline{\mu_{1}}}
    \cdots
    D^{\overline{\mu_{n}}}
    g
  \right).
  \label{star_prd_C2_SSU_sol}
\end{align}
\label{star_prd_C2_SSU}
\end{theorem}
\noindent
Here \(\mu_{k}, \nu_{k}=1,2\). %And note 
Note that we use the Einstein summation convention in Theorem \ref{star_prd_C2_SSU}. In \cite{SSU1,SSU2}, it is confirmed that the star product on \(\mathbb{C}P^{N}\) coincides with one obtained by Bordemann et al. \cite{BBEW}. See \cite{SSU1,SSU2} for more detail.
%%ここでKarabegovによるNoncommutative \(\mathbb{C}^{2}\)およびSako-Suzuki-UmetsuによるNoncommutative \(\mathbb{C}P^{2}\)についての結果，もといstar productの具体形を示す．Karabegovの結果については具体形を明示的に書いた論文がSako-Umetsuであるが，これについてはKarabegovの結果と称す．ただしその時点でもKronecker deltaがそのままだったりするので，より具体的な形（即ち計算結果と同じ形）を示す．またこれがVoros product（即ちVorosによるstar productそのもの）であることを述べ，更にこれがMoyal productと等価（正確に言えば変形量子化として同値であり，適切なintertwinerを通した変換則が作れる）であることを説明する．Sako-Suzuki-Umetsuの結果については特に具体形に変更はないので，同じ形で引用する．


==> NCK2_NewResult.tex <==
\section{Star product with separation of variables for a complex\\
two-dimensional locally symmetric K\"{a}hler manifold}
\label{NEW_RESULT}
\ In this section, we construct %describe 
the formula that explicitly determines a star product with separation of variables %such that they give a deformation quantization with separation of variables 
for a complex two-dimensional locally symmetric K\"{a}hler manifold. 
% obtained as our main result in this work.
In other words, we construct the solution of the recurrence relations in Theorem \ref{theorem:star_prd} for the two-dimensional case in this section.
\input{NR/NCK2_plus.tex}
\input{NR/NCK2_minus.tex}


==> NCK2_appA.tex <==
\appendix
\section{Some properties from K\"{a}hler geometry}
\label{app_kaehler}
\ We review some properties for K\"{a}hler manifolds that we use in this paper. See Kobayashi-Nomizu for more details \cite{KN}. Let \(M\) be a complex \(N\)-dimensional K\"{a}hler manifold, \(U\) be a holomorphic coordinate neighborhood of \(M\), and \(\nabla\) be the Levi-Civita connection on \(M\). For 
\(
  \partial_{B},
  \partial_{C}
  \in
  \Gamma\left(
    TM
    \left.
    \right|_{U}
  \right),
\) 
the Christoffel symbol \(\Gamma_{BC}^{A}\) is defined by 
\(
  \nabla_{\partial_{B}}
  \partial_{C}
  =
  \Gamma_{BC}^{A}
  \partial_{A},
\)
where 
\(
  A,B,C
  \in
  \left\{
    1,
    \cdots,
    N,
    \overline{1},
    \cdots,
    \overline{N}
  \right\},
  \
  \partial_{A}
  :=
  \frac{\partial}{\partial z^{A}},
\) 
and 
\(
  z^{\overline{i}}
  :=
  \overline{z}^{i}
\) 
for 
\(
  i
  \in
  \left\{
    1,
    \cdots,
    N
  \right\}.
\) 
In particular, \(\Gamma_{BC}^{A}\) is given by
\begin{align*}
  \Gamma_{BC}^{A}
  =
  \frac{1}{2}
  g^{AD}
  \left(
    \partial_{B}
    g_{DC}
    +
    \partial_{C}
    g_{DB}
    -
    \partial_{D}
    g_{BC}
  \right)
\end{align*}

\noindent
by using the components of the K\"{a}hler metric \(g\). Since \(M\) is K\"{a}hler, the non-trivial Christoffel symbols are \(\Gamma^{k}_{ij}\) and \(\Gamma^{\overline{k}}_{\overline{i}\,\overline{j}}\), where 
\(
  i,
  j,
  k
  \in
  \left\{
    1,
    \cdots,
    N
  \right\}.
\) 
Furthermore, the covariant derivative for \((k,l)\)-tensor field 
\(
  Y
  ^{
    A_{1}
    \cdots
    A_{k}
  }
  _{
    B_{1}
    \cdots
    B_{l}
  }
  \partial_{A_{1}}
  \otimes
  \cdots
  \otimes
  \partial_{A_{k}}
  \otimes
  dz^{B_{1}}
  \otimes
  \cdots
  \otimes
  dz^{B_{l}}
  \in
  \Gamma
  (
    (
      TM
    )^{
      \otimes
      k
    }
    \otimes
    (
      T^{^{\ast}}M
    )^{
      \otimes
      l
    }
  )
\) 
is given by using the Christoffel symbol as follows : 
\begin{align*}
  &
  \nabla_{\partial_{C}}
  \left(
    Y
    ^{
      A_{1}
      \cdots
      A_{k}
    }
    _{
      B_{1}
      \cdots
      B_{l}
    }
    \partial_{A_{1}}
    \otimes
    \cdots
    \otimes
    \partial_{A_{k}}
    \otimes
    dz^{B_{1}}
    \otimes
    \cdots
    \otimes
    dz^{B_{l}}
  \right)
  \\
  =&
  \left(
    \partial_{C}
    Y
    ^{
      \mu_{1}
      \cdots
      \mu_{k}
      \overline{\mu_{1}}
      \cdots
      \overline{\mu_{m}}
    }
    _{
      \nu_{1}
      \cdots
      \nu_{l}
      \overline{\nu_{1}}
      \cdots
      \overline{\nu_{n}}
    }
    +
    \sum_{q=1}^{k}
    \Gamma^{A_{q}}_{CD}
    Y
    ^{
      A_{1}
      \cdots
      A_{q-1}
      D
      A_{q+1}
      \cdots
      A_{k}
    }
    _{
      B_{1}
      \cdots
      B_{l}
    }
    -
    \sum_{q=1}^{l}
    \Gamma^{D}_{CB_{q}}
    Y
    ^{
      A_{1}
      \cdots
      A_{k}
    }
    _{
      B_{1}
      \cdots
      B_{q-1}
      D
      B_{q+1}
      \cdots
      B_{l}
    }
  \right)
  \\
  &
  \times
  \partial_{A_{1}}
  \otimes
  \cdots
  \otimes
  \partial_{A_{k}}
  \otimes
  dz^{B_{1}}
  \otimes
  \cdots
  \otimes
  dz^{B_{l}},
\end{align*}

\noindent
where 
\(
  A_{1},
  \cdots,
  A_{k},
  B_{1},
  \cdots,
  B_{l},
  C,
  D
  \in
  \left\{
    1,
    \cdots,
    N,
    \overline{1},
    \cdots,
    \overline{N}
  \right\}.
\)
\\
\ Next, we define the Riemann curvature tensor 
\(
  R^{\nabla}
  :
  \Gamma
  \left(
    TM
  \right)
  \times
  \Gamma
  \left(
    TM
  \right)
  \times
  \Gamma
  \left(
    TM
  \right)
  \to
  \Gamma
  \left(
    TM
  \right)
\) 
on \(M\) for the vector fields 
\(
  X,Y
  \in
  \Gamma
  \left(
    TM
  \right)
\) 
and its component 
\(
  R^{\nabla}
  \left(
    \partial_{A},
    \partial_{B}
  \right)
  \partial_{C}
\) 
by 
\begin{align*}
  R^{\nabla}
  \left(
  X,Y
  \right)
  &:=
  \nabla_{X}\nabla_{Y}
  -
  \nabla_{Y}\nabla_{X}
  -
  \nabla_{\left[X,Y\right]},
  \\
  R^{\nabla}
  \left(
    \partial_{A},
    \partial_{B}
  \right)
  \partial_{C}
  &:=
  R_{ABC}^{\quad \ \ \, D}
  \partial_{D},
\end{align*}

\noindent
respectively. 
%Note that the notation of component is based on the notation by Hara-Sako \cite{HS}.
Note that the notation \(R_{ABC}^{\quad \ \ \, D}\) used in this paper can be expressed by the relation
\begin{align}
  R_{ABC}^{\quad \ \ \, D}
  =
  \mathfrak{R}_{\ \,CAB}^{D}
  \label{HS_KN}
\end{align}

\noindent
using the notation
\begin{align*}
  R^{\nabla}
  \left(
    \partial_{A},
    \partial_{B}
  \right)
  \partial_{C}
  :=
  \mathfrak{R}_{\ \,CAB}^{D}
  \partial_{D}
\end{align*}

\noindent
by Kobayashi-Nomizu \cite{KN}. In this paper, we fix the position of the indices of the components of the Riemann curvature tensor in the above equation. The components \(R_{ABC}^{\quad \ \ \, D}\) are also given by
\begin{align*}
  R_{ABC}^{\quad \ \ \, D}
  =
  \partial_{A}
  \Gamma_{BC}^{D}
  -
  \partial_{B}
  \Gamma_{AC}^{D}
  +
  \Gamma_{BC}^{E}
  \Gamma_{AE}^{D}
  -
  \Gamma_{AC}^{E}
  \Gamma_{BE}^{D}
\end{align*}

\noindent
by using the Christoffel symbols, and their non-trivial ones are
\begin{align*}
  R_{i\overline{j}k}^{\quad \, l}
  &=
  -
  \partial_{\overline{j}}
  \Gamma_{ik}^{l},
  \\
  R_{i\bar{j}\bar{k}}^{\quad \, \bar{l}}
  &=
  \partial_{i}
  \Gamma_{\bar{j}\bar{k}}^{\bar{l}}.
\end{align*}

\noindent
For 
\(
  R_{ABCD}
  =
  g_{DE}
  R_{ABC}^{\quad \ \ \, E},
\) 
it is also confirmed that the non-trivial components are 
\(
  R_{i\overline{j}k\bar{l}}
\) 
and 
\(
  R_{i\bar{j}\bar{k}l},
\) 
which are given by
\begin{align*}
  R_{i\overline{j}k\overline{l}}
  &=
  -
  g_{\overline{l}p}
  \partial_{\overline{j}}
  \Gamma_{ik}^{p}
  =
  -
  \partial_{i}\partial_{\overline{j}}\partial_{k}\partial_{\overline{l}}\Phi
  +
  g^{p\overline{q}}
  \left(
    \partial_{i}\partial_{\overline{q}}\partial_{k}\Phi
  \right)
  \left(
    \partial_{p}\partial_{\overline{j}}\partial_{\overline{l}}\Phi
  \right),
  \\
  R_{i\overline{j}\overline{k}l}
  &=
  g_{l\overline{p}}
  \partial_{i}
  \Gamma_{\overline{j}\overline{k}}^{\overline{p}}
  =
  \partial_{\overline{j}}\partial_{i}\partial_{\overline{k}}\partial_{l}\Phi
  -
  g^{\overline{p}q}
  \left(
    \partial_{\overline{j}}\partial_{q}\partial_{\overline{k}}\Phi
  \right)
  \left(
    \partial_{\overline{p}}\partial_{i}\partial_{l}\Phi
  \right)
\end{align*}

\noindent
respectively, where \(\Phi\) is the K\"{a}hler potential, i.e. \(\Phi\) is a function on \(M\) such that 
\(
  g_{i\overline{j}}
  =
  \partial_{i}
  \partial_{\overline{j}}
  \Phi.
\)
\\
\ Here we consider 
\(
  R_{\bar{i} \ \ \, \bar{c}}^{\ \, \bar{k}\bar{l}}
  =
  g^{\overline{k}p}
  g^{\overline{l}q}
  R_{\overline{i}pq\overline{c}}
\) 
which often appears in this paper. We refer to 
\(
  R_{\bar{i} \ \ \, \bar{c}}^{\ \, \bar{k}\bar{l}}
\) 
simply as ``curvature". This curvature 
\(
  R_{\bar{i} \ \ \, \bar{c}}^{\ \, \bar{k}\bar{l}}
\) 
has the following symmetries %with respect to
concerning the indices 
\(
  \overline{i},
  \overline{c},
  \overline{k},
\)
and
\(
  \overline{l}
\)
 :
\begin{align}
  R_{\bar{i} \ \ \, \bar{c}}^{\ \, \bar{k}\bar{l}}
  =
  R_{\bar{c} \ \ \, \bar{i}}^{\ \, \bar{k}\bar{l}}
  =
  R_{\bar{i} \ \ \, \bar{c}}^{\ \, \bar{l}\bar{k}}
  =
  R_{\bar{c} \ \ \, \bar{i}}^{\ \, \bar{l}\bar{k}}.
  \label{curv_kaehler_prop}
\end{align}

\noindent
This property plays an important role in this paper.
\bigskip
\\
\ We now turn our attention to a locally symmetric K\"{a}hler manifold : the fact that \(M\) is locally symmetric is equivalent to the fact that 
\(
  \nabla_{\partial_{E}}
    R_{ABC}^{\quad \ \ \, D}
    =
    0,
\) 
for 
\(
  A,B,C,D,E
  \in
  \left\{
    1,
    \cdots,
    N,
    \overline{1}.
    \cdots,
    \overline{N}
  \right\}.
\)


==> NCK2_appB.tex <==
%\appendix
\section{Calculations for both sides of \eqref{minus_thm_eq_ens} in Subsection \ref{NR_minus}}
\label{app_minus_n2}

\ We show that \eqref{minus_thm_eq_ens} for \(n=2\) holds in Subsection \ref{NR_minus}. In this appendix, we denote the detailed calculations for each component of both sides of \eqref{minus_thm_eq_ens} in Subsection \ref{NR_minus}. They can be enumerated as follows.
\vspace{3mm}
\\
\noindent
\underline{
  The left-hand side
}
\begin{align}
  \left(1,1\right)
  &=
  \hbar^{2}
  \left\{
    \left(
      2
      +
      \hbar
      R_{1 \ \ \, 1}^{\ \, 11}
    \right)
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    2
    \hbar
    R_{1 \ \ \, 1}^{\ \, 21}
    g_{\overline{1}1}
    g_{\overline{1}2}
    +
    \hbar
    R_{1 \ \ \, 1}^{\ \, 22}
    \left(
      g_{\overline{1}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  \hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    \hbar
    R_{1\bar{1}\bar{1}1}
  \right\},
  \label{lhs_first}
  \\
  \left(1,2\right)
  &=
  2\hbar^{2}
  \left\{
    \left(
	  2
      +
      \hbar
      R_{1 \ \ \, 1}^{\ \, 11}
    \right)
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \hbar
    R_{1 \ \ \, 1}^{\ \, 21}
    \left(
      g_{\overline{1}1}
      g_{\overline{2}2}
      +
      g_{\overline{1}2}
      g_{\overline{2}1}
    \right)
    +
    \hbar
    R_{1 \ \ \, 1}^{\ \, 22}
    g_{\overline{1}2}
    g_{\overline{2}2}
  \right\}
  \nonumber
  \\
  &=
  2\hbar^{2}
  \left\{
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \hbar
    R_{1\bar{2}\bar{1}1}
  \right\},
  \\
  \left(1,3\right)
  &=
  \hbar^{2}
  \left\{
    \left(
	  2
      +
      \hbar
      R_{1 \ \ \, 1}^{\ \, 11}
    \right)
    \left(
      g_{\overline{2}1}
    \right)^{2}
    +
    2
    \hbar
    R_{1 \ \ \, 1}^{\ \, 21}
    g_{\overline{2}1}
    g_{\overline{2}2}
    +
    \hbar
    R_{1 \ \ \, 1}^{\ \, 22}
    \left(
      g_{\overline{2}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  \hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{2}1}
    \right)^{2}
    +
    \hbar
    R_{1\bar{2}\bar{2}1}
  \right\},
  \\
  \left(2,1\right)
  &=
  0,
  \\
  \left(2,2\right)
  &=
  0,
  \\
  \left(2,3\right)
  &=
  0,
  \\
  \left(3,1\right)
  &=
  -
  \hbar^{2}
  \left\{
    \hbar
    R_{2 \ \ \, 2}^{\ \, 11}
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    2
    \hbar
    R_{2 \ \ \, 2}^{\ \, 21}
    g_{\overline{1}1}
    g_{\overline{1}2}
    +
    \left(
      2
      +
      \hbar
      R_{2 \ \ \, 2}^{\ \, 22}
    \right)
    \left(
      g_{\overline{1}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  -\hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{1}2}
    \right)^{2}
    +
    \hbar
    R_{2\bar{1}\bar{1}2}
  \right\},
  \\
  \left(3,2\right)
  &=
  -
  2
  \hbar^{2}
  \left\{
    \hbar
    R_{2 \ \ \, 2}^{\ \, 11}
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \hbar
    R_{2 \ \ \, 2}^{\ \, 21}
    \left(
      g_{\overline{1}1}
      g_{\overline{2}2}
      +
      g_{\overline{1}2}
      g_{\overline{2}1}
    \right)
    +
    \left(
      2
      +
      \hbar
      R_{2 \ \ \, 2}^{\ \, 22}
    \right)
    g_{\overline{1}2}
    g_{\overline{2}2}
  \right\}
  \nonumber
  \\
  &=
  -2\hbar^{2}
  \left\{
    2
    g_{\overline{1}2}
    g_{\overline{2}2}
    +
    \hbar
    R_{2\bar{2}\bar{1}2}
  \right\},
  \\
  \left(3,3\right)
  &=
  -
  \hbar^{2}
  \left\{
    \hbar
    R_{2 \ \ \, 2}^{\ \, 11}
    \left(
      g_{\overline{2}1}
    \right)^{2}
    +
    2
    \hbar
    R_{2 \ \ \, 2}^{\ \, 21}
    g_{\overline{2}1}
    g_{\overline{2}2}
    +
    \left(
      2
      +
      \hbar
      R_{2 \ \ \, 2}^{\ \, 22}
    \right)
    \left(
      g_{\overline{2}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  -\hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{2}2}
    \right)^{2}
    +
    \hbar
    R_{2\bar{2}\bar{2}2}
  \right\}.
\end{align}
\noindent
\underline{
  The right-hand side
}
\begin{align}
  \left(1,1\right)
  &=
  \hbar^{2}
  \left\{
    \left(
      2
      +
      \hbar
      R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    \right)
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    2
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    \left(
      g_{\overline{2}1}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  \hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    \hbar
    R_{1\bar{1}\bar{1}1}
  \right\},
  \\
  \left(1,2\right)
  &=
  2\hbar^{2}
  \left\{
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    \left(
      2
      +
      2
      \hbar
      R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
    \right)
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    \left(
      g_{\overline{2}1}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  2\hbar^{2}
  \left\{
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \hbar
    R_{1\bar{2}\bar{1}1}
  \right\},
  \\
  \left(1,3\right)
  &=
  \hbar^{2}
  \left\{
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}}
    \left(
      g_{\overline{1}1}
    \right)^{2}
    +
    2
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}}
    g_{\overline{1}1}
    g_{\overline{2}1}
    +
    \left(
      2
      +
      \hbar
      R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
    \right)
    \left(
      g_{\overline{2}1}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  \hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{2}1}
    \right)
    +
    \hbar
    R_{1\bar{2}\bar{2}1}
  \right\},
  \\
  \left(2,1\right)
  &=
  0,
  \\
  \left(2,2\right)
  &=
  0,
  \\\left(2,3\right)
  &=
  0,
  \\
  \left(3,1\right)
  &=
  -
  \hbar^{2}
  \left\{
    \left(
      2
      +
      \hbar
      R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    \right)
    \left(
      g_{\overline{1}2}
    \right)^{2}
    +
    2
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
    g_{\overline{1}2}
    g_{\overline{2}2}
    +
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    \left(
      g_{\overline{2}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  -\hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{1}2}
    \right)^{2}
    +
    \hbar
    R_{2\bar{1}\bar{1}2}
  \right\},
  \\
  \left(3,2\right)
  &=
  -2
  \hbar^{2}
  \left\{
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    \left(
      g_{\overline{1}2}
    \right)^{2}
    +
    \left(
      2
      +
      2
      \hbar
      R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
    \right)
    g_{\overline{1}2}
    g_{\overline{2}2}
    +
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    \left(
      g_{\overline{2}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  -2\hbar^{2}
  \left\{
    2
    g_{\overline{1}2}
    g_{\overline{2}2}
    +
    \hbar
    R_{2\bar{2}\bar{1}2}
  \right\},
  \\
  \left(3,3\right)
  &=
  -
  \hbar^{2}
  \left\{
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}}
    \left(
      g_{\overline{1}2}
    \right)^{2}
    +
    2
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}}
    g_{\overline{1}2}
    g_{\overline{2}2}
    +
    \left(
      2
      +
      \hbar
      R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
    \right)
    \left(
      g_{\overline{2}2}
    \right)^{2}
  \right\}
  \nonumber
  \\
  &=
  -\hbar^{2}
  \left\{
    2
    \left(
      g_{\overline{2}2}
    \right)^{2}
    +
    \hbar
    R_{2\bar{2}\bar{2}2}
  \right\}.
  \label{rhs_last}
\end{align}

\noindent
Note that we denote each \(\left(i,j\right)\) component of both sides simply as \(\left(i,j\right)\). Hence, from the calculations \eqref{lhs_first}--\eqref{rhs_last}, \eqref{minus_thm_eq_ens} in Subsection \ref{NR_minus} for \(n=2\) is verified directly.


==> NCK2_appC.tex <==
\section{
Hermiteness of 
\(
  T_{n}
\)
}
\label{prf_Tn_dagger}

In Subsection \ref{NR_minus}, we use the fact that \(T_{n}\) is Hermite conjugate, i.e. 
\(
  T_{n}
  =
  T_{n}^{\dagger}.
\) 
So we shall derive this property of \(T_{n}\) in this appendix.

\begin{lemma}[Sako-Umetsu\cite{SU1}]
  The coefficients \(T_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}^{n}\) satisfy
  \begin{align*}
    T_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}^{n}
    =
    \overline{
      T_{\overrightarrow{\beta_{n}},\,\overrightarrow{\alpha_{n}^{\ast}}}^{n}
    }
  \end{align*}
  
  \noindent
  or equivalently
  \begin{align}
    T_{n}
    =
    T_{n}^{\dagger},
    \label{star_conj_mtx}
  \end{align}
\end{lemma}

\begin{prf*}
%後で以下の文章に変更すること
%From Proposition \ref{star_cplx_conj},
From Proposition 3.1. in \cite{SU1},
\begin{align}
  \overline{
    f
    \ast
    g
  }
  =
  \overline{g}
  \ast
  \overline{f}.
  \label{star_conj}
\end{align}

\noindent
Substituting \eqref{star_expand} into the left-hand side of \eqref{star_conj}, we have
\begin{align*}
  \overline{
    f
    \ast
    g
  }
  =&
  \sum_{n=0}^{\infty}
  \sum_{
    \overrightarrow{\alpha_{n}},
    \overrightarrow{\beta_{n}^{\ast}}
  }
  \overline{
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  }
  \left\{
    \left(
      D^{\overline{1}}
    \right)^{\alpha_{1}^{n}}
    \cdots
    \left(
      D^{\overline{N}}
    \right)^{\alpha_{N}^{n}}
    \overline{f}
  \right\}
  \left\{
    \left(
      D^{1}
    \right)^{\beta_{1}^{n}}
    \cdots
    \left(
      D^{N}
    \right)^{\beta_{N}^{n}}
    \overline{g}
  \right\}
  \\
  =&
  \sum_{n=0}^{\infty}
  \sum_{
    \overrightarrow{\alpha_{n}},
    \overrightarrow{\beta_{n}^{\ast}}
  }
  \overline{
    T_{\overrightarrow{\beta_{n}},\overrightarrow{\alpha_{n}^{\ast}}}^{n}
  }
  \left(
    D^{\overrightarrow{\alpha_{n}}}\overline{g}
  \right)
  \left(
    D^{\overrightarrow{\beta_{n}^{\ast}}}\overline{f}
  \right).
\end{align*}

\noindent
Here we rewrote %rewritten 
the dummy indices in the last equation. On the other hand, since 
\begin{align*}
  \overline{g}
  \ast
  \overline{f}
  =
  \sum_{n=0}^{\infty}
  \sum_{
    \overrightarrow{\alpha_{n}},
    \overrightarrow{\beta_{n}^{\ast}}
  }
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  \left(
    D^{\overrightarrow{\alpha_{n}}}\overline{g}
  \right)
  \left(
    D^{\overrightarrow{\beta_{n}^{\ast}}}\overline{f}
  \right)
\end{align*}

\noindent
by the assumption for the star product with separation of variables, we obtain 
\begin{align*}
  T_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}^{n}
  =
  \overline{
    T_{\overrightarrow{\beta_{n}},\,\overrightarrow{\alpha_{n}^{\ast}}}^{n}
  }
\end{align*}

\noindent
by comparing the coefficients on both sides of \eqref{star_conj}. The above equation can be expressed as an equivalent equation 
\(
  T_{n}
  =
  T_{n}^{\dagger}.
  _{\blacksquare}
\)
\end{prf*}


==> NCK2_discussion.tex <==
\section{Discussions}
\label{DQ_Discussion}
%\ In this paper, we obtained the explicit star product with separation of variables for two-dimensional locally symmetric K\"{a}hler manifold by solving the recurrence relations in \cite{HS1,HS2}. In addition, we gave the noncommutative \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) as concrete examples, and verified that our result works well. We can also explicitly construct other concrete examples of two-dimensional noncommutative locally symmetric K\"{a}hler manifolds. The examples of two-dimensional ones that have not yet been constructed are, for example, quadratic surface \(Q^{2}\), \(\mathbb{C}P^{1}\times\mathbb{C}H^{1}\), and so on. Furthermore, we may be able to propose the physics on noncommutative locally symmetric K\"{a}hler manifolds from our result. For example, the construction of gauge theories, solitons and instantons on noncommutative locally symmetric K\"{a}hler manifolds are expected, since they have already proposed by Nekrasov-Schwarz \cite{NS}, Spradlin-Volovich \cite{SV}, Maeda-Sako \cite{MS1,MS2}, Maeda-Sako-Suzuki-Umetsu \cite{MSSU} and Sako-Suzuki-Umetsu \cite{SSU3}. In particular, the noncommutative instanton on \(\mathbb{C}P^{2}\) have not yet been constructed. By resolving it, we may discover the relation between the noncommutative instanton on \(\mathbb{C}P^{2}\) and Hermitian-Einstein metrics. A previous work by Hara-Sako-Yang is known for \(\mathbb{C}^{2}\). In contrast to the strict case, the formal case is difficult to make sense of the physics. However, it is possible to construct Fock representations in the formal case. In fact, the twsted Fock representations can be constructed by using a formal star product as discussed in Section \ref{DQ_Review}. Recalling that quantium field theory can be stated by using Fock representations, we can expect to propose the quantum field theory on noncommutative K\"{a}hler manifolds. In addition, it is expected to clarify the relationship between fuzzy manifolds and deformation quantization, since Fock representations can be interpreted by using a matrix represenatation. On the other hand, it is known that supersymmetric nonlinear sigma models whose target spaces are K\"{a}hler manifolds studied by Higashijima-Nitta \cite{HN1,HN2,HN3}, Higashijima-Kimura-Nitta \cite{HKN} and Kondo-Takahashi \cite{KT}. They include the models on \(\mathbb{C}P^{N}\) and \(Q^{2}\) as the target spaces. So we may be able to construct the supersymmetric nonlinear sigma models on noncommutative \(\mathbb{C}P^{2}\) and \(Q^{2}\) by using oru result.
%\ In this paper, we obtained the explicit star product with separation of variables for two-dimensional locally symmetric K\"{a}hler manifold by solving the recurrence relations in \cite{HS1,HS2}.\\
%\ On the other hand, it is known that Noncommutative differentiable manifolds are applied for physics. For example, noncommutative solitons on K\"{a}hler manifolds, gauge theories in noncommutative K\"{a}ler manifolds and noncommutative instantons on \(\mathbb{R}^{4}\) \cite{HSY,MS1,MS2,MSSU,NS,SV}.
%%今回の主結果が直接寄与するわけではないものの，話題としてNoncommutative instanton of noncommutative \(\mathbb{C}P^{2}\)の話などを入れる．（メモ：行列サイズの大きさに起因する計算の複雑さが原因で，一般論について証明が与えられていないのが実情らしい．ただ\(\mathbb{C}P^{2}\)についての計算がかつて試みられたのだとか．）
%\ In this paper, we obtained the explicit star product with separation of variables for two-dimensional locally symmetric K\"{a}hler manifold by solving the recurrence relations in \cite{HS1,HS2}. %In other words, we expanded as the previous result for two-dimension in \cite{HS1,HS2} by using a matrix representation. 
%In addition, we verify that the equation \eqref{main_them_N2_Tinf} in Theorem \ref{main_thm_N2} satisfies the identity \eqref{minus_thm_N2_eq_rsz} (or equivalently \eqref{minus_thm_N2_eq_another_rsz}) in Section \ref{NR_minus}. By using Theorem \ref{main_thm_N2}, we can construct a deformation quantization with separation of variables for any complex two-dimensional locally symmetric K\"{a}hler manifold. Furthermore, we gave the noncommutative \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) as concrete examples. In addition, we verified that Theorem \ref{main_thm_N2} works well, since the noncommutative \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) coincide with the provious results by Karabegov \cite{Kara1} and Sako-Suzuki-Umetsu \cite{SSU1,SSU2}, respectively.
%\bigskip
%\\
%\ On the other hand, the concrete example of two dimensional locally symmetric K\"{a}hler manifold is quadratic surface 
%\(
%  Q^{2}
%  \left(\mathbb{C}\right)
%  =
%  SO(N)/
%  \left(
%    SO(N-2)
%    \times
%    U(1)
%  \right)
%\)
%. 
%However, the deformation quantization for \(Q^{2}\left(\mathbb{C}\right)\) have not yet been constructed. 
%It is known that the K\"{a}hler potential of \(Q^{2}\left(\mathbb{C}\right)\) is given by
%\begin{align}
%  \Phi_{Q^{2}\left(\mathbb{C}\right)}
%  =
%  \log
%  \left(
%    1
%    +
%    \sum_{k=1}^{2}
%    |z^{k}|^{2}
%    +
%    \frac{1}{4}
%    \sum_{k,l=1}^{2}
%    (
%      \overline{z}^{k}
%    )^{2}
%    (
%      z^{l}
%    )^{2}
%  \right).
%\label{kahler_p_Q2}
%\end{align}
%\noindent
%See \cite{HN1} for more detail. Since K\"{a}hler metric and curvature are expressed by using a K\"{a}hler potential, it may be able to explicitly construct the noncommutative ones as the concrete examples by using Theorem \ref{main_thm_N2}. In particular, it is known that supersymmetric nonlinear sigma models whose target spaces are K\"{a}hler manifolds studied by Higashijima-Nitta \cite{HN1,HN2,HN3}, Higashijima-Kimura-Nitta \cite{HKN} and Kondo-Takahashi \cite{KT}. They include the models on \(\mathbb{C}P^{N}\) and \(Q^{2}\left(\mathbb{C}\right)\) as the target spaces. So we may be able to construct the supersymmetric nonlinear sigma models on noncommutative \(\mathbb{C}P^{2}\) and \(Q^{2}\) by using Theorem \ref{main_thm_N2}.
%\bigskip
%\\
%\ We can expect to develop the physics on noncommutative locally symmetric K\"{a}hler manifolds from our result. For example, the constructions of quantum field theories and gauge theories on noncommutative ones are expected. In contrast to the strict deformation quantization case, the formal deformation quantization case is difficult to make sense of the physics. However, it is possible to construct Fock representations in the formal deformation quantization case. In fact, (twisted) Fock representations can be constructed by using a formal star product as discussed in Section \ref{DQ_Review} (See \cite{SSU1,SSU2,SU1,SU2,SU3} for more detailed discussions). Recalling that quantium field theories can be stated by using Fock representations, we can expect to propose the quantum field theory on noncommutative K\"{a}hler manifold. In addition, it is expected to clarify the relationship between fuzzy manifolds and deformation quantization, since Fock representations can be interpreted by using a matrix represenatation. Furthermore, we can concretely construct examples of gauge theories by using (twisted) Fock representations. In fact, they have already studied by Maeda-Sako-Suzuki-Umetsu \cite{MSSU} on noncommutative homogeneous K\"{a}hler manifolds and Sako-Suzuki-Umetsu \cite{SSU3} for noncommutative \(\mathbb{C}P^{N}\). If the noncommutative \(Q^{2}\left(\mathbb{C}\right)\) are given by Theorem \ref{main_thm_N2}, we may be able to propose gauge theories on noncommutative \(Q^{2}\left(\mathbb{C}\right)\). In particular, we expect to propose the supersymmetric nonlinear sigma models on ``noncommutative" \(\mathbb{C}P^{N}\) and \(Q^{2}\left(\mathbb{C}\right)\), as the gauge theories given by \cite{MSSU,SSU3} on them.
\ In this paper, we obtained the explicit star products with separation of variables for two-dimensional locally symmetric K\"{a}hler manifolds by solving the recurrence relations in \cite{HS1,HS2}. By using Theorem \ref{main_thm_N2}, we can construct a deformation quantization with separation of variables for any complex two-dimensional locally symmetric K\"{a}hler manifold. Furthermore, we gave the noncommutative \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) as concrete examples. We verified these noncommutative \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) coincide with the 
%provious 
previous results by Karabegov \cite{Kara1} and Sako-Suzuki-Umetsu \cite{SSU1,SSU2}, respectively.
\bigskip
\\
%\ What other examples of noncommutative deformations have not yet been proved to which the Theorem \ref{main_thm_N2} can be applied?
\ In this section, we discuss what can be done in the future using the theorems obtained in this paper. We give an example of a two-dimensional 
%symmmetric 
symmetric K\"{a}hler manifold to which Theorem \ref{main_thm_N2} is applicable and for which deformation quantization has not yet been obtained. The concrete example of two dimensional locally symmetric K\"{a}hler manifold is a quadratic surface 
\(
  Q^{2}
  \left(\mathbb{C}\right)
  =
  SO(4)/
  \left(
    SO(2)
    \times
    U(1)
  \right)
\). 
However, the deformation quantization for \(Q^{2}\left(\mathbb{C}\right)\) have not yet been constructed. 
It is known that the K\"{a}hler potential of \(Q^{2}\left(\mathbb{C}\right)\) is given by
\begin{align}
  \Phi_{Q^{2}\left(\mathbb{C}\right)}
  =
  \log
  \left(
    1
    +
    \sum_{k=1}^{2}
    |z^{k}|^{2}
    +
    \frac{1}{4}
    \sum_{k,l=1}^{2}
    (
      \overline{z}^{k}
    )^{2}
    (
      z^{l}
    )^{2}
  \right).
\label{kahler_p_Q2}
\end{align}
\noindent
See \cite{Ell,HN1,Nitta} for more detail. 
%Since K\"{a}hler metric and curvature are expressed by using a K\"{a}hler potential, it is able to explicitly construct the noncommutative ones as the concrete examples by using Theorem \ref{main_thm_N2}. In particular, it is known that supersymmetric nonlinear sigma models whose target spaces are K\"{a}hler manifolds studied by Higashijima-Nitta \cite{HN1,HN2,HN3}, Higashijima-Kimura-Nitta \cite{HKN} and Kondo-Takahashi \cite{KT}. They include the models on \(\mathbb{C}P^{N}\) and \(Q^{2}\left(\mathbb{C}\right)\) as the target spaces.
Since K\"{a}hler metric and curvature are expressed by using a K\"{a}hler potential, it is %able 
possible to explicitly construct the noncommutative 
%ones 
\(Q^{2}\left(\mathbb{C}\right)\) by using Theorem \ref{main_thm_N2}, explicitly. Supersymmetric nonlinear sigma models whose target spaces are K\"{a}hler manifolds are studied by Higashijima-Nitta \cite{HN1,HN2,HN3}, Higashijima-Kimura-Nitta \cite{HKN} and Kondo-Takahashi \cite{KT}. Some models of them are defined on \(\mathbb{C}P^{N}\) and \(Q^{2}\left(\mathbb{C}\right)\) as the target spaces. 
%So we may be able to construct the supersymmetric nonlinear sigma models on noncommutative \(\mathbb{C}P^{2}\) and \(Q^{2}\).
%So we may be able to construct the supersymmetric nonlinear sigma models on noncommutative \(\mathbb{C}P^{2}\) and \(Q^{2}\left(\mathbb{C}\right)\).
It should be possible to extend the nonlinear sigma models to ones on noncommutative \(\mathbb{C}P^{N}\) and \(Q^{2}\left(\mathbb{C}\right)\), naively.
\bigskip
\\
\ We can expect to develop the physics on noncommutative locally symmetric K\"{a}hler manifolds from our result. For example, the constructions of some field theories and gauge theories on noncommutative ones are expected. 
%In contrast to the strict deformation quantization case, the formal deformation quantization case is difficult to make interpretation as the physics. However, it is possible to construct Fock representations from the formal deformation quantization. In fact, (twisted) Fock representations can be constructed by using a deformation quantization with separation of variables product as discussed in Section \ref{DQ_Review} (See \cite{SSU1,SSU2,SU1,SU2,SU3} for more detailed discussions). 
%Some one 
Someone might think that in contrast to %the 
strict deformation quantization, %the 
formal deformation quantization is difficult to 
%make interpretation as 
interpret some physics. However, it is possible to construct Fock representations from the formal deformation quantization in our cases. In fact, (twisted) Fock representations can be constructed by using a deformation quantization with separation of variables as discussed in Section \ref{DQ_Review}. See \cite{SSU1,SSU2,SU1,SU2,SU3} for more detailed discussions. Recalling that field theories can be 
%discribed 
described by using Fock representations, we can expect to propose the field 
%theoies 
theories on noncommutative K\"{a}hler manifold. 
%In addition, it is expected to clarify the relationship between fuzzy manifolds and deformation quantization, since Fock representations can be interpreted by using a matrix represenatation.
In addition, it is expected to clarify the relationship between fuzzy manifolds and deformation quantization, since Fock representations can be interpreted by using a matrix representation. 
%Furthermore, we can concretely construct examples of gauge theories by using (twisted) Fock representations. In fact, they have already studied by Maeda-Sako-Suzuki-Umetsu \cite{MSSU} and Sako-Suzuki-Umetsu \cite{SSU3} on noncommutative homogeneous K\"{a}hler manifolds. For example, if the noncommutative \(Q^{2}\left(\mathbb{C}\right)\) are given by Theorem \ref{main_thm_N2}, we can propose gauge theories on noncommutative \(Q^{2}\left(\mathbb{C}\right)\).
Furthermore, we can concretely construct gauge theories by using (twisted) Fock representations. 
%In fact, they 
They have been already studied by Maeda-Sako-Suzuki-Umetsu \cite{MSSU} and Sako-Suzuki-Umetsu \cite{SSU3} on noncommutative homogeneous K\"{a}hler manifolds. See \cite{Sako} for the review 
%about 
of these facts. For example, if the noncommutative \(Q^{2}\left(\mathbb{C}\right)\) are given by Theorem \ref{main_thm_N2}, we can propose gauge theories on noncommutative \(Q^{2}\left(\mathbb{C}\right)\).
\bigskip
\\
\ As described above, it is expected that various physical theories on complex two-dimensional noncommutative locally symmetric K\"{a}hler manifold can be obtained by using the Theorem \ref{main_thm_N2}. They are left for future 
%works.
work.


==> NCK2_ex.tex <==
\section{Examples}
\label{conc_ex}
\ In this section, we describe the deformation quantization with separation of variables for \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) as concrete examples realized from Theorem \ref{main_thm_N2}. The deformation quantizations were already given by the other methods as we will see in the next subsection. To compare our results with them, we can check if Theorem \ref{main_thm_N2} works well. Moreover, we show that %their %there 
the concrete examples satisfy the identities in Theorem \ref{minus_thm_N2}.
\input{EX/NCK2_Previous.tex}
\input{EX/NCK2_C2.tex}
%\input{EX/NCK2_CP2_journal.tex}
\input{EX/NCK2_CP2_Varna.tex}


==> NCK2_intro.tex <==
\section{Introduction}
\label{INTRO}
%the history of deformation quantization
\ Deformation quantization is one of the 
%a 
quantization method based on a deformation for a Poisson algebra and is known as a method of constructing noncommutative differentiable manifolds. There are two types of this, ``formal deformation quantization" proposed by Bayen et al. \cite{BFFLS}, and ``strict deformation quantization", based on \(C^{\star}\)-algebra proposed by Rieffel \cite{Rief1}. In this paper, we study %a 
formal deformation quantization, and in the following, ``deformation quantization" is used in the sense of ``formal deformation quantization".

\begin{definition}
  Let 
  \(M\)
  be a Poisson manifold, 
  \(
    C^{\infty}\left(M\right)
  \)
  be a set of \(C^{\infty}\) functions on \(M\),
  \(
  \left\{
    \cdot,
    \cdot
  \right\}
  :
  C^{\infty}\left(M\right)
  \times
  C^{\infty}\left(M\right)
  \to
  C^{\infty}\left(M\right)
  \)
  be a Poisson bracket, and 
  \(
    C^{\infty}
    \left(M\right)
    \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    :=
    \left\{
      f
      \middle|
      f
      =
      \sum_{k}
      f_{k}
      \hbar^{k},
      \
      f_{k}
      \in
      C^{\infty}\left(M\right)
    \right\}
  \)
  be the ring of formal power series over
  \(
    C^{\infty}\left(M\right),
  \)
   where \(\hbar\) is a formal parameter. Let a product \(\ast\) on
  \(
    C^{\infty}
    \left(M\right)
    \left[\!
      \left[
        \hbar
      \right]\!
    \right],
  \)
   called the star product, be a product denoted by
  \begin{align*}
    f
    \ast
    g
    =
    \sum_{k=0}^{\infty}
    C_{k}\left(f,g\right)
    \hbar^{k}
  \end{align*}
  satisfying the following conditions:
  \begin{enumerate}
    \item
    \(\ast\)
    is associative, i.e. for any 
    \(
      f,g,h
      \in
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    \)
    , 
    \(
      f
      \ast
      \left(
        g
        \ast
        h
      \right)
      =
      \left(
        f
        \ast
        g
      \right)
      \ast
      h.
    \)
    \item
    Each 
    \(
      C_{k}
      \left(
        \cdot,
        \cdot
      \right)
      :
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
      \times
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
      \to
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    \)
    is a bi-differential operator, i.e. for any 
    \(
      f,g
      \in
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right],
    \)
    \(
      C_{k}
      \left(
        f,
        g
      \right)
    \) 
    can be written as 
    \begin{align*}
      C_{k}
      \left(
        f,
        g
      \right)
      =
      \sum_{I,J}
      a_{I,J}
      \partial^{I}
      f
      \partial^{J}
      g,
    \end{align*}
    where \(I,J\) are multi-indices.
    \item
    For any
    \(
      f,g
      \in
      C^{\infty}
      \left(M\right)
    \)
    ,
    \begin{align*}
      C_{0}
      \left(
        f,
        g
      \right)
      &=
      fg,
      \\
      C_{1}
      \left(
        f,
        g
      \right)
      -
      C_{1}
      \left(
        g,
        f
      \right)
      &=
      \left\{f,g\right\}.
    \end{align*}
    \item
    For any
    \(
      f
      \in
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    \)
    ,
    \(
      f
      \ast
      1
      =
      1
      \ast
      f
      =
      f.
    \)
  \end{enumerate}
  The pair 
  \(
    \left(
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right],
      \ast
    \right)
  \) 
  is called a deformation quantization for \(M.\)
  \label{dq_def}
\end{definition}
\noindent
For a more detailed review of deformation quantization, see e.g. \cite{GUT}. The construction method of deformation quantization for symplectic manifolds has been known by de Wilde-Lecomte \cite{DL}, Omori-Maeda-Yoshioka \cite{OMY1} and Fedosov \cite{Fedo}. %,
After these works, a method for Poisson manifolds was proposed by Kontsevich \cite{Kont1}.
%Karabegov
 For any K\"{a}hler manifold, Karabegov studied a construction method of deformation quantization with separation of variables \cite{Kara1,Kara2}.

\begin{definition}
  Let \(M\) be a K\"{a}hler manifold. A star product \(\ast\) on \(M\) is the separation of variables if the following two conditions are satisfied for any open set \(U\) of \(M\) and 
  \(
    f
    \in
    C^{\infty}
    \left(
      U
    \right)
  \) 
  :
  \begin{enumerate}
    \item
    For a holomorphic function
    \(
      a
    \) 
    on \(U,\) 
    \(
      a
      \ast
      f
      =
      af.
    \)
    \item
    For an anti-holomorphic function 
    \(
      b
    \) 
    on \(U,\) 
    \(
      f
      \ast
      b
      =
      fb.
    \)
  \end{enumerate}
  \label{sep_of_bar_starprd}
\end{definition}

\noindent
\ Furthermore, inspired by Karabegov's idea, a construction method for a locally symmetric K\"{a}hler manifold, i.e. a K\"{a}hler manifold such that 
\(
  \nabla_{\partial_{E}}
  R_{ABC}^{\quad \ \ \, D}
  =
  0
\) 
for 
\(
  A,B,C,D,E
  \in
  \left\{
    1,
    \cdots,
    N,
    \overline{1},
    \cdots,
    \overline{N}
  \right\},
\) 
was later proposed by Sako-Suzuki-Umetsu \cite{SSU1,SSU2} and Hara-Sako \cite{HS1,HS2}. Some notations in this paper are explained in more detail in Appendix \ref{app_kaehler}.
\bigskip
\\
\ In this paper, we propose an explicit formula that gives a deformation quantization with separation of variables for a complex two-dimensional locally symmetric K\"{a}hler manifold. This main result that is given in Theorem \ref{main_thm_N2} in Section \ref{NEW_RESULT} gives the explicit star product which is expanded in differential operators whose coefficients consist of covariantly constant. Each coefficient is explicitly determined by some matrix multiplications, and it contains the Riemann curvature tensor. This theorem is shown by solving the recurrence relations given by Hara-Sako \cite{HS1,HS2}. To explain our main result, we must introduce 
%a number of 
several definitions. So we shall not state our main theorem concretely, here.
\bigskip
\\
\
This paper is organized mainly into four Sections and three Appendices. In Section \ref{DQ_Review}, %we review a construction method of a deformation quantization with separation of variables for locally symmetric K\"{a}hler manifolds, which is a previous work by Hara-Sako\cite{HS1,HS2}.
we review the previous works by Karabegov \cite{Kara1,Kara2} and Hara-Sako \cite{HS1,HS2}, as the %historical 
background %with respect to 
concerning a deformation quantization with separation of variables for K\"{a}hler manifolds.
In Section \ref{NEW_RESULT}, we show our main results 
%that
which are the explicit formula to give the star product and the identities. In Section \ref{conc_ex}, we construct concrete examples for \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\) and they reproduce the previous results. 
In Section \ref{DQ_Discussion}, we state future works related to our main results from both mathematical and physical perspectives. 
In each Appendices \ref{app_kaehler}--\ref{prf_Tn_dagger}, we describe the properties and detailed calculations used in this paper. In Appendix \ref{app_kaehler}, we summarize some properties of K\"{a}hler manifolds used in this paper. In Appendix \ref{app_minus_n2}, we calculate in detail the identity \eqref{minus_thm_eq_ens} in Subsection \ref{NR_minus} for the 2nd order. In Appendix \ref{prf_Tn_dagger}, 
the Hermiteness of the coefficients of a star product is shown.
%%注意：section2に加筆したので，その部分についても加筆する必要あり．


==> NCK2_ref.tex <==
\begin{thebibliography}{99}
    \bibitem{ABIY} G.~Alexanian, A.~P.~Balachandran, G.~Immirzi and B.~Ydri, ``Fuzzy \(\mathbb{C}P^{2}\)", J.~Geom.~Phys.~\textbf{42}(1-2), (2002), 28--53.
    \bibitem{APS} G.~Alexanian, A.~Pinzul and A.~Stern, ``Generalized coherent state approach to star products and applications to the fuzzy sphere", Nucl.~Phys.~B~\textbf{600}(3), (2001), 531--547.
    \bibitem{BDMLO} A.~P.~Balachandran, B.~P.~Dolan, J.~H.~Lee, X.~Martin and D.~O'Connor, ``Fuzzy complex projective spaces and their star products", 
J.~Geom.~Phys.~\textbf{43}, (2002), 184--204.
    \bibitem{BFFLS} F.~Bayen, M.~Flato, C.~Fronsdal, A.~Lichnerowicz and D.~Sternheimer, ``Deformation theory and quantization. I. Deformations of symplectic structures", Ann.~Phys.~\textbf{111}, (1978), 61--111.
    \bibitem{Bere1} F.~A.~Berezin, ``Quantization", MATH~USSR--Izv, \textbf{8}(5), (1974), 1109-–1165.
    \bibitem{Bere2} F.~A.~Berezin, ``General concept of quantization", Comm.~Math.~Phys.~\textbf{40}(2), (1975), 153--174.
	\bibitem{BBEW} M.~Bordemann, M.~Brischle, C.~Emmrich and S.~Waldmann, ``Phase Space Reduction for Star-Products: An Explicit Construction for \(\mathbb{C}P^{n}\)", Lett.~Math.~Phys.~\textbf{36}, (1995), 357--371.
    \bibitem{BMS} M.~Bordemann, E.~Meinrenken and M.~Schlichenmaier, ``Toeplitz quantization of K\"{a}hler manifolds and \(gl(N), N\to\infty\) limits", Comm. Math. Phys.~\textbf{165}(2), (1994), 281--296.
    \bibitem{BW1} M.~Bordemann and S.~Waldmann, ``A Fedosov star product of the Wick type for K\"{a}hler manifolds", Lett.~Math.~Phys.~\textbf{41}(3), (1997), 243--253.
    \bibitem{BW2} M.~Bordemann and S.~Waldmann, ``Formal GNS construction and states in deformation quantization", Comm.~Math.~Phys.~\textbf{195}(3), (1998), 549--583.
    \bibitem{CGR1} M.~Cahen, S.~Gutt, and J.~Rawnsley, ``Quantization of K\"{a}hler manifolds. I", J.~Geom.~Phys.~\textbf{7}(1), (1991), 45--62.
    \bibitem{CGR2} M.~Cahen, S.~Gutt, and J.~Rawnsley, ``Quantization of K\"{a}hler manifolds. II", Trans.~Amer.~Math.~Soc.~\textbf{337}, (1993), 73--98.
    \bibitem{CGR3} M.~Cahen, S.~Gutt, and J.~Rawnsley, ``Quantization of K\"{a}hler manifolds. III", Lett.~Math.~Phys.~\textbf{30}, (1994), 291--305.
    \bibitem{CGR4} M.~Cahen, S.~Gutt, and J.~Rawnsley, ``Quantization of K\"{a}hler manifolds. IV", Lett.~Math.~Phys.~\textbf{34}, (1995), 159--168.
    \bibitem{CSW} U.~Carow-Watamura, H.~Steinacker and S.~Watamura, ``Monopole bundles over fuzzy complex projective spaces", J.~Geom.~Phys.~\textbf{54}(4), (2005), 373--399.
    \bibitem{DL} M.~de Wilde and P.~B.~A.~Lecomte, ``Existence of star-products and of formal deformations of the Poisson Lie algebra of arbitrary symplectic manifolds", Lett.~Math.~Phys.~\textbf{7}, (1983), 487--496.
    \bibitem{Dirac} P.~A.~M.~Dirac, ``The fundamental equations of quantum mechanics", Proc.~R.~Soc.~Lond.~A~\textbf{109}(752), (1925), 642--653.
    \bibitem{Ell} U.~Ellwanger, ``Supersymmetric \(\sigma\)-models in four dimensions as quantum theories", Nucl.~Phys.~B, \textbf{281}(3-4), (1987), 489--508.
    \bibitem{Fedo} B.~V.~Fedosov, ``A simple geometrical construction of deformation quantization", J.~Differ.~Geom.~\textbf{40(2)}, (1994), 213--238.
    \bibitem{GS} H.~Grosse and A.~Strohmaier, ``Towards a nonperturbative covariant regularization in 4D quantum field theory", Lett.~Math.~Phys.~\textbf{48}, (1999), 163--179.
    \bibitem{GUT} S.~Gutt, ``Deformation quantization of Poisson manifolds", Geometry and Topology Monographs~\textbf{17}, (2011), 171--220.
    \bibitem{HS1} K.~Hara and A.~Sako, ``Noncommutative Deformations of Locally Symmetric K\"{a}hler manifolds", J.~Geom.~Phys.~\textbf{114}, (2017), 554--569.
    \bibitem{HS2} K.~Hara and A.~Sako, ``Quantization of Locally Symmetric K\"ahler manifolds", Geometry Integrability and Quantization~\textbf{19}, (2018), 122--131.
    %\bibitem{HSY} K.~Hara, A.~Sako, and H.~S.~Yang, ``Hermitian-Einstein metrics from noncommutative \(U\left(1\right)\) instantons", J.~Math.~Phys.~\textbf{60}(9), 092501 (2019), 1--34.
    \bibitem{HNT} K.~Hayasaka, R.~Nakayama and Y.~Takaya, ``A New Noncommutative Product on the Fuzzy Two-Sphere Corresponding to the Unitary Representation of \(SU(2)\) and the Seiberg-Witten Map", Phys.~Lett.~B~\textbf{553(1--2)}, (2003), 109--118.
    \bibitem{HKN} K.~Higashijima, T.~Kimura and M.~Nitta, ``Gauge theoretical construction of non-compact Calabi–Yau manifolds", Ann.~Phys.~(N.Y.)~\textbf{296}(2), (2002), 347--370.
    \bibitem{HN1} K.~Higashijima and M.~Nitta, ``Supersymmetric nonlinear sigma models as gauge theories", Prog.~Theor.~Phys.~\textbf{103}(3), (2000), 635--663.
    \bibitem{HN2} K.~Higashijima and M.~Nitta, ``Quantum equivalence of auxiliary field methods in supersymmetric theories", Prog.~Theor.~Phys.~\textbf{103}(4), (2000), 833-846.
    \bibitem{HN3} K.~Higashijima and M.~Nitta, ``Supersymmetric nonlinear sigma models", Quantum chromodynamics and color confinement. Proceedings, International Symposium, Confinement 2000, Osaka, March 7--10, (2000), 279--286.
    \bibitem{Hop} J.~Hoppe, ``Quantum theory of a massless relativistic surface and a two-dimensional bound state problem", Soryushiron~Kenkyu~Electronics~\textbf{80}(3), (1989), 145--202.
    \bibitem{Kara1} A.~V.~Karabegov, ``On the Deformation Quantization, on a K\"{a}hler Manifold, Associated with a Berezin Quantization", Funct.~Anal.~its~Appl.~\textbf{30(2)}, (1996), 142--144.
    \bibitem{Kara2} A.~V.~Karabegov, ``Deformation quantization with separation of variables on a K\"{a}hler manifold", Comm.~Math.~Phys.~\textbf{180}, (1996), 745--755.
    \bibitem{KS1} A.~V.~Karabegov and M.~Schlichenmaier, ``Identification of Berezin-Toeplitz deformation quantization", Crelle's Journal~\textbf{2001}, (2000), 49--76.
    \bibitem{KN} S.~Kobayashi and K.~Nomizu, ``Foundations of Differential Geometry II", New York:~John~Wiley\&Sons, (1969), 470 pp.
    \bibitem{KT} A.~Kondo and T.~Takahashi, ``Supersymmetric nonlinear sigma models as anomalous gauge theories", Phys.~Rev.~D~\textbf{102}(2), 025014, (2020), 1--13.
    %\bibitem{Koda} 小平邦彦，『複素多様体論』，岩波書店，(1992), 486 pp.
    %\bibitem{Konno} 今野宏，『微分幾何学』，東京大学出版会，(2013), 277 pp.
    \bibitem{Kont1} M.~Kontsevich, ``Deformation quantization of Poisson manifolds", Lett.~Math.~Phys.~\textbf{66}, (2003), 157--216.
    %\bibitem{Kont2} M.Kontsevich, ``Deformation quantization of algebraic varieties", Lett.Math.Phys.56, (2001), 271--294.
    %\bibitem{MK1} 前田吉昭，梶浦宏成，『弦理論と変形量子化』，数学55巻3号，日本数学会，(2003), 245--265.
    %\bibitem{MK2} 前田吉昭，梶浦宏成，『変形量子化入門』，東京大学大学院数理科学研究科セミナー刊行会，(2002), 178 pp.
    \bibitem{Kos} B.~Kostant, ``Quantization and unitary representations", Berlin: Springer, Lectures in Modern Analysis and Applications III. Lecture Notes in Mathematics \textbf{170}, (1970), 87--208pp.
    \bibitem{Mad1} J.~Madore, ``The Fuzzy sphere", Class~Quantum~Gravity~\textbf{9}, (1992), 69--87.
    \bibitem{Mad2} J.~Madore, ``An Introduction to Noncommutative Differential Geometry and its Physical Applications", (2nd ed., London Mathematical Society Lecture Note Series). Cambridge:~Cambridge~University~Press, (1999), 371pp.
    %\bibitem{MS1} Y.~Maeda and A.~Sako, ``Noncommutative deformation of instantons", J.~Geom.~Phys.~\textbf{58}(12), (2008), 1784--1791.
    %\bibitem{MS2} Y.~Maeda and A.~Sako, ``Noncommutative deformation of spinor zero mode and Atiyah-Drinfeld-Hitchin-Manin construction", J.~Math.~Phys.~\textbf{53}(2), 022303, (2012), 1--34.
    \bibitem{MSSU} Y.~Maeda, A.~Sako, T.~Suzuki and H.~Umetsu, ``Gauge theories in noncommutative homogeneous K\"{a}hler manifolds", J.~Math.~Phys.~\textbf{55}(9), 092301, (2014), 1--27.
    \bibitem{Mor1} C.~Moreno, ``\(\ast\)-products on some K\"{a}hler manifolds", Lett.~Math.~Phys.~\textbf{11}, (1986),361--372.
    \bibitem{Mor2} C.~Moreno, ``Invariant star products and representations of compact semisimple Lie groups", Lett.~Math.~Phys.~\textbf{12}, (1986), 217--229.
    \bibitem{Moya} J.~E.~Moyal, ``Quantum Mechanics as a Statistical Theory", Proceedings of the Cambridge Philosophical Society~\textbf{45(1)}, (1949), 99--124.
    %\bibitem{MS1} 前田吉昭，佐古彰史，『幾何学の量子化』，SGCライブラリ95, サイエンス社，176 pp.
    %\bibitem{MS2} 前田吉昭，佐古彰史，『非可換微分幾何学の基礎』，共立出版株式会社，(2020), 282 pp.
    %\bibitem{Naka} M.Nakahara, "Geometry, Topology and Physics", Taylor \& Francis, (2003), 596 pp.
    %\bibitem{NM} 夏目利一，森吉仁志，『作用素環と幾何学』，数学メモアール2巻，日本数学会，(2001), 228 pp.
    %\bibitem{NM_trans} T.Natsume and H.Moriyoshi, ``Operator Algebras and Geometry", Translations of Mathematical Monographs Vol.237, American Mathematical Society, (2008), 155 pp.
    %\bibitem{NS} N.~Nekrasov and A.~Schwarz, ``Instantons on noncommutative \(\mathbb{R}^{4}\), and \((2,0)\) superconformal six dimensional theory", Comm.~Math.~Phys.~\textbf{198}(3), (1998), 689--703.
    \bibitem{Nitta} M.~Nitta, ``K\"{a}hler Potential for Global Symmetry Breaking in Supersymmetric Theories", hep-th/9903174, (1999).
    \bibitem{OMY1} H.~Omori, Y.~Maeda and A.~Yoshioka, ``Weyl Manifolds and Deformation Quantization", Adv.~Math.~\textbf{85}, (1991), 224--255.
    \bibitem{OMY2} H.~Omori, Y.~Maeda and A.~Yoshioka, ``Non-Commutative Complex Projective Space", Adv.~Math.~\textbf{22}, (1993), 133--152.
    \bibitem{OMMY} H.~Omori, Y.~Maeda, N.~Miyazaki and A.~Yoshioka, ``Poincar\'{e}--Cartan Class and Deformation Quantization of K\"{a}hler Manifolds", Comm.~Math.~Phys.~textbf{194}, (1998), 207--230.
    %\bibitem{PS} L.E.Pursell and M.E.Shanks, ``The Lie algebra of a smooth manifold", Proc. Amer. Math. Soc. \textbf{5}, (1954), 468--472.
    \bibitem{OS_Varna} T.~Okuda and A.~Sako, ``Deformation quantization with separation of variables for complex two-dimensional locally symmetric K\"{a}hler manifold", to appear in the proceedings of the conference ``Geometry Integrability and Quantization~\textbf{25}".
    \bibitem{Pere} A.~M.~Perelomov, ``Generalized coherent states and their applications", Berlin: Springer, (1986), 320pp.
    \bibitem{Rawn} J.~H.~Rawnsley, ``Coherent states and K\"{a}hler manifolds", Q.~J.~Math.~\textbf{28}(4), (1977), 403--415.
    \bibitem{Rief1} M.~Rieffel, ``Deformation quantization of Heisenberg manifolds", Comm.~Math.~Phys.~\textbf{122}(4), (1989), 531--562.
    \bibitem{Rief2} M.~Rieffel, ``Deformation quantization for actions of \(\mathbb{R}^{d}\)", Mem.~Amer.~Math.~Soc.~\textbf{106}(506), 1993, 93pp.
    \bibitem{Rief3} M.~Rieffel, ``Quantization and C*-algebras", Contemporary Mathematics~\textbf{167}, (1994), 67--97.
    \bibitem{Sako} A.~Sako, ``A Recipe To Construct A Gauge Theory On A Noncommutative K\"{a}hler Manifold", Noncommutative Geometry and Physics \textbf{4}, (2017), 361--404.
    \bibitem{SSU1} A.~Sako, T.~Suzuki and H.~Umetsu, ``Explicit Formulae for Noncommutative Deformations of \(\mathbb{C}P^{N}\) and \(\mathbb{C}H^{N}\)", J.~Math.~Phys.~\textbf{53}(7), 073502, (2012), 1--16.
    \bibitem{SSU2} A.~Sako, T.~Suzuki and H.~Umetsu, ``Noncommutative \(\mathbb{C}P^{N}\) and \(\mathbb{C}H^{N}\) and their physics", J.~Phys.~Conf.~Ser.~\textbf{442}, 012052, (2013), 1--10.
    \bibitem{SSU3} A.~Sako, T.~Suzuki and H.~Umetsu, ``Gauge theories on noncommutative \(\mathbb{C}P^{N}\) and Bogomol'nyi-Prasad-Sommerfield-like equations", J.~Math.~Phys.~\textbf{56}, 113506, (2015), 1--22.
    \bibitem{SU1} A.~Sako and H.~Umetsu, ``Twisted Fock Representations of Noncommutative K\"{a}hler Manifolds", J.~Math.~Phys.~\textbf{57}(9), 093501, (2016), 1--30.
    \bibitem{SU2} A.~Sako and H.~Umetsu, ``Deformation Quantization of K\"{a}hler Manifolds and Their Twisted Fock Representation", Geometry, Integrability and Quantization~\textbf{18}, (2016), 225--240.
    \bibitem{SU3} A.~Sako and H.~Umetsu, ``Fock Representations and Deformation Quantization of K\"ahler Manifolds", Advances in Applied Clifford Algebras~\textbf{27}, (2017), 2769--2794.
    \bibitem{Schli1} M.~Schlichenmaier, ``Deformation quantization of compact K\"{a}hler manifolds via Berezin-Toeplitz operators", in Group 21: physical applications and mathematical aspects of geometry, groups and algebras; proceeding of the XXI International Colloquium on Group Theoretical Methods in Physics, July 15--20, 1996, Goslar, (1996), 396--400.
    \bibitem{Schli2} M.~Schlichenmaier, ``Berezin-Toeplitz quantization of compact K\"{a}hler manifolds", in Quantization, coherent states and Poisson structures: proceedings of the XIV Workshop on Geometric Methods in Physics, Bia\l
    owie\.{z}a, July 9--15, 1995, (1998), 101--115.
    \bibitem{Schli3} M.~Schlichenmaier, ``Berezin-Toeplitz quantization and Berezin symbols for arbitrary compact K\"{a}hler manifolds", in Coherent states, quantization and gravity : proceedings of the XVII Workshop on Geometric Methods in Physics, Bia\l
    owie\.{z}a, July 3--9, 1998, (2001), 45--46.
    \bibitem{Schli4} M.~Schlichenmaier, ``Deformation quantization of compact K\"{a}hler manifolds by Berezin-Toeplitz quantization", In Conf\'{e}rence Mosh\'{e} Flato 1999. Springer, Dordrecht, (2000), 289--306.
    \bibitem{Schli5} M.~Schlichenmaier, ``Berezin-Toeplitz quantization and Berezin transform", In Long time behaviour of classical and quantum systems, (2001), 271--287.
    \bibitem{Schli6} M.~Schlichenmaier, ``Berezin-Toeplitz quantization for compact K\"{a}hler manifolds. A review of results", Adv.~Math.~Phys.~\textbf{2010}, (2010), 643--680.
    \bibitem{Schli7} M.~Schlichenmaier, ``Berezin–Toeplitz quantization and star products for compact K\"{a}hler manifolds", Contemp.~Math.~\textbf{583}, (2012), 257--294.
    \bibitem{Sou} J.~Souriau, ``Structure des syst\'{e}mes dynamiques", Paris: Dunod, (1970), 414pp.
    %\bibitem{SV} M.~Spradlin and A.~Volovich, ``Noncommutative solitons on K\"{a}hler manifolds", J.~High~Energy~Phys.~\textbf{2002}(03), (2002), 011--011.
    \bibitem{Voro} A.Voros, ``Wentzel-Kramers-Brillouin method in the Bargmann representation", Phys.~Rev.~A~\textbf{40} (1989), 6814--6825.
    %\bibitem{Wein} A.~Weinstein, ``Deformation quantization", Ast\'{e}risque~\textbf{227}, 389--409.
\end{thebibliography}
%%追加文献引用済．


==> NCK2_rev.tex <==
\section{Review of Noncommutative K\"{a}hler manifolds}
\label{DQ_Review}

\ %The Quantization of K\"{a}hler manifolds was studied by Berezin \cite{Bere1,Bere2}, Karabegov \cite{Kara1,Kara2}, Sako-Suzuki-Umetsu \cite{SSU1,SSU2,SSU3} and Hara-Sako \cite{HS1,HS2}. 
The Quantization of K\"{a}hler manifolds was studied by Berezin \cite{Bere1,Bere2}, Moreno \cite{Mor1,Mor2}, Cahen-Gutt-Rawnsley \cite{CGR1,CGR2,CGR3,CGR4}, Karabegov \cite{Kara1,Kara2}, Omori-Maeda-Miyazaki-Yoshioka \cite{OMMY}, Schlichenmaier \cite{Schli1,Schli2,Schli3,Schli4,Schli5,Schli6,Schli7}, Karabegov-Schlichenmaier \cite{KS1}, Sako-Suzuki-Umetsu \cite{SSU1,SSU2} and Hara-Sako \cite{HS1,HS2}. In particular, Karabegov's method was proposed as a way to give noncommutative K\"{a}hler manifolds via a deformation quantization with separation of variables. After that, Sako-Suzuki-Umetsu and Hara-Sako methods were proposed for a locally symmetric case, inspired by this method. In addition, Sako-Suzuki-Umetsu was mentioned the Fock representations of noncommutative \(\mathbb{C}P^{N}\) and \(\mathbb{C}H^{N}\). %Moreover, these previous results was generalized for any noncommutative K\"{a}hler manifolds by Sako-Umetsu \cite{SU1,SU2,SU3}. In Section \ref{NCK_History}, we state the methods by Karabegov as the %historical 
%background of noncomutative K\"{a}hler manifolds. And in Section \ref{DQ_LSK}, we review method by Hara-Sako since our result is obtained by the recurrence relations in this method.
Moreover, these previous results were generalized for any noncommutative K\"{a}hler manifolds by Sako-Umetsu \cite{SU1,SU2,SU3}. In Section \ref{NCK_History}, we review the methods by Karabegov as the background of this paper, and in Section \ref{DQ_LSK}, we review the method by Hara-Sako since our result is obtained from the recurrence relations in this method.

\input{REV/NCK2_History.tex}
\input{REV/NCK2_HS.tex}


==> NR/NCK2_minus.tex <==
\subsection{Another formula}
\label{NR_minus}
\ The formula \eqref{main_them_N2_Tinf} was obtained by summation with respect to the index \(i\) of the complex coordinate in the recurrence relation \eqref{rec_rel}. In Subsection \ref{NR_plus}, we made one recurrence relation by adding two recurrence relations and determined the solution using only that recurrence relation. On the other hand, we have not yet considered another recurrence relation. 
%, and it realized a deformation quantization with separation of variables for complex 2-dimensional locally symmetric K\"{a}hler manifold. On the other hand, if we change the treatment of the recurrence relation \eqref{rec_rel}, if we change the way we treat the recurrence relation \eqref{rec_rel}, then we obtain another recurrence relation. 
In this subsection, we consider another formula obtained by ``subtracting" for \(i=1,2\) rather than ``adding" two recurrence relations for \(i=1,2\) as we did in Subsection \ref{NR_plus}.

\begin{theorem}
  Let \(M\) be a locally symmetric K\"{a}hler manifold, \(U\) be an open set of \(M\),
  and 
  \(
    f,g
    \in
    C^{\infty}
    \left(U\right),
    \
    \ast
  \)
  be a star product with separation of variables on \(U\) such that
  \begin{align*}
    f
    \ast
    g
%    =&
%    \sum_{n=0}^{\infty}
%    \sum_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}
%    T_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}^{n}
%    \left(
%      D^{\overrightarrow{\alpha_{n}}}f
%    \right)
%    \left(
%      D^{\overrightarrow{\beta_{n}^{\ast}}}g
%    \right)
%    \\
    =&
    \sum_{n=0}^{\infty}
    \sum_{i,j=1}^{n+1}
    T_{ij}^{n}
    \left\{
    \left(
      D^{1}
    \right)^{n-i+1}
    \left(
      D^{2}
    \right)^{i-1}
    f
    \right\}
    \left\{
    \left(
      D^{\bar{1}}
    \right)^{n-j+1}
    \left(
      D^{\bar{2}}
    \right)^{j-1}
    g
    \right\}.
%    \
%    \left(
%      f,g
%      \in
%      C^{\infty}
%      \left(
%        U
%      \right)
%    \right).
  \end{align*}
  Then
  \begin{align}
    T_{n}
    Y_{n}
    =
    \hbar
    C'_{n}
    \label{minus_thm_N2_eq}
  \end{align}
  or equivalently
  \begin{align}
    Y_{n}^{\dagger}
    T_{n}
    =
    \hbar
    C_{n}^{'\dagger},
    \label{minus_thm_N2_eq_another}
  \end{align}
  where 
%  \(
%    T_{n}
%    :=
%    \left(
%      T^{n}_{ij}
%    \right)
%    \in
%    M_{n+1}
%    \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%  \right)
%  \) 
%  is given by \eqref{main_them_N2_Tinf}
  \begin{align*}
%    T_{n}
%    &
%    :=
%    \left(
%      T^{n}_{ij}
%    \right)
%    \in
%    M_{n+1}
%    \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%  \right),
%    \\
%    T^{n}_{ij}
%    &
%    :=
%    T_{
%      \left(
%        n-i+1,
%        i-1
%      \right),
%      \left(
%        n-j+1,
%        j-1
%      \right)
%    }^{n}
%    T_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}^{n},
%    \\
    C'_{n}
    &
    =
    \left(C_{ij}^{'n}\right)
    =
    \left(
      \sum_{k,l=1}^{2}
      \left(
        -1
      \right)^{\delta_{k2}}
      g_{\overline{k}l}
      T^{n-1}_{i-\delta_{2l},j-\delta_{2k}}
    \right)
    \in
    M_{n+1}
    \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\end{align*}
and 
\(
  Y_{n}
  \in
  M_{n+1}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\)
is a pentadiagonal matrix such that its 
%these 
components are given as follows :
\begin{align*}
    Y_{j-2,j}^{n}
    &=
    -
    \tbinom{n-j+3}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}},
    \\
    Y_{j-1,j}^{n}
    &=
    -
    \left(
      n-j+2
    \right)
    \left(
      j-2
    \right)
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}},
    \\
    Y_{j,j}^{n}
    &=
    n
    -
    2j
    +
    2
    +
    \tbinom{n-j+1}{2}
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    -
    \tbinom{j-1}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}},
    \\
    Y_{j+1,j}^{n}
    &=
    j
    \left(
      n-j
    \right)
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    Y_{j+2,j}^{n}
    &=
    \tbinom{j+1}{2}
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}},
    \\
    Y_{j,k}^{n}
    &=
    0
    \
    \left(
      \left|
        j-k
      \right|
      >
      2
    \right).
  \end{align*}
  \label{minus_thm_N2}
\end{theorem}

\begin{prf*}
This is shown in %by 
the same way as in Theorem \ref{main_thm_N2}.\(_{\blacksquare}\)
\end{prf*}
\noindent
Note that equation \eqref{minus_thm_N2_eq} is also expressed as an embedding version
\begin{align}
  T_{n}\left(\infty\right)
  Y_{n}\left(\infty\right)
  =
  \hbar
  C'_{n}\left(\infty\right)
  \label{minus_thm_N2_eq_rsz}
\end{align}
\noindent
or equivalently
\begin{align}
  Y_{n}^{\dagger}\left(\infty\right)
  T_{n}\left(\infty\right)
  =
  \hbar
  C_{n}^{'\dagger}\left(\infty\right),
  \label{minus_thm_N2_eq_another_rsz}
\end{align}
\noindent
where the embedding \(Y_{n}\left(\infty\right)\) for \(Y_{n}\) is as in the way of \eqref{emb_gene} in Subsection \ref{NR_plus}. 
%follows :
%\begin{align*}
%  Y_{n}
%  \mapsto
%  Y_{n}\left(\infty\right)
%  :=
%  \left(
%    \begin{array}{c|ccc}
%      Y_{n} & & \text{\huge{0}} & \\  \hline
%       &  & & \\
%      \text{\huge{0}} & & \text{\huge{0}} & \\
%       &  & &
%    \end{array}
%  \right).
%\end{align*}
%
%\noindent
Here we use 
\(
  T_{n}
  =
  T_{n}^{\dagger}.
\) 
Its derivation is in Appendix \ref{prf_Tn_dagger}.
\bigskip
\\
\
It is known from Karabegov's result that there is always a star product with separation of variables on a K\"{a}hler manifold \cite{Kara1,Kara2}. A star product with separation of variables on a locally symmetric K\"{a}hler manifold is %uniquely 
determined by \eqref{main_them_N2_Tinf} in Theorem \ref{main_thm_N2}. Therefore, \(T_{n}\left(\infty\right)\) given by \eqref{main_them_N2_Tinf} should satisfy \eqref{minus_thm_N2_eq_rsz}. To ensure that the result obtained by Theorem \ref{main_thm_N2} does not contradict Theorem \ref{minus_thm_N2}, we consider the following equation: 
\begin{align}
  Y_{n}^{\dagger}
  T_{n}
  X_{n}
  =
  \hbar
  C_{n}^{'\dagger}
  X_{n}.
  \label{minus_thm_eq_ens}
\end{align}
\noindent
%Here, \eqref{minus_thm_eq_ens} is \eqref{minus_thm_N2_eq_another} multiplied by \(X_{n}\) from the right.
Here, \eqref{minus_thm_eq_ens} is obtained by multiplying \eqref{minus_thm_N2_eq_another} by \(X_{n}\) from the right. This is merely a change to a form that allows direct substitution of the result of Theorem \ref{main_thm_N2}. The reason for using \eqref{minus_thm_N2_eq_another} rather than \eqref{minus_thm_N2_eq} is that \(X^{-1}_{n}\) appears if we try to check \eqref{minus_thm_N2_eq} directly, and it is difficult to calculate because it is an infinite power series matrix. In this discussion, we shall simply show only the cases \(n=1\) and \(2\).
\vspace{3mm}
\\
\noindent
\underline{
  Case:
  \(
    n
    =
    1
  \)
}
\vspace{3mm}
\\
Since Proposition \ref{prop:covar_const_0and1} and
\begin{align*}
  X_{1}
  &=
  \left(
    \begin{array}{cc}
      X_{11}^{1}  &  X_{12}^{1}  \\
      X_{21}^{1}  &  X_{22}^{1}
    \end{array}
  \right)
  =
  \mathrm{Id}_{2},
  \\
  Y_{1}
  &=
  \left(
    \begin{array}{cc}
      Y_{11}^{1}  &  Y_{12}^{1}  \\
      Y_{21}^{1}  &  Y_{22}^{1}
    \end{array}
  \right)
  =
  \left(
    \begin{array}{cc}
      1
      &
      0
      \\
      0
      &
      -
      1
    \end{array}
  \right),
\end{align*}
\noindent
it follows that
\begin{align*}
  Y_{1}^{\dagger}
  T_{1}
  X_{1}
  &=
  \hbar
  \left(
    \begin{array}{cc}
      g_{1\overline{1}}  &  g_{2\overline{1}}  \\
      -g_{1\overline{2}}  &  -g_{2\overline{2}}
    \end{array}
  \right),
  \\
  C_{1}^{\dagger}
  X_{1}
  &=
  \left(
    \begin{array}{cc}
      g_{\overline{1}1}  &  -g_{\overline{2}1}
      \\
      g_{\overline{1}2}  &  -g_{\overline{2}2}
    \end{array}
  \right)^{\dagger}=
  \left(
    \begin{array}{cc}
      g_{1\overline{1}}  &  g_{2\overline{1}}  \\
      -g_{1\overline{2}}  &  -g_{2\overline{2}}
    \end{array}
  \right).
\end{align*}
\noindent
Therefore 
\(
  Y_{1}^{\dagger}
  T_{1}
  X_{1}
  =
  \hbar
  C'_{1}
  X_{1}
\)
, equivalently 
\(
  Y_{1}^{\dagger}\left(\infty\right)
  T_{1}\left(\infty\right)
  X_{1}\left(\infty\right)
  =
  \hbar
  C'_{1}\left(\infty\right)
  X_{1}\left(\infty\right).
\)
\vspace{3mm}
\\
\noindent
\underline{
  Case:
  \(
    n
    =
    2
  \)
}
\vspace{3mm}
\\
Calculations for both sides of \eqref{minus_thm_eq_ens} yields
\begin{align}
  Y_{2}^{\dagger}
  T_{2}
  X_{2}
  =
  \hbar^{2}
  \left(
    \begin{array}{ccc}
      2
      +
      \hbar
      R_{1 \ \ \, 1}^{\ \, 11}
      &
      \hbar
      R_{1 \ \ \, 1}^{\ \, 21}
      &
      \hbar
      R_{1 \ \ \, 1}^{\ \, 22}
      \\
      0
      &
      0
      &
      0
      \\
      -
      \hbar
      R_{2 \ \ \, 2}^{\ \, 11}
      &
      -
      \hbar
      R_{2 \ \ \, 2}^{\ \, 21}
      &
      -2
      -
      \hbar
      R_{2 \ \ \, 2}^{\ \, 22}
    \end{array}
  \right)
  \left(
    \begin{array}{ccc}
      \left(
        g_{\overline{1}1}
      \right)^{2}
      &
      2
      g_{\overline{1}1}
      g_{\overline{2}1}
      &
      \left(
        g_{\overline{2}1}
      \right)^{2}
      \\
      2
      g_{\overline{1}1}
      g_{\overline{1}2}
      &
      2
      \left(
        g_{\overline{1}1}
        g_{\overline{2}2}
        +
        g_{\overline{1}2}
        g_{\overline{2}1}
      \right)
      &
      2
      g_{\overline{2}1}
      g_{\overline{2}2}
      \\
      \left(
        g_{\overline{1}2}
      \right)^{2}
      &
      2
      g_{\overline{1}2}
      g_{\overline{2}2}
      &
      \left(
        g_{\overline{2}2}
      \right)^{2}
    \end{array}
  \right)
\end{align}
\noindent
and
\begin{align}
  \hbar
  C'_{2}
  X_{2}
  =
  \hbar^{2}
  \left(
    \begin{array}{ccc}
      \left(
        g_{\overline{1}1}
      \right)^{2}
      &
      2
      g_{\overline{1}1}
      g_{\overline{2}1}
      &
      \left(
        g_{\overline{2}1}
      \right)^{2}
      \\
      0
      &
      0
      &
      0
      \\
      -
      \left(
        g_{\overline{1}2}
      \right)^{2}
      &
      -2
      g_{\overline{1}2}
      g_{\overline{2}2}
      &
      -
      \left(
        g_{\overline{2}2}
      \right)^{2}
    \end{array}
  \right)
  \left(
    \begin{array}{ccc}
      2
      +
      \hbar
      R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
      &
      2
      \hbar
      R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
      &
      \hbar
      R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}}
      \\
      \hbar
      R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
      &
      2
      +
      2
      \hbar
      R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
      &
      \hbar
      R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}}
      \\
      \hbar
      R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
      &
      2
      \hbar
      R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
      &
      2
      +
      \hbar
      R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
    \end{array}
  \right)
\end{align}
\noindent
respectively. Here we use 
\begin{align}
  T_{2}
  X_{2}
  =
  \hbar
  A'_{2}
  =
  \left(
    \begin{array}{ccc}
      \left(
        g_{\overline{1}1}
      \right)^{2}
      &
      2
      g_{\overline{1}1}
      g_{\overline{2}1}
      &
      \left(
        g_{\overline{2}1}
      \right)^{2}
      \\
      2
      g_{\overline{1}1}
      g_{\overline{1}2}
      &
      2
      \left(
        g_{\overline{1}1}
        g_{\overline{2}2}
        +
        g_{\overline{1}2}
        g_{\overline{2}1}
      \right)
      &
      2
      g_{\overline{2}1}
      g_{\overline{2}2}
      \\
      \left(
        g_{\overline{1}2}
      \right)^{2}
      &
      2
      g_{\overline{1}2}
      g_{\overline{2}2}
      &
      \left(
        g_{\overline{2}2}
      \right)^{2}
    \end{array}
  \right).
\end{align}
\noindent
Furthermore, each component 
%s 
of both sides of \eqref{minus_thm_eq_ens} coincides with each other from the calculations \eqref{lhs_first}--\eqref{rhs_last} in Appendix \ref{app_minus_n2}. Hence, it is shown that \eqref{minus_thm_eq_ens} for \(n=2\) holds.


==> NR/NCK2_plus.tex <==
\subsection{Complex two-dimensional formula}
\label{NR_plus}
\ The explicit formula for the coefficient 
\(
  T_{
    \overrightarrow{\alpha_{n}},
    \,
    \overrightarrow{\beta_{n}^{\ast}}
  }^{n}
\) 
for any order 
\(
  n
  \in
  \mathbb{Z}_{\geq0}
\) 
is obtained by not dealing with the recurrence relations independently but attributing them to one recurrence relation.% by summing over the index \(i\) that appears in given recurrence relations.
\begin{theorem}
  Let \(M\) be a complex two-dimensional locally symmetric K\"{a}hler manifold, \(U\) be an open set of \(M\), and 
  \(
%    f,g
%    \in
%    C^{\infty}
%    \left(U\right),
%    \
    \ast
  \) 
  be a star product with separation of variables on \(U\) such that
  \begin{align*}
    f
    \ast
    g
    =&
    \sum_{n=0}^{\infty}
    \sum_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}
    T_{\overrightarrow{\alpha_{n}},\,\overrightarrow{\beta_{n}^{\ast}}}^{n}
    \left(
      D^{\overrightarrow{\alpha_{n}}}f
    \right)
    \left(
      D^{\overrightarrow{\beta_{n}^{\ast}}}g
    \right)
    \\
    =&
    \sum_{n=0}^{\infty}
    \sum_{i,j=1}^{n+1}
    T_{ij}^{n}
    \left\{
      \left(
        D^{1}
      \right)^{n-i+1}
      \left(
        D^{2}
      \right)^{i-1}
      f
    \right\}
    \left\{
      \left(
        D^{\overline{1}}
      \right)^{n-j+1}
      \left(
        D^{\overline{2}}
      \right)^{j-1}
      g
    \right\}
  \end{align*}
  for 
  \(
    f,g
    \in
    C^{\infty}
    \left(U\right).
  \) 
  Then, 
  \begin{align}
    T_{n}
    X_{n}
    =
    \hbar
    A'_{n},
    \label{main_them_N2_T}
  \end{align}
  where
  \begin{align*}
    T_{n}
    &
    :=
    \left(
      T^{n}_{ij}
    \right)
    \in
    M_{n+1}
    \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right),
    \\
    T^{n}_{ij}
    &
    :=
    T_{
      \left(
        n-i+1,
        i-1
      \right),
      \left(
        n-j+1,
        j-1
      \right)
    }^{n},
    \\
    A'_{n}
    &
    =
    \left(A_{ij}^{'n}\right)
    =
    \left(
      \sum_{k,l=1}^{2}
      g_{\overline{k}l}
      T^{n-1}_{i-\delta_{2l},j-\delta_{2k}}
    \right)
    \in
    M_{n+1}
    \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right),
\end{align*}
and 
\(
  X_{n}
  \in
  M_{n+1}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\)
is a pentadiagonal matrix such that these components are given as follows :
\begin{align*}
    X_{j-2,j}^{n}
    &=
    \tbinom{n-j+3}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}},
    \\
    X_{j-1,j}^{n}
    &=
    2
    \tbinom{n-j+2}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    +
    \left(
      n-j+2
    \right)
    \left(
      j-2
    \right)
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}},
    \\
    X_{j,j}^{n}
    &=
    n
    +
    \tbinom{n-j+1}{2}
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    +
    \tbinom{j-1}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
    +
    2
    \left(
      n-j+1
    \right)
    \left(
      j-1
    \right)
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    X_{j+1,j}^{n}
    &=
    2
    \tbinom{j}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    +
    j
    \left(
      n-j
    \right)
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    X_{j+2,j}^{n}
    &=
    \tbinom{j+1}{2}
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}},
    \\
    X_{j,k}^{n}
    &=
    0
    \
    \left(
      \left|
        j-k
      \right|
      >
      2
    \right),
  \end{align*}
  \noindent
  where 
  \(
    \tbinom{m}{n}
  \) 
  is a binomial coefficient.
  \label{prop:general}
\end{theorem}

\begin{prf*}
  Note that, 
  \(
    \overrightarrow{\alpha_{n}}
    =
    \left(
      \alpha_{1}^{n},
      \alpha_{2}^{n}
    \right)
  \) 
  and 
  \(
    \overrightarrow{\beta_{n}}
    =
    \left(
      \beta_{1}^{n},
      \beta_{2}^{n}
    \right)
  \) 
  satisfy 
  \(
    \alpha_{1}^{n}
    +
    \alpha_{2}^{n}
    =
    \beta_{1}^{n}
    +
    \beta_{2}^{n}
    =
    n
  \). 
  All possible combinations of 
  \(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  \)
  are
  \(
    \left(
      n+1
    \right)^{2}
  \) 
  ways :
  %and they are as follows : 
  \begin{align*}
    \begin{array}{ccc}
      T_{
        \left(n,0\right),
        \left(n,0\right)
      }^{n}
      &
      \cdots
      &
      T_{
        \left(n,0\right),
        \left(0,n\right)
      }^{n},
      \\
      \vdots
      &
      \ddots
      &
      \vdots
      \\
      T_{
        \left(0,n\right),
        \left(n,0\right)
      }^{n}
      &
      \cdots
      &
      T_{
        \left(0,n\right),
        \left(0,n\right)
      }^{n}.
    \end{array}
  \end{align*}
  
  \noindent
  The recurrence relations for these 
  \(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  \) 
  satisfies
  \begin{flalign}
    &
    \sum_{d=1}^{2}
    \hbar
    g_{\overline{i}d}
    T_{\overrightarrow{\alpha_{n}}-\overrightarrow{e_{d}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{i}}}^{n-1}
    &
    \nonumber
    \\
    &=
    \beta_{i}^{n}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
    +
    \sum_{k=1}^{2}
    \sum_{c=1}^{2}
    \frac{
      \hbar
      \left(\beta_{k}^{n}-\delta_{kc}-\delta_{ik}+1\right)
      \left(\beta_{k}^{n}-\delta_{kc}-\delta_{ik}+2\right)
    }{2}
    R_{\overline{c} \ \ \ \,\overline{i}}^{\ \,\overline{k}\,\overline{k}}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{c}}+2\overrightarrow{e_{k}}-\overrightarrow{e_{i}}}^{n}
    &
    \nonumber
    \\
    &
    \mbox{}
    \quad
    +
    \sum_{c=1}^{2}
    \hbar
    \left(
      \beta_{1}^{n}
      -
      \delta_{1c}
      -
      \delta_{i1}
      +
      1
    \right)
    \left(
      \beta_{2}^{n}
      -
      \delta_{2c}
      -
      \delta_{i2}
      +
      1
    \right)
    R_{\overline{c} \ \ \ \,\overline{i}}^{\ \,\overline{2}\,\overline{1}}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{c}}+\overrightarrow{e_{1}}+\overrightarrow{e_{2}}-\overrightarrow{e_{i}}}^{n}
    &
    \label{rec_rel}
\end{flalign}

  \noindent
  from Theorem \ref{theorem:star_prd}, and two types of them for \(i=1,2\) exist. Both sides of these recurrence relations are linear combinations of some 
  \(
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}.
  \) 
  So we now make one new recurrence relation below by summing over the index \(i\) on both sides of them.
  \begin{flalign}
    &
    \sum_{i,d=1}^{2}
    \hbar
    g_{\overline{i}d}
    T_{\overrightarrow{\alpha_{n}}-\overrightarrow{e_{d}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{i}}}^{n-1}
    &
    \nonumber
    \\
    &=
    \sum_{i=1}^{2}
    \beta_{i}^{n}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
    +
    \sum_{i,k,c=1}^{2}
    \frac{
      \hbar
      \left(\beta_{k}^{n}-\delta_{kc}-\delta_{ik}+1\right)
      \left(\beta_{k}^{n}-\delta_{kc}-\delta_{ik}+2\right)
    }{2}
    R_{\overline{c} \ \ \ \,\overline{i}}^{\ \,\overline{k}\,\overline{k}}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{c}}+2\overrightarrow{e_{k}}-\overrightarrow{e_{i}}}^{n}
    &
    \nonumber
    \\
    &
    \mbox{}
    \quad
    +
    \sum_{i,c=1}^{2}
    \hbar
    \left(
      \beta_{1}^{n}
      -
      \delta_{1c}
      -
      \delta_{i1}
      +
      1
    \right)
    \left(
      \beta_{2}^{n}
      -
      \delta_{2c}
      -
      \delta_{i2}
      +
      1
    \right)
    R_{\overline{c} \ \ \ \,\overline{i}}^{\ \,\overline{2}\,\overline{1}}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{c}}+\overrightarrow{e_{1}}+\overrightarrow{e_{2}}-\overrightarrow{e_{i}}}^{n}.
    &
    \label{rec_rel_sum}
\end{flalign}
  
  \noindent
  Using the fact 
%  Note that each 
%  \(
%    \overrightarrow{\alpha_{n}}
%    =
%    \left(
%      \alpha_{1}^{n},
%      \alpha_{2}^{n}
%    \right)
%  \) 
%  and 
%  \(
%    \overrightarrow{\beta_{n}}
%    =
%    \left(
%      \beta_{1}^{n},
%      \beta_{2}^{n}
%    \right)
%  \) 
%  satisfy 
  \(
    \alpha_{1}^{n}
    +
    \alpha_{2}^{n}
    =
    n
  \) 
  and 
  \(
    \beta_{1}^{n}
    +
    \beta_{2}^{n}
    =
    n
  \), 
%  respectively. Thus, 
we can 
  %We now for any 
%\(
%  n
%  \in
%  \mathbb{Z}_{\geq0}
%\) 
redefine the coefficients 
\(
  %T^{n}_{i,j}
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}
\) 
%and the indices 
%\(
%  i,
%  \
%  j
%\)
%with
as
\begin{align*}
  T^{n}_{i,j}
  :=
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n},
  \
  i
  :=
  \alpha_{2}^{n}+1,
  \
  j
  :=
  \beta_{2}^{n}+1.
\end{align*}
  \noindent
  Then the %both sides of this 
  recurrence relation \eqref{rec_rel_sum} is rewritten as
  \begin{align}
    \hbar
    \sum_{k,l=1}^{2}
    g_{\overline{k}l}
    T^{n-1}_{i-\delta_{2l},j-\delta_{2k}}
    =
    X_{j-2}^{n}
    T_{i,j-2}^{n}
    +
    X_{j-1}^{n}
    T_{i,j-1}^{n}
    +
    X_{j}^{n}
    T_{i,j}^{n}
    +
    X_{j+1}^{n}
    T_{i,j+1}^{n}
    +
    X_{j+1}^{n}
    T_{i,j+2}^{n},
    \label{rec_rel_lhs_symb}
\end{align}

  %Expanding both sides of this recurrence relation \eqref{rec_rel_sum} to clarify the coefficient part of each 
%  \(
%    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n},
%  \)
%  \begin{align*}
%    &
%    \hbar
%    \left(
%      g_{\overline{1}1}
%      T_{\left(\alpha_{1}^{n}-1,\alpha_{2}^{n}\right),
%      \left(\beta_{1}^{n}-1,\beta_{2}^{n}\right)}^{n-1}
%      +
%      g_{\overline{1}2}
%      T_{\left(\alpha_{1}^{n},\alpha_{2}^{n}-1\right),
%      \left(\beta_{1}^{n}-1,\beta_{2}^{n}\right)}^{n-1}
%      +
%      g_{\overline{2}1}
%      T_{\left(\alpha_{1}^{n}-1,\alpha_{2}^{n}\right),
%      \left(\beta_{1}^{n},\beta_{2}^{n}-1\right)}^{n-1}
%      +
%      g_{\overline{2}2}
%      T_{\left(\alpha_{1}^{n},\alpha_{2}^{n}-1\right),
%      \left(\beta_{1}^{n},\beta_{2}^{n}-1\right)}^{n-1}
%    \right)
%    \\
%    &=
%    X_{\left(\beta_{1}^{n}+2,\beta_{2}^{n}-2\right)}^{n}
%    T_{\overrightarrow{\alpha_{n}},
%    \left(\beta_{1}^{n}+2,\beta_{2}^{n}-2\right)}^{n}
%    +
%    X_{\left(\beta_{1}^{n}+1,\beta_{2}^{n}-1\right)}^{n}
%    T_{\overrightarrow{\alpha_{n}},
%    \left(\beta_{1}^{n}+1,\beta_{2}^{n}-1\right)}^{n}
%    +
%    X_{\left(\beta_{1}^{n},\beta_{2}^{n}\right)}^{n}
%    T_{\overrightarrow{\alpha_{n}},
%    \left(\beta_{1}^{n},\beta_{2}^{n}\right)}^{n}
%    \\
%    &
%    \quad
%    +
%    X_{\left(\beta_{1}^{n}-1,\beta_{2}^{n}+1\right)}^{n}
%    T_{\overrightarrow{\alpha_{n}},
%    \left(\beta_{1}^{n}-1,\beta_{2}^{n}+1\right)}^{n}
%    +
%    X_{\left(\beta_{1}^{n}-2,\beta_{2}^{n}+2\right)}^{n}
%    T_{\overrightarrow{\alpha_{n}},
%    \left(\beta_{1}^{n}-2,\beta_{2}^{n}+2\right)}^{n},
%\end{align*}

\noindent
where each 
\(
  X_{j}^{n}
\) 
is given as
\begin{align*}
    X_{j-2}^{n}
    &=
    \tbinom{n-j+3}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}},
    \\
    X_{j-1}^{n}
    &=
    2
    \tbinom{n-j+2}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    +
    \left(
      n
      -
      j+2
    \right)
    \left(
      j
      -
      2
    \right)
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}},
    \\
    X_{j}^{n}
    &=
    n
    +
    \tbinom{n-j+1}{2}
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    +
    \tbinom{j-1}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
    +
    2
    \left(
      n
      -
      j
      +
      1
    \right)
    \left(
      j-1
    \right)
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    X_{j+1}^{n}
    &=
    2
    \tbinom{j}{2}
    \hbar
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    +
    j
    \left(
      n
      -
      j
    \right)
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    X_{j+2}^{n}
    &=
    \tbinom{j+1}{2}
    \hbar
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}},
  \end{align*}
%using properties of the curvature \eqref{curv_kaehler_prop} in Appendix \ref{app_kaehler} and 
%\(
%  \left|
%    \overrightarrow{\beta_{n}^{\ast}}
%  \right|
%  =
%  \beta_{1}^{n}
%  +
%  \beta_{2}^{n}
%  =
%  n
%\)
%and 
%\(
%  X_{\left(-,-\right)}^{n}
%\) 
%is given 
%also put the coefficient part of 
%\(
%  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n},
%\) 
%as 
%  \begin{align*}
%    X_{\left(\beta_{1}^{n}+2,\beta_{2}^{n}-2\right)}^{n}
%    &=
%    \tbinom{n-\beta_{2}^{n}+2}{2}
%    \hbar
%    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}},
%    \\
%    X_{\left(\beta_{1}^{n}+1,\beta_{2}^{n}-1\right)}^{n}
%    &=
%    2
%    \tbinom{n-\beta_{2}^{n}+1}{2}
%    \hbar
%    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
%    +
%    \left(
%      \beta_{2}^{n}
%      -
%      1
%    \right)
%    \left\{
%      n
%      -
%      \left(
%        \beta_{2}^{n}
%        -
%        1
%      \right)
%    \right\}
%    \hbar
%    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}},
%    \\
%    X_{\left(\beta_{1}^{n},\beta_{2}^{n}\right)}^{n}
%    &=
%    X_{\overrightarrow{\beta_{n}}}^{n}
%    =
%    n
%    +
%    \tbinom{n-\beta_{2}^{n}}{2}
%    \hbar
%    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
%    +
%    \tbinom{\beta_{2}^{n}}{2}
%    \hbar
%    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
%    +
%    2
%    \beta_{2}^{n}
%    \left(
%      n
%      -
%      \beta_{2}^{n}
%    \right)
%    \hbar
%    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
%    \\
%    X_{\left(\beta_{1}^{n}-1,\beta_{2}^{n}+1\right)}^{n}
%    &=
%    2
%    \tbinom{\beta_{2}^{n}+1}{2}
%    \hbar
%    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
%    +
%    \left(
%      \beta_{2}^{n}
%      +
%      1
%    \right)
%    \left\{
%      n
%      -
%      \left(
%        \beta_{2}^{n}
%        +
%        1
%      \right)
%    \right\}
%    \hbar
%    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
%    \\
%    X_{\left(\beta_{1}^{n}-2,\beta_{2}^{n}+2\right)}^{n}
%    &=
%    \tbinom{\beta_{2}^{n}+2}{2}
%    \hbar
%    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}},
%  \end{align*}
%respectively. 
%To denote each 
%\(
%  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
%\) 
%using a matrix representation, we rewrite this recurrence relation using geometric vectors. 
%For any 
%\(
%  n
%  \in
%  \mathbb{Z}_{\geq0},
%  \
%  T^{n}_{\alpha_{2}^{n}+1,\beta_{2}^{n}+1}
%\) 

%and 
%\(X^{n;\beta_{2}^{n}+1}\) 

%are defined by
%\begin{align*}
%  T^{n}_{\alpha_{2}^{n}+1,\beta_{2}^{n}+1}
%  &:=
%  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}}}^{n}.
  %\\
  %X_{\overrightarrow{\beta_{n}}}^{n}
  %&:=
  %X_{\beta_{2}^{n}+1}^{n}
%\end{align*}

%\noindent
%respectively. 
%Note that from such a correspondence for 
%\(
%  \overrightarrow{\alpha_{n}},
%  \overrightarrow{\beta_{n}}
%\) 
%and 
%\(
%  \alpha_{2}^{n},
%  \beta_{2}^{n},
%\) 
%the notation by indices \(i\) and \(j\) can be rewritten as
%\begin{align*}
%  T^{n}_{ij}
%  &
%  :=
%  T_{
%    \left(
%      n-i+1,
%      i-1
%    \right),
%    \left(
%      n-j+1,
%      j-1
%    \right)
%  }^{n},
%  \\
%  %X_{j}^{n}
%  &
%  X_{
%    \left(
%      n-j+1,
%      j-1
%    \right)
%  }^{n}
%  :=
%  X_{\overrightarrow{\beta_{n}}}^{n}
%  =
%  X_{\left(\beta_{1}^{n},\beta_{2}^{n}\right)}^{n}
%\end{align*}

%\noindent
%with \(i:=\alpha_{2}^{n}+1\) and \(j:=\beta_{2}^{n}+1.\) 

\noindent
respectively. We put 
%Note 
that 
\(
  X_{j}^{n}
  :=
  0
\) 
when \(j<0\) or \(j>n+1\).
%where for either \(i<0,\) \(i>n+1,\) \(j<0\) or \(j>n+1\), we define 
%\(
%  X_{ij}^{n}:=0
%\) 
%for 
%\(
%  X_{ij}^{n},
%\) 
%and 
%\(
%  T^{n}_{ij},
%\) 
%which will be discussed later, are 0 by the definition of 
%\(
%  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}}}^{n}.
%\) 
%Therefore
Here, introducing 
%redefining 
each 
\(
  X_{k,j}^{n}
\) 
for 
\(
  k
  =
  1,
  \cdots,
  j,
  \cdots,
  n+1
\) 
by
\begin{flalign*}
  &
  \left(
      \begin{array}{ccccccccccc}
        0
        &
        \cdots
        &
        0
        &
        X_{j-2,j}^{n}
        &
        X_{j-1,j}^{n}
        &
        X_{j,j}^{n}
        &
        X_{j+1,j}^{n}
        &
        X_{j+2,j}^{n}
        &
        0
        &
        \cdots
        &
        0
      \end{array}
  \right)^{T}
  &
  \\
  &
  :=
  \left(
      \begin{array}{ccccccccccc}
        0
        &
        \cdots
        &
        0
        &
        X_{j-2}^{n}
        &
        X_{j-1}^{n}
        &
        X_{j}^{n}
        &
        X_{j+1}^{n}
        &
        X_{j+2}^{n}
        &
        0
        &
        \cdots
        &
        0
      \end{array}
  \right)^{T}
  ,
  &
\end{flalign*}

\noindent
then %each sides of the recurrence relation \eqref{rec_rel_sum} can be written as
the right-hand side of the recurrence relation \eqref{rec_rel_lhs_symb} can be written as
  \begin{align*}
    \left(r.h.s.\right)
    &=
    \left(
      \begin{array}{ccc}
        T^{n}_{i,1}
        &
        \cdots
        &
        T^{n}_{i,n+1}
      \end{array}
    \right)
    \left(
      \begin{array}{ccccccccccc}
        0
        &
        \cdots
        &
        0
        &
        X_{j-2,j}^{n}
        &
        X_{j-1,j}^{n}
        &
        X_{j,j}^{n}
        &
        X_{j+1,j}^{n}
        &
        X_{j+2,j}^{n}
        &
        0
        &
        \cdots
        &
        0
      \end{array}
    \right)^{T}.
%    \\
%    \left(l.h.s.\right)
%    &=
%    \hbar
%    \sum_{k,l=1}^{2}
%    g_{\overline{k}l}
%    T^{n-1}_{i-\delta_{2l},j-\delta_{2k}},
  \end{align*}
  \noindent
%  respectively. %Here, . 
  Furthermore, to summarize the recurrence relation \eqref{rec_rel_lhs_symb} by a matrix representation, we introduce \(A_{ij}^{'n}\) for the left-hand side and 
  \(
    \mathbf{X}_{j}
  \)
%  \(
%    \left(
%      0,
%      \cdots,
%      0,
%      X_{j-2,j}^{n},
%      X_{j-1,j}^{n},
%      X_{j,j}^{n},
%      X_{j+1,j}^{n},
%      X_{j+2,j}^{n},
%      0,
%      \cdots,
%      0
%    \right)^{T}
%  \) 
  for the right-hand side as 
  \begin{align*}
    A_{ij}^{'n}
    :=&
%    \hbar
    \sum_{k,l=1}^{2}
    g_{\overline{k}l}
    T^{n-1}_{i-\delta_{2l},j-\delta_{2k}}
    \\
    \mathbf{X}_{j}
%    =&
%    \left(
%      \begin{array}{ccccccccccc}
%        0
%        &
%        \cdots
%        &
%        0
%        &
%        X_{j-2}^{n;j}
%        &
%        X_{j-1}^{n;j}
%        &
%        X_{j}^{n;j}
%        &
%        X_{j+1}^{n;j}
%        &
%        X_{j+2}^{n;j}
%        &
%        0
%        &
%        \cdots
%        &
%        0
%      \end{array}
%    \right)
%    \\
    :=&
    \left(
      \begin{array}{ccccccccccc}
        0
        &
        \cdots
        &
        0
        &
        X_{j-2,j}^{n}
        &
        X_{j-1,j}^{n}
        &
        X_{j,j}^{n}
        &
        X_{j+1,j}^{n}
        &
        X_{j+2,j}^{n}
        &
        0
        &
        \cdots
        &
        0
      \end{array}
    \right)^{T},
  \end{align*}
  \noindent
  respectively. Thus, by summarizing the recurrence relation \eqref{rec_rel_lhs_symb} for each \(i\) and using a matrix representation, we have
  \begin{align*}
    \hbar
    A'_{n}
    =
    T_{n}
    X_{n}
  \end{align*}
  \noindent
  for the coefficient 
  \(
    T^{n}_{i,j}
    =
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n},
  \) 
  where 
  \(
    T_{n}
    :=
    \left(
      T^{n}_{ij}
    \right),
    \
    A'_{n}
    =
    \left(A_{ij}^{'n}\right)
    \in
    M_{n+1}
    \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
    \right)
  \), 
  and
  \begin{align*}
    %T^{n}_{ij}
    %&
    %:=
    %T_{
    %  \left(
    %    n-i+1,
    %    i-1
    %  \right),
    %  \left(
    %    n-j+1,
    %    j-1
    %  \right)
    %}^{n},
    %\\
    %A'_{n}
    %&
    %=
    %\left(A_{ij}^{'n}\right)
    %=
    %\left(
    %  \sum_{k,l=1}^{2}
    %  g_{\overline{k}l}
    %  T^{n-1}_{i-\delta_{2l},j-\delta_{2k}}
    %\right)
    %\in
    %M_{n}
    %\left(
    %\mathbb{C}
    %\left[\!
    %  \left[
    %    \hbar
    %  \right]\!
    %\right]
    %\right),
    %\\
    X_{n}
    &=
    \left(
      \mathbf{X}_{1},
      \cdots,
      \mathbf{X}_{n+1}
    \right)
    \\
    &=
    \left(
    \left.
      \begin{array}{ccccccccccc}
        X_{11}^{n} & X_{12}^{n} & X_{13}^{n} & 0 & 0 & & & & & & \text{\huge{0}} \\
        X_{21}^{n} & X_{22}^{n} & X_{23}^{n} & X_{24}^{n} & 0 & \ddots & & & & & \\
        X_{31}^{n} & X_{32}^{n} & X_{33}^{n} & X_{34}^{n} & X_{35}^{n} & \ddots & \ddots & & & & \\
        0          & X_{22}^{n} & X_{43}^{n} & X_{44}^{n} & X_{45}^{n} & \ddots & \ddots & \ddots & & & \\
        0          & 0          & X_{53}^{n} & X_{54}^{n} & X_{55}^{n} & \ddots & \ddots & \ddots & \ddots & & \\
                              & \ddots     & \ddots     & \ddots     & \ddots     & \ddots & \ddots & \ddots & \ddots & \ddots & \\
                              & & \ddots     & \ddots & \ddots & \ddots & X_{n-3,n-3}^{n} & X_{n-3,n-2}^{n} & X_{n-3,n-1}^{n} & 0 & 0 \\
                   &  &  & \ddots & \ddots & \ddots & X_{n-2,n-3}^{n} & X_{n-2,n-2}^{n} & X_{n-2,n-1}^{n} & X_{n-2,n}^{n} & 0 \\
                   &            &            &        & \ddots & \ddots & X_{n-1,n-3}^{n} & X_{n-1,n-2}^{n} & X_{n-1,n-1}^{n} & X_{n-1,n}^{n} & X_{n-1,n+1}^{n} \\
                   &            &            & & & \ddots & 0 & X_{n,n-2}^{n} & X_{n,n-1}^{n} & X_{n,n}^{n} & X_{n,n+1}^{n} \\
        \text{\huge{0}} &            & & & & & 0 & 0 & X_{n+1,n-1}^{n} & X_{n+1,n}^{n} & X_{n+1,n+1}^{n}
      \end{array}
    \right.
    \right).
  \end{align*}
  
  \noindent
%  and 
%  \(
%    X_{i,j}^{n}
%    :=
%    X_{i}^{n;j}.
%  \) 
  This proof was completed.\(_{\blacksquare}\)
\end{prf*}

\noindent
\ Here, we note %the following points
the fact with respect to \(X_{k}\) %. It follows 
that each \(X_{k}^{-1}\), the inverse matrix of each \(X_{k}\), is determined by a formal power series with respect to a matrix 
\(
  H_{k}
  \in
  M_{k+1}
  \left(
    \mathbb{C}
  \right).
\) 
Here \(H_{k}\) is a pentadiagonal matrix such that each component depends on Riemann curvature tensors on \(M\).
%However, the regularity of each \(X_{k}\) is not yet clearly known in general. For example, it is known that each \(X_{k}\) is regular for \(\mathbb{C}^{2}, \mathbb{C}P^{2}\) and \(\mathbb{C}H^{2}\). So we show that if the each \(X_{k}\) is regular, then the inverse \(X_{k}^{-1}\) is determined a formal power series of a pentadiagonal matrix which each component depends on Riemann curvature tensor on \(M\).
We 
%now \(X_{k}\) 
decompose \(X_{k}\) into the two matrices:
\begin{align*}
  X_{k}
  =
  k
  \mathrm{Id}_{k+1}
  +
  \hbar
  H_{k},
\end{align*}

\noindent
where 
\(
  H_{k}
\)
 %is a matrix such that each component is independent of \(\hbar\) and 
 is given as follows :
\begin{align*}
    H_{j-2,j}^{k}
    &=
    \tbinom{k-j+3}{2}
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}},
    \\
    H_{j-1,j}^{k}
    &=
    2
    \tbinom{k-j+2}{2}
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    +
    \left(
      k-j+2
    \right)
    \left(
      j-2
    \right)
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}},
    \\
    H_{j,j}^{k}
    &=
    \tbinom{k-j+1}{2}
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
    +
    \tbinom{j-1}{2}
    R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
    +
    2
    \left(
      k-j+1
    \right)
    \left(
      j-1
    \right)
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    H_{j+1,j}^{k}
    &=
    2
    \tbinom{j}{2}
    R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
    +
    j
    \left(
      k-j
    \right)
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}},
    \\
    H_{j+2,j}^{k}
    &=
    \tbinom{j+1}{2}
    R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}},
    \\
    H_{j,l}^{k}
    &=
    0
    \
    \left(
      \left|
        j-l
      \right|
      >
      2
    \right).
  \end{align*}
%Next, we assume that the inverse \(X_{k}^{-1}\) is given by a formal parameter series of some matrices 
%\(
%  G_{p}
%  \in
%  M_{k+1}
%  \left(
%    \mathbb{C}
%  \right)
%\)
%\begin{align}
%  X_{k}^{-1}
%  =
%  \sum_{p=0}^{\infty}
%  \hbar^{p}
%  G_{p}.
%  \label{formal_Xk_inv}
%\end{align}
%
%\noindent
%Thus, \(X_{k}^{-1}\) will be obtained by sequentially determining the above \(G_{p}\). Substituting \eqref{formal_Xk_inv} into the left-hand side of \(X_{k}X_{k}^{-1}=\mathrm{Id}_{k+1}\), we have
%\begin{align*}
%  \mathrm{Id}_{k+1}
%  =&
%  \left(
%    k
%    \mathrm{Id}_{k+1}
%    +
%    \hbar
%    H
%  \right)
%  \sum_{p=0}^{\infty}
%  \hbar^{p}
%  G_{p}
%  \\
%  =&
%  k
%  +
%  \hbar
%  \left(
%    k
%    G_{1}
%    +
%    H
%    G_{0}
%  \right)
%  +
%  \hbar^{2}
%  \left(
%    k
%    G_{2}
%    +
%    H
%    G_{1}
%  \right)
%  +
%  \cdots.
%\end{align*}
%
%\noindent
%Comparing the coefficients on both sides of the above equation, we obtain
%\begin{align*}
%  G_{0}
%  =&
%  \frac{1}{k}
%  \mathrm{Id}_{k+1},
%  \\
%  G_{1}
%  =&
%  -
%  \frac{1}{k}
%  HG_{0},
%  \\
%  G_{2}
%  =&
%  -
%  \frac{1}{k}
%  HG_{1},
%  \\
%  &\vdots
%\end{align*}
%\noindent
%that is,
%\begin{align*}
%  G_{0}
%  =
%  \frac{1}{k}
%  \mathrm{Id}_{k+1},
%  \
%  G_{1}
%  =
%  -
%  \frac{1}{k^{2}}
%  H,
%  \
%  G_{2}
%  =
%  \frac{1}{k^{3}}
%  H^{2},
%  \
%  \cdots.
%\end{align*}
%
%\noindent
%Hence,
%\begin{align}
%  G_{p}
%  =
%  \frac{
%    \left(-1\right)^{p}
%  }{
%    k^{p+1}
%  }
%  H^{p}
%  \
%  \left(
%    p\geq0
%  \right).
%  \label{explicit_Gp}
%\end{align}
%
\noindent
%Substituting \eqref{explicit_Gp} into \eqref{formal_Xk_inv}, it is turn out that
Then, \(X_{k}^{-1}\) is given by
\begin{align}
  X_{k}^{-1}
  =&
  \sum_{p=0}^{\infty}
  \frac{
    \left(
      -\hbar
    \right)^{p}
  }{
    k^{p+1}
  }
  \left(H_{k}\right)^{p}.
  \label{Xk_inv_fps}
\end{align}

\noindent
Note that, since a power of a pentadiagonal matrix is not a pentadiagonal matrix in general, \(X_{k}\) is pentadiagonal but \(X_{k}^{-1}\) is not always pentadiagonal.
\bigskip
\\
\ For each 
\(
  n
  \in
  \mathbb{Z}_{\geq0}
\), 
\(
  T_{n}
  \in
  M_{n+1}
  \left(
  \mathbb{C}
  \left[\!
    \left[
      \hbar
    \right]\!
  \right]
  \right),
\) 
%which \(T_{n}\) is a square matrix of order \(n+1\), 
%so 
\eqref{main_them_N2_T} is also a square matrix of order \(n+1\). %However, these 
These matrices are not a unified expression, as the size of matrices depends on \(n\), then it is inconvenient to solve the general term. This problem can be solved by embedding ``finite-dimensional" matrices into ``infinite-dimensional" matrices, and such a procedure provides a unified expression for \(n\geq2\). %In this discussion, we use the following embedding from 
%\(
%  M_{n}\left(\mathbb{C}\right)
%\)
%to 
%\(
%  M_{\infty}\left(\mathbb{C}\right)
%\). 
%\vspace{3mm}
%\\
%\noindent
%\underline{
%  Case : The others
%}
%\vspace{3mm}
%\\
For matrices 
\(
  A
  \in
  M_{n}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\) 
%that are not \(\mathrm{Id}_{n},\) \(F_{d,n}\) or \(F_{r,n}\) 
the embedding of \(A\) is carried out so that the component whose row or column is greater than \(n\) is 0. That is, the embedding is
%into 
%\(
%  M_{\infty}\left(\mathbb{C}\right)
%\) 
%for \(A\) is carried out as follows :
\begin{align}
  A
  =
  \left(
    \begin{array}{ccc}
      a_{11}  &  \cdots  &  a_{1n}  \\
      \vdots  &  \ddots  &  \vdots  \\
      a_{n1}  &  \cdots  &  a_{nn}
    \end{array}
  \right)
  \mapsto
  A\left(\infty\right)
  :=
  \left(
    \begin{array}{ccc|ccc}
      a_{11}  &  \cdots  &  a_{1n} &   &  \\
      \vdots  &  \ddots  &  \vdots &  &  \text{\huge{0}}  & \\
      a_{n1}  &  \cdots  &  a_{nn}  &  &  &  \\ \hline
        &  &  &  &  & \\
        &  \text{\huge{0}}  &  &  &  \text{\huge{0}}  &  \\
        &  &  &  &  &  \\
    \end{array}
  \right)
  =
  \left(
    \begin{array}{c|c}
      A & 0 \\  \hline
      0 & 0
    \end{array}
  \right).
  \label{emb_gene}
\end{align}

\noindent
%As in the case of \(\mathrm{Id},\) \(F_{d,n}\) and \(F_{r,n},\) the embedding matrix of \(A\) is denoted as \(A\left(\infty\right).\)
%\vspace{3mm}
%\\
%
%\noindent
%\underline{
%  Case : \(\mathrm{Id}_{n}\)
%}
%\vspace{3mm}
%\\
In the following calculations, we use \(\mathrm{Id}_{n}\), \(\mathrm{Id}\left(\infty\right)\), \(F_{d,n}\), \(F_{d}\left(\infty\right)\) \(F_{r,n}\) and \(F_{r}\left(\infty\right)\) given by %\\
%\ For the identity matrix 
%\(
%  \mathrm{Id}_{n},
%\) 
%the embedding into 
%\(
%  M_{\infty}\left(\mathbb{C}\right) :
%\) 
%is as follows :
\begin{align}
  &
  \mathrm{Id}_{n}
  =
  \left(
    \begin{array}{ccc}
      1 & & 0 \\
       & \ddots &  \\
      0 & & 1
    \end{array}
  \right),
  &
%  \mapsto
%  \left(
%    \begin{array}{c|ccc}
%      \mathrm{Id}_{n} & & \text{\huge{0}} & \\ \hline
%        & 1 & 0 & \\
%      \text{\huge{0}} & 0 & 1 & \\
%        &  & & \ddots
%    \end{array}
%  \right)
%  =
  &
  \mathrm{Id}\left(\infty\right)
  =
  \left(
    \begin{array}{ccc}
%      1 & & 0 & & & \\
%       & \ddots & & & \text{\huge{0}} & \\
%      0 & & 1 & & & \\  \hline
       1 & 0 & \\
       0 & 1 & \\
         &  & \ddots
    \end{array}
  \right),
  &
  \label{emb_id}
  \\
  &
  F_{d,n}
  =
  \left(
    \begin{array}{cccc}
      0 &  & & \\
      1 & 0 &  & \\
       & \ddots & \ddots \\
       & &  1  &  0
    \end{array}
  \right),
  &
%  \mapsto  
%  \left(
%    \begin{array}{cccc|ccc}
%      0 &  & & & & & \\
%      1 & 0 &  & & & \text{\huge{0}} & \\
%       & \ddots & \ddots & & & \\
%       & &  1  &  0 & & & \\  \hline
%       & &  &  1 & 0  & & \\
%       & \text{\huge{0}} &  &  &  1  &  0  &  \\
%       & &  &  & & \ddots &  \ddots
%    \end{array}
%  \right)
  &
  F_{d}\left(\infty\right)
  =
  \left(
    \begin{array}{cccc}
      0 &  & & \\
      1 & 0 &  & \\
       & 1 & 0 \\
       & &  \ddots  &  \ddots
    \end{array}
  \right),
  &
%  =:
  \label{emb_Fd}
  \\
  &
  F_{r,n}
  =
  F_{d,n}^{T},
  &
%  \left(
%    \begin{array}{cccc}
%      0 & 1 & & \\
%       & 0 & \ddots & \\
%       & & \ddots & 1 \\
%       & & & 0
%    \end{array}
%  \right)
%  \mapsto
%  \left(
%    \begin{array}{cccc|ccc}
%      0 & 1 & & & & & \\
%       & 0 & \ddots & & & \text{\huge{0}} & \\
%       & & \ddots & 1 & & \\
%       & & & 0 & 1 & & \\  \hline
%       & &  & & 0 & 1 & \\
%       & \text{\huge{0}} &  &  & & 0 & \ddots \\
%       & &  &  & & &  \ddots
%    \end{array}
%  \right)
  &
  F_{r}\left(\infty\right)
  =
%  \left(
%    \begin{array}{cccc}
%      0 & 1 & & \\
%       & 0 & 1 & \\
%       & & 0 & \ddots \\
%       & & & \ddots
%    \end{array}
%  \right)
%  =:
  F_{d}\left(\infty\right)^{T}.
  &
  \label{emb_Fr}
\end{align}
%
%\noindent
%where we denote the embedding matrix for \(\mathrm{Id}_{n}\) by \(\mathrm{Id}\left(\infty\right).\)
%\vspace{3mm}
%\\
%\noindent
%\underline{
%  Case : \(F_{d,n}\) and \(F_{r,n}\)
%}
%\vspace{3mm}
%\\
%\ We now %define
%introduce the lower and upper shift matrices \(F_{d,n}\) and \(F_{r,n}\) by
%\begin{align*}
%  F_{d,n}
%  :=
%  \left(
%    \begin{array}{cccc}
%      0 &  & & \\
%      1 & 0 &  & \\
%       & \ddots & \ddots \\
%       & &  1  &  0
%    \end{array}
%  \right),
%  \
%  F_{r,n}
%  :=
%  \left(F_{d,n}\right)^{T}
%  =
%  \left(
%    \begin{array}{cccc}
%      0 & 1 & & \\
%       & 0 & \ddots & \\
%       & & \ddots & 1 \\
%       & &  &  0
%    \end{array}
%  \right),
%\end{align*}
%
%\noindent
%respectively. %Note that multiplying \(F_{d,n}\) from the left corresponds to ``the operation of shifting each row of the matrix down by one row", and multiplying \(F_{r,n}\) from the right corresponds to ``the operation of shifting each column of the matrix right by one column".
%For \(F_{d,n},\) the embedding into 
%\(
%  M_{\infty}\left(\mathbb{C}\right)
%\) 
%is as follows :
%
%\begin{align}
%  
%\end{align}
%
%\noindent
%The embedding into 
%\(
%  M_{\infty}\left(\mathbb{C}\right)
%\) 
%for \(F_{r,n}\) is also carried out in a similar way :
%\begin{align}
%  
%\end{align}
%
%\noindent
%Here we denote the embedding matrices for \(F_{d,n}\) and \(F_{r,n}\) by \(F_{d}\left(\infty\right)\) and \(F_{r}\left(\infty\right).\)

\begin{remark}
  Note that multiplying \(F_{d,n}\) from the left corresponds to %``the operation of shifting each row of the matrix down by one row".
  ``shifting the components of the matrix downward by one position, with zeros appearing in the top row". And multiplying \(F_{r,n}\) from the right corresponds to ``shifting the components of the matrix rightward by one position, with zeros appearing in the first column". %So we can say that 
  \(F_{d}\left(\infty\right)\) and \(F_{r}\left(\infty\right)\) correspond %s 
  to their infinite-dimensional versions.
  \label{rem_Fd_Fr}
\end{remark}

%Recalling that \(F_{d}\) (or \(F_{r}\)) corresponds to the operation with respect to matrices such that the number of rows (or columns) is \(n,\) we can say that \(F_{d}\left(\infty\right)\) (or \(F_{r}\left(\infty\right)\)) corresponds to their infinite dimensional versions.
%\vspace{3mm}
%\\
\ %We now extend the embedding to the case of 
%\(
%  M_{n}
%  \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%  \right)
%\) 
%and 
%\(
%  M_{\infty}
%  \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%  \right)
%\) 
%and attempt to apply it to give \(T_{n}\) explicitly. 
%First, from Proposition \ref{prop:covar_const_0and1},
%\begin{align*}
%  T^{0}_{11}
%  =
%  T_{\overrightarrow{\alpha_{0}},\overrightarrow{\beta_{0}^{\ast}}}^{0}
%  =
%  T^{0}_{\left(0,0\right),\left(0,0\right)}
%  =
%  1,
%  \
%  \left(
%      \begin{array}{cc}
%        T_{
%          \left(1,0\right),
%          \left(1,0\right)
%        }^{1}
%        &
%        T_{
%          \left(1,0\right),
%          \left(0,1\right)
%        }^{1}
%        \\
%       T_{
%          \left(0,1\right),
%          \left(1,0\right)
%        }^{1}
%        &
%        T_{
%          \left(0,1\right),
%          \left(0,1\right)
%        }^{1}
%      \end{array}
%    \right)
%    =
%    \hbar
%    \left(
%      \begin{array}{cc}
%        g_{1\bar{1}}
%        &
%        g_{1\bar{2}}
%        \\
%        g_{2\bar{1}}
%        &
%        g_{2\bar{2}}
%      \end{array}
%    \right),
%\end{align*}
%
%\noindent
% so \(T_{0}\) and \(T_{1}\) are immediately obtained as
%\begin{align*}
%  T_{0}
%  =
%  \left(1\right),
%  \
%  T_{1}
%  =
%  \hbar
%  \left(
%    \begin{array}{cc}
%      g_{1\bar{1}}
%      &
%      g_{1\bar{2}}
%      \\
%      g_{2\bar{1}}
%      &
%      g_{2\bar{2}}
%    \end{array}
%  \right),
%\end{align*}
%
%\noindent
%where 
%\(
%  T_{0}
%  \in
%  M_{1}\left(\mathbb{C}\right).
%\) 
%These are the initial values of the recurrence relations respectively, so we denote 
From Proposition \ref{prop:covar_const_0and1}, the embeddings of 
\(
  T_{0}\left(\infty\right)
\) 
and 
\(
  T_{1}\left(\infty\right)
\) 
are 
\begin{align*}
  T_{0}
  =
  \left(1\right)
  &
  \mapsto
  T_{0}\left(\infty\right)
  :=
  \left(
  \begin{array}{c|c}
    T_{0} & 0 \\  \hline
    0 & 0
  \end{array}
  \right)
  =
  \left(
  \begin{array}{ccc}
    1 & 0 & \cdots \\
    0 & 0 & \\
    \vdots & & \ddots
  \end{array}
  \right),
  \\
  T_{1}
  =
  \hbar
  \left(
    \begin{array}{cc}
      g_{1\bar{1}}
      &
      g_{1\bar{2}}
      \\
      g_{2\bar{1}}
      &
      g_{2\bar{2}}
    \end{array}
  \right)
  &
  \mapsto
  T_{1}\left(\infty\right)
  :=
  \left(
  \begin{array}{c|c}
    T_{1} & 0 \\  \hline
    0 & 0
  \end{array}
  \right)
  =
  \hbar
  \left(
    \begin{array}{cccc}
      g_{1\bar{1}}
      &
      g_{1\bar{2}}
      &
      0
      &
      \cdots
      \\
      g_{2\bar{1}}
      &
      g_{2\bar{2}}
      &
      0
      &
      \\
      0
      &
      0
      &
      0
      &
      \\
      \vdots
      &
      &
      &
      \ddots
    \end{array}
  \right),
\end{align*}
\noindent
respectively. Similarly, \eqref{main_them_N2_T} in Theorem \ref{prop:general} is embedded as
%we consider the embedding for each matrices \(T_{n}\) for \(n\in\mathbb{N}\) as follows :
\begin{align}
%  T_{n}
%  =
%  \hbar
%  A'_{n}
%  X_{n}^{-1}
%  \mapsto
  T_{n}\left(\infty\right)
  =
  \hbar
  A'_{n}\left(\infty\right)
  X^{-1}_{n}\left(\infty\right),
  \label{T_emb_inf}
\end{align}

\noindent
where \(A'_{n}\left(\infty\right)\) and 
\(X^{-1}_{n}\left(\infty\right)\) are
%are the embedding for \(A'_{n}\) and \(X^{-1}_{n}\) such that
\begin{align*}
  A'_{n}\left(\infty\right)
  :=
  \left(
  \begin{array}{c|c}
    A'_{n} & 0 \\  \hline
    0 & 0
  \end{array}
  \right),
  \qquad
  X^{-1}_{n}\left(\infty\right)
  :=
  \left(
  \begin{array}{c|c}
    X^{-1}_{n} & 0 \\  \hline
    0 & 0
  \end{array}
  \right).
\end{align*}

\noindent
%respectively. 
%The embedding for \(X_{n}\) is carried out in the same way. \(X_{n}^{-1}\) (or \(X_{n}\)) can be a scalar matrix (e.g. \(\mathbb{C}^{2}\) and \(\mathbb{C}P^{2}\); see Section \ref{conc_ex}). However, for \(X_{n}^{-1}\) (or \(X_{n}\)), we make an exception and embed the above. 
Note that \(X_{n}^{-1}\left(\infty\right)\) is not the 
%an 
inverse matrix of \(X_{n}\left(\infty\right)\). As we saw in Theorem \ref{prop:general}, 
\(
  A'_{n}
  \in
  M_{n+1}
  \left(
    \mathbb{C}
    \left[\!
      \left[
        \hbar
      \right]\!
    \right]
  \right)
\) 
is %also 
expressed as
\begin{align*}
  A'_{n}
  =
  \left(
    \sum_{k,l=1}^{2}
    g_{\overline{k}l}
    T^{n-1}_{i-\delta_{2l},j-\delta_{2k}}
  \right)
  =
  \left(
    g_{\overline{1}1}
    T^{n-1}_{i,j}
    +
    g_{\overline{1}2}
    T^{n-1}_{i-1,j}
    +
    g_{\overline{2}1}
    T^{n-1}_{i,j-1}
    +
    g_{\overline{2}2}
    T^{n-1}_{i-1,j-1}
  \right).
\end{align*}

\noindent
%using the coefficients of \(n-1\) th order \(T^{n-1}_{i,j}.\) 
Recall %that 
%\(
%  T^{n-1}_{i-1,j},
%  \
%  T^{n-1}_{i,j-1}
%\) 
%and 
%\(
%  T^{n-1}_{i-1,j-1}
%\) 
%are shifted by the indices \(i, j\) from \(T^{n-1}_{i,j}\) depending on the K\"{a}hler metric \(g_{kl}\) and 
that \(T^{n-1}_{i,j}=0\)  if 
\(
  i<0,
  \
  i>n-1,
  \
  j<0
\) 
or 
\(
  j>n-1
\) 
by definition. %The above expression
%\(
%  A'_{n}
%  \in
%  M_{n+1}
%  \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%  \right)
%\) 
%is rewritten as
By a matrix representation
\begin{align*}
  &
  \left(
    g_{\overline{1}1}
    T^{n-1}_{i,j}
    +
    g_{\overline{1}2}
    T^{n-1}_{i-1,j}
    +
    g_{\overline{2}1}
    T^{n-1}_{i,j-1}
    +
    g_{\overline{2}2}
    T^{n-1}_{i-1,j-1}
  \right)
  \\
  &=
  g_{\overline{1}1}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  +
  g_{\overline{1}2}
  \left(
  \begin{array}{c|c}
    \mathbf{0}_{n-1}^{T} & 0 \\  \hline
    T_{n-1} & \mathbf{0}_{n-1}
  \end{array}
  \right)
  +
  g_{\overline{2}1}
  \left(
  \begin{array}{c|c}
    \mathbf{0}_{n-1} & T_{n-1} \\  \hline
    0 & \mathbf{0}_{n-1}^{T}
  \end{array}
  \right)
  +
  g_{\overline{2}2}
  \left(
  \begin{array}{c|c}
    0 & \mathbf{0}_{n-1}^{T} \\  \hline
    \mathbf{0}_{n-1} & T_{n-1}
  \end{array}
  \right)
\end{align*}

\noindent
with \(T_{n-1}\) which %that 
is the square matrix of order \(n\), % by matrix representation, 
where \(\mathbf{0}_{n-1}\) is an \(n-1\) dimensional zero vector. Since these matrices can be expressed as

\begin{align*}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  =&
  \mathrm{Id_{n+1}}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  \mathrm{Id_{n+1}},
  \\
  \left(
  \begin{array}{c|c}
    \mathbf{0}_{n-1}^{T} & 0 \\  \hline
    T_{n-1} & \mathbf{0}_{n-1}
  \end{array}
  \right)
  =&
  F_{d,n+1}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  \mathrm{Id_{n+1}},
  \\
  \left(
  \begin{array}{c|c}
    \mathbf{0}_{n-1} & T_{n-1} \\  \hline
    0 & \mathbf{0}_{n-1}^{T}
  \end{array}
  \right)
  =&
  \mathrm{Id_{n+1}}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  F_{r,n+1},
  \\
  \left(
  \begin{array}{c|c}
    0 & \mathbf{0}_{n-1}^{T} \\  \hline
    \mathbf{0}_{n-1} & T_{n-1}
  \end{array}
  \right)
  =&
  F_{d,n+1}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  F_{r,n+1},
\end{align*}

\noindent
using \(\mathrm{Id}_{n+1},\) \(F_{d,n+1}\) and \(F_{r,n+1},\) respectively, then we have

\begin{align*}
  &
  g_{\overline{1}1}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  +
  g_{\overline{1}2}
  \left(
  \begin{array}{c|c}
    \mathbf{0}_{n-1}^{T} & 0 \\  \hline
    T_{n-1} & \mathbf{0}_{n-1}
  \end{array}
  \right)
  +
  g_{\overline{2}1}
  \left(
  \begin{array}{c|c}
    \mathbf{0}_{n-1} & T_{n-1} \\  \hline
    0 & \mathbf{0}_{n-1}^{T}
  \end{array}
  \right)
  +
  g_{\overline{2}2}
  \left(
  \begin{array}{c|c}
    0 & \mathbf{0}_{n-1}^{T} \\  \hline
    \mathbf{0}_{n-1} & T_{n-1}
  \end{array}
  \right)
  \\
  &=
  g_{\overline{1}1}
  \mathrm{Id_{n+1}}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  \mathrm{Id_{n+1}}
  +
  g_{\overline{1}2}
  F_{d,n+1}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  \mathrm{Id_{n+1}}
  \\
  &
  \mbox{}
  \quad
  +
  g_{\overline{2}1}
  \mathrm{Id_{n+1}}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  F_{r,n+1}
  +
  g_{\overline{2}2}
  F_{d,n+1}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  F_{r,n+1}.
\end{align*}

\noindent
By introducing some functions 
\(
  \Theta_{\bar{\mu}}^{p},
  \Theta_{\nu}^{p}
  \in
  C^{\infty}
  \left(
    U
  \right)
  \
  \left(
    p
    \in
    \left\{
      1,
      \cdots,
      4
    \right\}
  \right)
\) 
such that 
\(
  g_{\overline{\mu}\nu}
  =
  \Theta_{\bar{\mu}}^{p}
  \Theta_{\nu}^{p},
\) 
%then 
\(A'_{n}\) can be expressed %in factorization 
%factored form 
as
\begin{align*}
  A'_{n}
  =
  \sum_{p=1}^{4}
  \left(
    \Theta_{1}^{p}
    \mathrm{Id}_{n+1}
    +
    \Theta_{2}^{p}
    F_{d,n+1}
  \right)
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  \left(
    \Theta_{\bar{1}}^{p}
    \mathrm{Id}_{n+1}
    +
    \Theta_{\bar{2}}^{p}
    F_{r,n+1}
  \right).
\end{align*}
\noindent
These 
\(
  \Theta_{\bar{\mu}}^{p}
\) 
and 
\(
  \Theta_{\nu}^{p}
\) 
play a similar role of 
%to 
``a vierbein", but not a vierbein because they are not necessarily to be orthonormal. Furthermore, by introducing the new matrices 
\(
  F^{p}_{n},
  \
  B^{p}_{n}
  \in
  M_{n+1}
  \left(
  \mathbb{C}
  \left[\!
    \left[
      \hbar
    \right]\!
  \right]
  \right)
\) 
as
%by necessary to be 
%\(
%  F^{p}_{n}
%\) 
%and 
%\(
%  B^{p}_{n}
%\) 
%as
\begin{align*}
  F^{p}_{n}
  :=
  \Theta_{1}^{p}
  \mathrm{Id}_{n+1}
  +
  \Theta_{2}^{p}
  F_{d,n+1},
  \qquad
  B^{p}_{n}
  :=
  \Theta_{\bar{1}}^{p}
  \mathrm{Id}_{n+1}
  +
  \Theta_{\bar{2}}^{p}
  F_{r,n+1}
\end{align*}
\noindent
respectively, \(A'_{n}\) is expressed as
\begin{align*}
  A'_{n}
  =
  \sum_{p=1}^{4}
  F^{p}_{n}
  \left(
  \begin{array}{c|c}
    T_{n-1} & \mathbf{0}_{n-1} \\  \hline
    \mathbf{0}_{n-1}^{T} & 0
  \end{array}
  \right)
  B^{p}_{n},
\end{align*}

\noindent
so \(A'_{n}\left(\infty\right),\) that is, the embedding matrix for \(A'_{n}\), is expressed as 
\begin{align*}
  A'_{n}\left(\infty\right)
  &=
  \sum_{p=1}^{4}
  F^{p}_{n}\left(\infty\right)
  T_{n-1}\left(\infty\right)
  B^{p}_{n}\left(\infty\right).
\end{align*}

\noindent
Here, \(F^{p}_{n}\) and \(B^{p}_{n}\) were replaced by \(F^{p}_{n}\left(\infty\right)\) and \(B^{p}_{n}\left(\infty\right)\), where
%By using \(F^{p}_{n}\left(\infty\right)\) and \(B^{p}_{n}\left(\infty\right),\) where \(F^{p}_{n}\left(\infty\right)\) and \(B^{p}_{n}\left(\infty\right)\) are the embedding for \(F^{p}_{n}\) and \(B^{p}_{n},\) that is

\begin{align}
%  F^{p}_{n}
%  \mapsto
  F^{p}_{n}\left(\infty\right)
  :=
  \Theta_{1}^{p}
  \mathrm{Id}\left(\infty\right)
  +
  \Theta_{2}^{p}
  F_{d}\left(\infty\right),
  \qquad
%  B^{p}_{n}
%  \mapsto
  B^{p}_{n}\left(\infty\right)
  :=
  \Theta_{\bar{1}}^{p}
  \mathrm{Id}\left(\infty\right)
  +
  \Theta_{\bar{2}}^{p}
  F_{r}\left(\infty\right).
  \label{emb_Fn_Bn}
\end{align}

\noindent
%respectively. 
Therefore, \(T_{n}\left(\infty\right)\) %, that is the embedding for \(T_{n}\)
%\begin{align}
%  T_{n}
%  \mapsto
%  T_{n}\left(\infty\right)
%  :=
%  \left(
%    \begin{array}{c|ccc}
%      T_{n} & & \text{\huge{0}} & \\  \hline
%       &  & & \\
%      \text{\huge{0}} & & \text{\huge{0}} & \\
%       &  & &
%    \end{array}
%  \right)
%  \label{Tn_emb}
%\end{align}
%
%\noindent
is obtained as
\begin{align*}
  T_{n}\left(\infty\right)
  =
  \hbar
  \sum_{p=1}^{4}
  F^{p}_{n}\left(\infty\right)
  T_{n-1}\left(\infty\right)
  B^{p}_{n}\left(\infty\right)
  X^{-1}_{n}\left(\infty\right).
\end{align*}
\noindent
%where \(F^{p}_{n}\left(\infty\right)\) and \(B^{p}_{n}\left(\infty\right)\) are the embedding for \(F^{p}_{n}\) and \(B^{p}_{n}\), respectively, i.e.
%\begin{align*}
%  F^{p}_{n}\left(\infty\right)
%  =
%  \Theta_{1}^{p}
%  \mathrm{Id}\left(\infty\right)
%  +
%  \Theta_{2}^{p}
%  F_{d}\left(\infty\right),
%  \
%  B^{p}_{n}\left(\infty\right)
%  =
%  \Theta_{\bar{1}}^{p}
%  \mathrm{Id}\left(\infty\right)
%  +
%  \Theta_{\bar{2}}^{p}
%  F_{r}\left(\infty\right).
%\end{align*}
By using recursively the above procedure, 
%By repeating the above procedure, 
%we obtain an explicit formula for \(T_{n}\left(\infty\right)\) :
%\begin{align}
%  T_{n}\left(\infty\right)
%  =
%  \hbar^{n}
%  \sum_{p_{1},\cdots,p_{n}=1}^{4}
%  F^{p_{n}}_{n}\left(\infty\right)
%  \cdots
%  F^{p_{1}}_{1}\left(\infty\right)
%  T_{0}\left(\infty\right)
%  \left(
%    B^{p_{1}}_{1}\left(\infty\right)
%    X^{-1}_{1}\left(\infty\right)
%  \right)
%  \cdots
%  \left(
%    B^{p_{n}}_{n}\left(\infty\right)
%    X^{-1}_{n}\left(\infty\right)
%  \right).
%  \label{main_them_N2_Tinf}
%\end{align}
%\noindent
%Hence, 
we obtain the following main theorem.

\begin{theorem}[Main result]
%  \(T_{n}\left(\infty\right)\) is given by some 
%  \(
%    F^{p_{k}}_{k}\left(\infty\right),
%    B^{p_{k}}_{k}\left(\infty\right),
%    X^{-1}_{k}\left(\infty\right)
%    \in
%    M_{\infty}
%    \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%    \right),
%  \)
%   (i.e. the embedding matrix for
%  \(
%    F^{p_{k}}_{k},
%    B^{p_{k}}_{k}
%    \in
%    M_{k+1}\left(\mathbb{C}\right)
%  \)
%  and 
%  \(
%    X_{k}^{-1}
%    \in
%    M_{k+1}
%    \left(
%    \mathbb{C}
%    \left[\!
%      \left[
%        \hbar
%      \right]\!
%    \right]
%    \right)
%  \)
%   for 
%  \(
%    k
%    =
%    1,\cdots,n
%  \)
%  )
%   the following explicit formula :
  Let \(M\) be a complex two-dimensional locally symmetric K\"{a}hler manifold, \(U\) be an open set of \(M\), and \(\ast\) be a star product with separation of variables on \(M\). 
  For 
  \(
    f,g
    \in
    C^{\infty}
    \left(U\right),
    \
    f
    \ast
    g
  \) 
  is given by
  \begin{align*}
    f
    \ast
    g
    =
    \sum_{n=0}^{\infty}
    \sum_{i,j=1}^{n+1}
    T_{ij}^{n}
    \left\{
    \left(
      D^{1}
    \right)^{n-i+1}
    \left(
      D^{2}
    \right)^{i-1}
    f
    \right\}
    \left\{
    \left(
      D^{\bar{1}}
    \right)^{n-j+1}
    \left(
      D^{\bar{2}}
    \right)^{j-1}
    g
    \right\}.
  \end{align*}
  
  \noindent
  Here %the 
  each of the coefficient 
   \(
     T_{ij}^{n}
%     =
%     T_{
%       \alpha_{2}^{n}+1,
%       \beta_{2}^{n}+1
%     }^{n}
%     =
%     T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
   \)
   is
  \begin{align*}
     {T_{n}\left(\infty\right)}_{ij}
     =
     \begin{cases}
     T_{ij}^{n}
     %=
     %T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
    &
    \
    \left(
      1
      \leq
      i,j
      \leq
      n+1
    \right)
    \\
    0
    &
    \
    \left(
      \mathrm{otherwise}
    \right)
  \end{cases}
  ,
\end{align*}

  \noindent
  and \(T_{n}\left(\infty\right)\) %uniquely 
  is determined by
  \begin{align}
  T_{n}\left(\infty\right)
  &=
  \hbar^{n}
  \sum_{p_{1},\cdots,p_{n}=1}^{4}
  F^{p_{n}}_{n}\left(\infty\right)
  \cdots
  F^{p_{1}}_{1}\left(\infty\right)
  T_{0}\left(\infty\right)
  \left(
    B^{p_{1}}_{1}\left(\infty\right)
    X^{-1}_{1}\left(\infty\right)
  \right)
  \cdots
  \left(
    B^{p_{n}}_{n}\left(\infty\right)
    X^{-1}_{n}\left(\infty\right)
  \right),
  \label{main_them_N2_Tinf}
\end{align}
   \noindent
   where %the 
   each \(F^{p_{k}}_{k}\left(\infty\right)\), \(B^{p_{k}}_{k}\left(\infty\right)\) and \(X^{-1}_{k}\left(\infty\right)\) are given as above.
   %\eqref{main_them_N2_Tinf}.% as
  \label{main_thm_N2}
\end{theorem}

\noindent
 From Theorem \ref{main_thm_N2}, we obtain %a star product with separation of variables for complex two-dimensional locally symmetric K\"{a}hler manifold. Hence, 
 a deformation quantization with separation of variables for complex two-dimensional locally symmetric K\"{a}hler manifold is realized by this star product.


==> PL/DQ.tex <==
\subsection{Deformation Quantization}

\begin{definition}
  Let 
  \(M\)
  be a Poisson manifold, 
  \(
    C^{\infty}\left(M\right)
  \)
  be a set of \(C^{\infty}\) function on \(M\),
  \(
  \left\{
    \cdot,
    \cdot
  \right\}
  :
  C^{\infty}\left(M\right)
  \times
  C^{\infty}\left(M\right)
  \to
  C^{\infty}\left(M\right)
  \)
  be a Poisson bracket, and 
  \(
    C^{\infty}
    \left(M\right)
    \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    :=
    \left\{
      f
      \middle|
      f
      =
      \sum_{k}
      f_{k}
      \hbar^{k},
      \
      f_{k}
      \in
      C^{\infty}\left(M\right)
    \right\}
  \)
  be the ring of formal power series over
  \(
    C^{\infty}\left(M\right),
  \)
   where \(\hbar\) is a formal parameter. And also, let a product \(\ast\) on
  \(
    C^{\infty}
    \left(M\right)
    \left[\!
      \left[
        \hbar
      \right]\!
    \right],
  \)
   called the star product, be a product denoted by
  \begin{align*}
    f
    \ast
    g
    =
    \sum_{k=0}^{\infty}
    C_{k}\left(f,g\right)
    \hbar^{k}
  \end{align*}
  and satisfy the following conditions:
  \begin{enumerate}
    \item
    \(\ast\)
    is associative, i.e. for any 
    \(
      f,g,h
      \in
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    \)
    , 
    \(
      f
      \ast
      \left(
        g
        \ast
        h
      \right)
      =
      \left(
        f
        \ast
        g
      \right)
      \ast
      h.
    \)
    \item
    Each 
    \(
      C_{k}
      \left(
        \cdot,
        \cdot
      \right)
      :
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
      \times
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
      \to
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    \)
    is a bi-differential operator, i.e. for any 
    \(
      f,g
      \in
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right],
    \)
    \(
      C_{k}
      \left(
        f,
        g
      \right)
    \) 
    can be written as 
    \begin{align*}
      C_{k}
      \left(
        f,
        g
      \right)
      =
      \sum_{I,J}
      a_{I,J}
      \partial^{I}
      f
      \partial^{J}
      g,
    \end{align*}
    where \(I,J\) are multi-indices.
    \item
    For any
    \(
      f,g
      \in
      C^{\infty}
      \left(M\right)
    \)
    ,
    \begin{align*}
      C_{0}
      \left(
        f,
        g
      \right)
      &=
      fg,
      \\
      C_{1}
      \left(
        f,
        g
      \right)
      -
      C_{1}
      \left(
        g,
        f
      \right)
      &=
      \left\{f,g\right\}.
    \end{align*}
    \item
    For any
    \(
      f
      \in
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right]
    \)
    ,
    \(
      f
      \ast
      1
      =
      1
      \ast
      f
      =
      f.
    \)
  \end{enumerate}
  The pair 
  \(
    \left(
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right],
      \ast
    \right)
  \) 
  is called a deformation quantization for \(M.\)
  \label{dq_def}
\end{definition}

We now consider a deformation quantization which satisfies a condition called ``separation of variables". This condition was promoted by Karabegov in \cite{Kara2} .

\begin{definition}
  Let \(M\) be a K\"{a}hlermanifold. A star product \(\ast\) on \(M\) is separation of variables if the following two conditions are satisfied for any open set \(U\) of \(M\) and 
  \(
    f
    \in
    C^{\infty}
    \left(
      U
    \right)
  \) 
  :
  \begin{enumerate}
    \item
    For a holomorphic function
    \(
      a
    \) 
    on \(U,\) 
    \(
      a
      \ast
      f
      =
      af.
    \)
    \item
    For a anti-holomorphic function 
    \(
      b
    \) 
    on \(U,\) 
    \(
      f
      \ast
      b
      =
      fb.
    \)
  \end{enumerate}
  A star product \(\ast\) that satisfies the above conditions is called a star product with separation of variables, and the deformation quantization 
  \(
    \left(
      C^{\infty}
      \left(M\right)
      \left[\!
        \left[
          \hbar
        \right]\!
      \right],
      \ast
    \right)
  \) 
  obtained from it is called a deformation quantization with separation of variables for \(M\).
  \label{sep_of_bar_starprd}
\end{definition}


==> REV/NCK2_HS.tex <==
\subsection{Deformation quantization with separation of variables for locally symmetric K\"{a}hler manifold}
\label{DQ_LSK}

\ Let \(M\) be a complex \(N\)-dimensional locally symmetric K\"{a}hler manifold, \(U\) be a holomorphic coordinate neighborhood of \(M\). For any 
\(
  f,g
  \in
  C^{\infty}
  \left(
    U
  \right),
\) 
we assume the following form for a star product with separation of variables on \(M\) by Sako-Suzuki-Umetsu \cite{SSU1,SSU2} and Hara-Sako \cite{HS1,HS2} : 
\begin{align}
  f\ast g
  =
  L_{f}g
  :=
  \sum_{n=0}^{\infty}
  \sum_{
    \overrightarrow{\alpha_{n}},
    \overrightarrow{\beta_{n}^{\ast}}
  }
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  \left(
    D^{\overrightarrow{\alpha_{n}}}f
  \right)
  \left(
    D^{\overrightarrow{\beta_{n}^{\ast}}}g
  \right).
  \label{star_expand}
\end{align}
\noindent
%%以下に示しているD^{k}およびD^{\overline{k}}はsection2で導入したので，後で削除を検討．
Here \(L_{f}\) is a left star-multiplication operator with respect to \(f\), and
\(
  D^{\overrightarrow{\alpha_{n}}},
  D^{\overrightarrow{\beta_{n}^{\ast}}}
\)
are differential operators defined by
\begin{align*}
  &
  D^{k}
  :=
  g^{k\overline{l}}
  \partial_{\overline{l}},
  \
  D^{\overline{k}}
  :=
  g^{\overline{k}l}
  \partial_{l},
  \\
  &
  D^{\overrightarrow{\alpha_{n}}}
  :=
  D^{\alpha_{1}^{n}}\cdots D^{\alpha_{N}^{n}},
  \quad
  D^{\alpha_{k}^{n}}
  :=
  \left(
    D^{k}
  \right)^{\alpha_{k}^{n}},
  \\
  &
  D^{\overrightarrow{\beta_{n}^{\ast}}}
  :=
  \overline{
    D^{\overrightarrow{\beta_{n}}}
  }
  =
  \overline{D^{\beta_{1}^{n}}}
  \cdots
  \overline{D^{\beta_{N}^{n}}},
  \quad
  \overline{D^{\beta_{k}^{n}}}
  :=
  \left(
    D^{\overline{k}}
  \right)^{\beta_{k}^{n}},
  \\
  &
  \overrightarrow{\alpha_{n}},
  \overrightarrow{\beta_{n}}
  \in
  \left\{
    \left(\gamma_{1}^{n},\cdots,\gamma_{N}^{n}\right)
    \in
    \mathbb{Z}^{N}
    \middle|
    \sum_{k=1}^{N}
    \gamma_{k}^{n}
    =
    n
  \right\},
\end{align*}
\noindent
respectively, where
\(
  \left\{
    \left(\gamma_{1}^{n},\cdots,\gamma_{N}^{n}\right)
    \in
    \mathbb{Z}^{N}
    \middle|
    \sum_{k=1}^{N}
    \gamma_{k}^{n}
    =
    n
  \right\}
\)
is a \(N\)-dimensional module such that a sum of all components is a non-negative integer \(n\). If 
there exists at least one negative 
\(
  \alpha_{k}^{n}
  \notin\mathbb{Z}_{\geq0}
\) 
for 
\(
  k
  \in
  \left\{
    1,\cdots,N
  \right\}
\), then we define 
\(
  D^{\overrightarrow{\alpha_{n}}}:=0
\). 
We define 
\(
  D^{\overrightarrow{\beta_{n}^{\ast}}}:=0
\) 
in the same way when \(\overrightarrow{\beta_{n}^{\ast}}\) has negative components. Note that \eqref{star_expand} is not a power series in the formal parameter \(\hbar\), 
%an expansion with respect to \(\hbar\), 
but a power series 
%by 
%\(
%  \left|
%    \overrightarrow{\alpha_{n}}
%  \right|
%  =
%  n
%\) 
in the differential operators 
\(
  D^{k}
\) 
and 
\(
  D^{\bar{k}}.
\)
 Since \(M\) is locally symmetric, the coefficients of the star product 
\(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
\) can be assumed to be covariantly constants.
%coefficient satisfying 
%\begin{align*}
%  &
%  \nabla_{
%    \partial_{i}
%  }
%  \left(
%    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
%    dz^{1}
%    \otimes
%    \cdots
%    \otimes
%    dz^{N}
%    \otimes
%    d\overline{z}^{1}
%    \otimes
%    \cdots
%    \otimes
%    d\overline{z}^{N}
%  \right)
%  =
%  0,
%  \\
%  &
%  \nabla_{
%    \partial_{\overline{i}}
%  }
%  \left(
%    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
%    dz^{1}
%    \otimes
%    \cdots
%    \otimes
%    dz^{N}
%    \otimes
%    d\overline{z}^{1}
%    \otimes
%    \cdots
%   \otimes
%    d\overline{z}^{N}
%  \right)
%  =
%  0.
%\end{align*}
%
%\noindent
If 
\(
  \overrightarrow{\alpha_{n}}
  \notin
  \mathbb{Z}_{\geq0}^{n}
\) 
or
\(
  \overrightarrow{\beta_{n}}
  \notin
  \mathbb{Z}_{\geq0}^{n},
\)
then we define
\(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
  :=
  0
\) 
as well as 
\(
  D^{\overrightarrow{\alpha_{n}}}
\) 
and 
\(
  D^{\overrightarrow{\beta_{n}}}
\). 
In the following discussion, we shall omit \(\ast\) when 
\(
  \overrightarrow{\beta_{n}^{\ast}}
\) 
is expressed in explicit form. %, such as 
%\(
%  \left(1,2,3\right)^{\ast}
%\). 
For example, if 
\(
  \overrightarrow{\beta_{n}^{\ast}}
  =
  \left(1,2,3\right)^{\ast},
\) 
then we denote 
\(
  \left(1,2,3\right)^{\ast}
  =
  \left(1,2,3\right)
\). 
It is known that %for 
the coefficient 
\(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
\) 
for the zeroth and first orders in 
\(
  f
  \ast
  g
\) 
are given below.

\begin{prop}[Hara-Sako\cite{HS1,HS2}]
  For a star product with separation of variables \(\ast\) on \(U,\)
  \begin{align*}
    T_{\overrightarrow{\alpha_{0}},\overrightarrow{\beta_{0}^{\ast}}}^{0}
    =
    1,
    \
    T_{\overrightarrow{e_{i}},\overrightarrow{e_{j}}}^{1}
    =
    \hbar g_{i\overline{j}},
  \end{align*}
  \noindent
  where 
  \(
    \overrightarrow{e_{i}}
    =
    \left(\delta_{1i},\cdots,\delta_{Ni}\right).
  \)
  \label{prop:covar_const_0and1}
\end{prop}

\noindent
In other words, Proposition \ref{prop:covar_const_0and1} states that for any complex \(N\)-dimensional locally symmetric K\"{a}hler manifold, the zeroth and first orders are completely determined.
%en route

\begin{theorem}[Hara-Sako\cite{HS1,HS2}]
  For 
  \(
    f,g
    \in
    C^{\infty}\left(M\right),
  \) 
  there exists %an operator \(L_{f}\) giving 
  a star product with separation of variables \(\ast\) such that
  \begin{align*}
    L_{f}
    g
    :=
    f
    \ast
    g
    =
    \sum_{n=0}^{\infty}
    \sum_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
    \left(
      D^{\overrightarrow{\alpha_{n}}}f
    \right)
    \left(
      D^{\overrightarrow{\beta_{n}^{\ast}}}g
    \right),
    \
    \left(
      f,g
      \in
      C^{\infty}
      \left(
        M
      \right)
    \right),
  \end{align*}
  \noindent
  where the coefficient 
  \(
    T_{
      \overrightarrow{\alpha_{n}},
      \overrightarrow{\beta_{n}^{\ast}}
    }^{n}
  \) 
  satisfies the following recurrence relation :
  \begin{align*}
    &
    \sum_{d=1}^{N}
    \hbar
    g_{\overline{i}d}
    T_{\overrightarrow{\alpha_{n}}-\overrightarrow{e_{d}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{i}}}^{n-1}
    \\
    &=
    \beta_{i}^{n}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
    +
    \sum_{k=1}^{N}
    \sum_{\rho=1}^{N}
    \frac{
      \hbar
      \left(\beta_{k}^{n}-\delta_{k\rho}-\delta_{ik}+1\right)
      \left(\beta_{k}^{n}-\delta_{k\rho}-\delta_{ik}+2\right)
    }{2}
    R_{\overline{\rho} \ \ \ \,\overline{i}}^{\ \,\overline{k}\,\overline{k}}
    T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}-\overrightarrow{e_{\rho}}+2\overrightarrow{e_{k}}-\overrightarrow{e_{i}}}^{n}
    \\
    &
    \mbox{}
    \quad
    +
    \sum_{k=1}^{N-1}
    \sum_{l=1}^{N-k}
    \sum_{\rho=1}^{N}
    \hbar
    \left(
      \beta_{k}^{n}
      -
      \delta_{k\rho}
      -
      \delta_{ik}
      +
      1
    \right)
    \left(
      \beta_{k+l}^{n}
      -
      \delta_{k+l,\rho}
      -
      \delta_{i,k+l}
      +
      1
    \right)
    R_{\overline{\rho} \quad \ \ \ \,\overline{i}}^{\ \,\overline{k+l}\,\overline{k}}
    T_{
      \overrightarrow{\alpha_{n}},
      \overrightarrow{\beta_{n}^{\ast}}
      -
      \overrightarrow{e_{\rho}}
      +
      \overrightarrow{e_{k}}
      +
      \overrightarrow{e_{k+l}}
      -
      \overrightarrow{e_{i}}
    }^{n}.
  \end{align*}
  \label{theorem:star_prd}
\end{theorem}

\noindent
These recurrence relations in Theorem \ref{theorem:star_prd} are equivalent to the equations (6.9) in \cite{SSU1}. Hence, from Theorem \ref{theorem:star_prd}, a star product with separation of variables on any complex \(N\)-dimensional locally symmetric K\"{a}hler manifold is obtained. However, finding a general term 
\(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
\) 
that satisfies this system of recurrence relations is not easy, except in the one-dimensional case.
%For the two-dimensional case, 
%\(
%  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
%\) 
%was only obtained for %up to 
%\(
%  n
%  =
%  0,
%  \
%  1
%\) 
%and 
%\(
%  2
%\).
% Moreover, this product gives a deformation quantization with separation of variables for locally symmetric K\"{a}hler manifold, i.e. noncommutative locally symmetric K\"{a}hler manifold.

\begin{prop}[Hara-Sako\cite{HS1,HS2}]
  Let \(M\) be a one-dimensional locally symmetric K\"{a}hler manifold, and \(U\) be an open set of \(M\). For 
  \(
    f,g
    \in
    C^{\infty}\left(U\right)
  \), 
  the star product 
  \(
    f
    \ast
    g
  \) 
  is given by
  \begin{align*}
    f
    \ast
    g
    =
    \sum_{n=0}^{\infty}
    \left[
      \left(
        g_{1\overline{1}}
      \right)^{n}
      \left\{
        \prod_{k=1}^{n}
        \frac{4\hbar}{4k+\hbar k\left(k-1\right)R}
      \right\}
      \left\{
        \left(
        g^{1\overline{1}}
        \frac{\partial}{\partial \overline{z}}
      \right)^{n}
      f
      \right\}
      \left\{
        \left(
        g^{1\overline{1}}
        \frac{\partial}{\partial z}
        g
      \right)^{n}
      \right\}
    \right],
  \end{align*}
  where 
  \(
    R
    =
    2
    R_{\overline{1} \ \ \, \overline{1}}^{\ \, \overline{1}\overline{1}}
  \)
  is the scalar curvature on \(M\).
  \label{prop:cplx_1}
\end{prop}

\noindent
Note that Proposition \ref{prop:cplx_1} is corrected 
%revised 
some errata for the one-dimensional formula in \cite{HS1,HS2}. This proposition can be shown by direct calculations %, 
since the recurrence relation is a simple expression in the one-dimensional case.
\bigskip
\\
\ On the other hand,  
\(
  T_{\overrightarrow{\alpha_{n}},\overrightarrow{\beta_{n}^{\ast}}}^{n}
\) 
were 
%was 
only obtained for %up to 
\(
  n
  =
  0,
  \
  1
\) 
and 
\(
  2
\) 
for the two-dimensional case. The following proposition is shown by directly solving the recurrence relation in Theorem \ref{theorem:star_prd} for \(n=2\).

\begin{prop}[Hara-Sako\cite{HS1,HS2}]
  Let \(M\) be a complex two-dimensional locally symmetric K\"{a}hler manifold. Then the coefficients 
  \(
    T_{\overrightarrow{\alpha_{2}},\overrightarrow{\beta_{2}^{\ast}}}^{2}
  \)  
  are given by% :
  \begin{align*}
    \left(
      T^{2}_{ij}
    \right)
    =
    \hbar^{2}
    A_{2}
    X_{2}^{-1},
  \end{align*}
  
  \noindent
  where
  \begin{align*}
    &
    T^{2}_{ij}
    :=
    T_{
      \left(
        3-i,
        i-1
      \right),
      \left(
        3-j,
        j-1
      \right)
    }^{2},
    \\
    &
    A_{2}
    :=
    \left(
      \begin{array}{ccc}
        \left(
          g_{\bar{1}1}
        \right)^{2}
        &
        g_{\bar{1}1}
        g_{\bar{2}1}
        &
        \left(
          g_{\bar{2}1}
        \right)^{2}
        \\
        2
        g_{\bar{1}1}
        g_{\bar{1}2}
        &
        g_{\bar{1}2}
        g_{\bar{2}1}
        +
        g_{\bar{1}1}
        g_{2\bar{2}}
        &
        2
        g_{\bar{2}1}
        g_{\bar{2}2}
        \\
        \left(
          g_{\bar{1}2}
        \right)^{2}
        &
        g_{\bar{2}1}
        g_{\bar{2}2}
        &
        \left(
          g_{\bar{2}2}
        \right)^{2}
      \end{array}
    \right),
    \\
    &
    X_{2}
    :=
    \left(
      \begin{array}{ccc}
        2
        +
        \hbar
        R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
        &
        \hbar
        R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{1}\bar{1}}
        &
        \hbar
        R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{1}\bar{1}}
        \\
        \hbar
        R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
        &
        1
        +
        \hbar
        R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{1}}
        &
        \hbar
        R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{1}}
        \\
        \hbar
        R_{\bar{1} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
        &
        \hbar
        R_{\bar{2} \ \ \, \bar{1}}^{\ \, \bar{2}\bar{2}}
        &
        2
        +
        \hbar
        R_{\bar{2} \ \ \, \bar{2}}^{\ \, \bar{2}\bar{2}}
      \end{array}
    \right).
  \end{align*}
  \label{prop:n2}
\end{prop}

\noindent
We have reviewed the previous works. In general, solving recurrence relations is not easy. In particular, when we attempt to obtain the general term using a matrix representation, we need a square matrix of order \(n+1\). In addition, the matrix size increases with increasing order. Therefore, it had been considered difficult to obtain the general term. In this paper, we find that the expression of the general term does not become unlimitedly complex, and succeed in getting the general term by using this fact. We shall see that in the following sections. In Section \ref{NEW_RESULT}, we are going to describe the coefficients 
\(
  T_{
    \overrightarrow{\alpha_{n}},
    \,
    \overrightarrow{\beta_{n}^{\ast}}
  }^{n}
\) 
for any \(n\in\mathbb{Z}_{\geq0}\).
%The concrete expressions for the coefficient 
%\(
%  T_{
%    \overrightarrow{\alpha_{n}},
%    \,
%    \overrightarrow{\beta_{n}^{\ast}}
%  }^{n}
%\) 
%given by Hara-Sako \cite{HS1,HS2} are only 
%\(
%  T_{
%    \overrightarrow{\alpha_{0}},
%    \,
%    \overrightarrow{\beta_{0}^{\ast}}
%  }^{0},
%  \
%  T_{
%    \overrightarrow{\alpha_{1}},
%    \,
%    \overrightarrow{\beta_{1}^{\ast}}
%  }^{1}
%\) 
%and 
%\(
%  T_{
%    \overrightarrow{\alpha_{2}},
%    \,
%    \overrightarrow{\beta_{2}^{\ast}}
%  }^{2}
%\) 
%for complex two-dimensional case.


==> REV/NCK2_History.tex <==
\subsection{%Historical background
%Background of 
Noncommutative K\"{a}hler manifolds}
\label{NCK_History}

%\ Berezin was proposed by a general definition of quantization and construct the quantization of K\"{a}hler manifolds in the case of phase space via symbol algebras \cite{Bere1,Bere2}.
\ Berezin proposed a general definition of quantization and constructed the quantization of K\"{a}hler manifolds in the case of phase space via symbol algebras \cite{Bere1,Bere2}.  
%Several reviews have been published on Berezin-Toeplitz quantization. See \cite{KS1,Schli1,Schli2,Schli3,Schli4,Schli5,Schli6} for more detail. After that, The construction method of noncommutative K\"{a}hler manifolds was studied via the deformation quantization with separation of variables by Karabegov \cite{Kara1,Kara2}. 
The coherent states of K\"{a}hler manifolds arising from the geometric quantization of Kostant \cite{Kos} and Souriau \cite{Sou} have also been studied by Rawnsley \cite{Rawn}. It is known that this coherent state is related to Berezin quantization. See \cite{Pere} for more detail. 
%After that, the quantization of some K\"{a}hler manifolds by using a deformation quantization has been provided by Moreno \cite{Mor1,Mor2}. 
After that, the deformation quantization of K\"{a}hler manifolds have been provided by Moreno \cite{Mor1,Mor2} and Omori-Maeda-Miyazaki-Yoshioka \cite{OMMY}. The relations between deformation quantization and Berezin quantization have been studied by Cahen-Gutt-Rawnsley \cite{CGR1,CGR2,CGR3,CGR4}. 
%It has also studied the quantization of K\"{a}hler manifolds via T-quantization by Bordemann et al. \cite{BMS}. 
It has also studied the quantization of K\"{a}hler manifolds via Toeplitz quantization by Bordemann et al. \cite{BMS}. 
%Furthermore, Karabegov and Schlichenmaier have been provided Berezin-Toeplitz quantization in the case of compact K\"{a}hler ones \cite{Schli1,Schli2,Schli3,Schli4,Schli5,Schli7}. These previous works related to Berezin-Toeplitz quantizations for K\"{a}hler manifolds were reviewed by Schlichenmaier. See \cite{Schli6} for more detail. 
Furthermore, Karabegov and Schlichenmaier have provided Berezin-Toeplitz quantization in the case of compact K\"{a}hler ones \cite{Schli1,Schli2,Schli3,Schli4,Schli5,Schli7}. These previous works related to Berezin-Toeplitz quantizations for K\"{a}hler manifolds were reviewed by Schlichenmaier \cite{Schli6}. 
%From another angle of the quantization, the construction method of noncommutative K\"{a}hler manifolds was studied via the deformation quantization with separation of variables by Karabegov \cite{Kara1,Kara2}. 
From the other angle of the quantization, the construction method of noncommutative K\"{a}hler manifolds was studied via the deformation quantization with separation of variables by Karabegov \cite{Kara1,Kara2}. 
%In \cite{OMMY}, Omori-Maeda-Miyazaki-Yoshioka were given the deformation quantization for K\"{a}hler manifolds from their construction method in \cite{OMY1}. 
%Furthermore, for any noncommutative K\"{a}hler manifolds obtained by Karabegov's construction, Sako-Umetsu was constructed Fock representations of them \cite{SU1,SU2}. In this paper, we review a Karabegov's method and Fock representations of noncommutative K\"{a}hler manifolds by Sako-Umetsu.
Moreover, for any noncommutative K\"{a}hler manifolds obtained by Karabegov's construction, Sako-Umetsu constructed Fock representations of them \cite{SU1,SU2}. In this subsection, we review %a 
Karabegov's method and Fock representations of noncommutative K\"{a}hler manifolds by Sako-Umetsu.
%And for any noncommutative K\"{a}hler manifolds constructed via deformation quantization with separation of variables, Sako-Umetsu was constructed Fock representations of them \cite{SU1,SU2}. In this paper, we review a Karabegov's method and Fock representations of noncommutative K\"{a}hler manifolds by Sako-Umetsu.\\
%%以下Open bookのものを引用しているので，適宜文章を書き換えること．
\bigskip
\\
\ Let \(M\) be an \(N\)-dimensional K\"ahler manifold and 
\(
  U
  \subset
  M
\) be a holomorphic coordinate neighborhood of \(M\). We choose a local holomorphic coordinates by \(\left(z^{1},\cdots,z^{N}\right)\). For a K\"{a}hler manifolds, a K\"{a}hler 2-form \(\omega\) and a K\"{a}hler metric \(g\) can be locally expressed by using a K\"{a}hler potential \(\Phi\) as follows:
\begin{align*}
  \omega
  =
  i
  g_{k\bar{l}}
  dz^{k}
  \wedge
  d\bar{z}^{l},
  \qquad
  g_{k\bar{l}}
  =
  \frac{
    \partial^2
    \Phi
  }{
    \partial
    z^{k}
    \partial
    \bar{z}^{l}
  }.
\end{align*}
\noindent
Note that we use the Einstein summation convention on the above. We also denote the inverse matrix of \(\left(g_{\overline{k}l}\right)\) by \(\left(g^{\overline{k}l}\right)\). Here we introduce the differential operators
\(
  D^{k},
  D^{\overline{k}}
\) 
defined by
\begin{align*}
  &
  D^{k}
  :=
  g^{k\overline{l}}
  \partial_{\overline{l}},
  \quad
  D^{\overline{k}}
  :=
  g^{\overline{k}l}
  \partial_{l}.
\end{align*}
\noindent
%And we 
We define the set of differential operators 
\begin{align*}
  {\mathcal S}
  :=
  \left\{ 
    A
    \middle|
    A
    =
    \sum_{\alpha}
    a_{\alpha}
    D^{\alpha},
    \,
    a_{\alpha}
    \in
    C^{\infty}
    \left(U\right)
  \right\},
\end{align*}
\noindent
where 
\(
  \alpha
  =
  \left(
    \alpha_{1},
    \dots,
    \alpha_{N}
  \right)
\) is a multi-index% and
, i.e. 
\(
  D^{\alpha}
  :=
  \left(
    D^{\bar{1}}
  \right)^{\alpha_{1}}
  \cdots
  \left(
    D^{\bar{N}}
  \right)^{\alpha_{N}}
\). 
%\begin{theorem}[Karabegov\cite{Kara1}]
%  Let 
%  \(
%  D^{k},
%  \
%  D^{\overline{k}}
%  \) 
%  be the differential operators, and \(\Phi\) be the K\"{a}hler potential of \(U\). For \(k,l\in\left\{1,\cdots,N\right\}\), 
%  \(
%  D^{k}
%  \) 
%  and 
%  \(
%  D^{\overline{k}}
%  \) 
%  satisfy the following commutation relations:
%  \begin{align*}
%    \left[
%      D^{\overline{k}},
%      D^{\overline{l}}
%    \right]
%    =
%    0,
%    \quad
%    \left[
%      D^{\overline{k}},
%      \partial_{\overline{l}}
%      \Phi
%    \right]
%    =
%    {\delta^{\overline{l}}}_{\overline{m}},
%    \\
%    \left[
%      D^{k},
%      D^{l}
%    \right]
%    =
%    0,
%    \quad
%    \left[
%      D^{k},
%      \partial_{l}
%      \Phi
%    \right]
%    =
%    {\delta^{l}}_{m}.
%  \end{align*}
%  \label{thm_D_comm_rel}
%\end{theorem}
%\noindent
%By using Theorem \ref{thm_D_comm_rel}, we 
We can construct the left star-multiplication operator \(L_{f}\) for 
\(
  f
  \in
  C^{\infty}
  \left(U\right)
\) 
such that 
\(
  L_{f}
  g
  :=
  f
  \ast
  g
\)%.
:
\begin{theorem}[Karabegov\cite{Kara1}]
Let \(M\) be an \(N\)-dimensional K\"{a}hler manifold, \(U\) be a %holomorhpic
holomorphic coordinate neighborhood on \(M\), % \(\omega\)
and \(\omega\) be a K\"{a}hler form on \(M\). % and 
%\(
%  f,g
%  \in
%  C^{\infty}
%  \left(U\right)
%\). 
Then, there is %uniquely 
the left star-multiplication operator
\begin{align*}
  L_{f}
  =
  \sum_{n=0}^{\infty}
  \hbar^{n}
  A_{n},
  \qquad
  f
  \in
  C^{\infty}
  \left(U\right),
\end{align*}
where 
\(
  A_{n}
  :=
  a_{n,\alpha}\left(f\right)
  D^{\alpha}
  \in
  \mathcal{S}
\) 
are differential operators whose coefficients
\(
  a_{n,\alpha}\left(f\right)
  \in
  C^{\infty}
  \left(U\right)
\) 
 depend on \(f\).
%satisfying 
\(L_{f}\) is determined by the following conditions:
\begin{enumerate}
\item
\(
  \left[
    L_{f},
    R_{\partial_{\overline{l}}\Phi}
  \right]
  =
  0
\), 
where 
\(
  R_{\partial_{\overline{l}}\Phi}
  =
  \partial_{\overline{l}}\Phi
  +
  \hbar
  \partial_{\overline{l}}
\),
\item
\(
  L_{f}1
  =
  f
  \ast
  1
  =
  f
\),
\item
For any 
%\(
%  h
%  \in
%  C^{\infty}
%  \left(U\right)
%\)
\(
  g,h
  \in
  C^{\infty}
  \left(U\right)
\), 
the left star-multiplication operator is associative, i.e. 
\begin{align*}
  L_{f}
  \left(
    L_{g}
    h
  \right)
  =
  f
  \ast
  \left(
    g
    \ast
    h
  \right)
  =
  \left(
    f
    \ast
    g
  \right)
  \ast
  h
  =
  L_{
    L_{f}g
  }
  h%,
  .
\end{align*}
\end{enumerate}
%where 
%\(
%  A_{n}
%  :=
%  a_{n,\alpha}\left(f\right)
%  D^{\alpha}
%  \in
%  \mathcal{S}
%\) 
%are differential operators whose each coefficient
%\(
%  a_{n,\alpha}\left(f\right)
%  \in
%  C^{\infty}
%  \left(U\right)
%\) 
% depends on \(f\).
\label{thm_Kara_star_opr}
\end{theorem}
\noindent
%If multi-index \(\alpha\) is fixed, each \(A_{n}\) is uniquely determined by the commutativity of \(D^{\overline{i}}\). We can also construct the right star-multiplication operator \(R_{g}\) for 
%\(
%  g
%  \in
%  C^{\infty}
%  \left(U\right)
%\) 
%which is defined by 
%\(
%  R_{g}f
%  :=
%  f
%  \ast
%  g
%\). 
%It is determined by the following conditions:
%\begin{align*}
%  \left[
%    R_{g},
%    L_{\partial_{l}\Phi}
%  \right]
%  =
%  0,
%  \quad
%  R_{g}1
%  =
%  1
%  \ast
%  g
%  =
%  1,
%\end{align*}
%\noindent
%where 
%\(
%  L_{\partial_{l}\Phi}
%  = 
%  \partial_{l}\Phi
%  +
%  \hbar
%  \partial_{l}
%\). 
%These star-multiplication operators are explicitly given by the following proposition.
%\begin{prop}
%Let \(L_{f}\) and \(R_{f}\) be the left and right star-multiplication operators for 
%\(
%  f
%  \in
%  C^{\infty}
%  \left(U\right)
%\), 
%respectively. Then, these operators are given by
%\begin{align*}
%  L_{f}
%  &=
%  \sum_{\alpha}
%  \frac{1}{\alpha !}
%  \left\{
%    \left(
%      \frac{
%        \partial
%      }{
%        \partial
%        \overline{z}
%      }
%    \right)^{\alpha}
%    f
%  \right\}
%  \left(
%    L_{\overline{z}}
%    -
%    \overline{z}
%  \right)^{\alpha},
%  \\
%  R_{f}
%  &=
%  \sum_{\alpha} \frac{1}{\alpha!}
%  \left\{
%    \left(
%      \frac{
%        \partial
%      }{
%        \partial
%        z
%      }
%    \right)^{\alpha}
%    f
%  \right\}
%  \left(
%    R_{z}
%    -
%    z
%  \right)^{\alpha},
%\end{align*}
%where 
%\(
%  L_{\overline{z}}
%  :=
%  \left(
%    L_{\overline{z}^{1}},
%    \cdots,
%    L_{\overline{z}^{N}}
%  \right)
%\) 
%and 
%\(
%  \bar{z}
%  :=
%  \left(
%    \overline{z}^{1},
%    \cdots,
%    \overline{z}^{N}
%  \right)
%\).
%\label{Kara_left_right_star_oprs}
%\end{prop}
%\noindent
%For the star product with separation of variables, it has the property under the complex conjugate.
%\begin{prop}
%\begin{align}
%  \overline{L_{f}g}
%  =
%  \overline{
%    f
%    \ast
%    g
%  }
%  =
%  \overline{g}
%  \ast
%  \overline{f}.
%\end{align}
%\label{star_cplx_conj}
%\end{prop}
%See Proposition 3.1. in \cite{SU1} for more detailed proof of it. 
By using the definition of the separation of variables and the commutation relations of the star-multiplication operators, we obtain the following commutation relations 
%with respect to 
concerning \(z^{i}\), \(\overline{z}^{i}\), \(\partial_{i}\Phi\) and \(\partial_{\overline{i}}\Phi\).
\begin{align}
  \left[
    \frac{1}{\hbar} 
    \partial_{i}
    \Phi,
    z^{j}
  \right]_{\ast}
  &=
  \delta_{ij}, 
  \qquad
  \left[
    z^{i},
    z^{j}
  \right]_{\ast}
  =
  0,
  \qquad
  \left[
    \partial_{i}
    \Phi,
    \partial_{j}
  \Phi
  \right]_{\ast}  
  =
  0
  \label{star_comm_rel_1}
  \\
  \left[
    \overline{z}^{i},
    \frac{1}{\hbar}
    \partial_{\overline{j}}
    \Phi
  \right]_{\ast}
  &=
  \delta_{ij},
  \qquad
  \left[
    \overline{z}^{i},
    \overline{z}^{j}
  \right]_{\ast}
  =
  0,
  \qquad
  \left[
    \partial_{\overline{i}}
    \Phi,
    \partial_{\overline{j}}
    \Phi
  \right]_{\ast}
  =
  0.
  \label{star_comm_rel_2}
\end{align}
\noindent
Note that the commutator \(\left[\cdot,\cdot\right]_{\ast}\) is defined by 
\(
  \left[
    A,B
  \right]_{\ast}
  :=
  A
  \ast
  B
  -
  B
  \ast
  A
\). 
%These relations \eqref{star_comm_rel_1} and \eqref{star_comm_rel_2} are similar to canonical commutation relation with respect to creation and annihilation operators in quantum theory. So we can regard the sets
%\begin{align}
%  &\left\{
%    z^{i},
%    \partial_{i}\Phi
%    \middle|
%    i=1,\cdots,N
%  \right\},
%  \label{cre_ann_set_1}
%  \\
%  &\left\{
%    z^{\overline{i}},
%    \partial_{\overline{i}}\Phi
%    \middle|
%    i=1,\cdots,N
%  \right\}
%  \label{cre_ann_set_2}
%\end{align}
%\noindent
%as the set of creation and annihilation operators under the star product \(\ast\), respectively. On the other hand,
%\begin{align*}
%  \left\{
%    z^{i},
%    \partial_{i}\Phi,
%    z^{\overline{i}},
%    \partial_{\overline{i}}\Phi
%    \middle|
%    i=1,\cdots,N
%  \right\}
%\end{align*}
%\noindent
%is not the set of creation and annihilation operators since operators in \eqref{cre_ann_set_1} do not commute with ones in \eqref{cre_ann_set_2}. In fact, \(z^{i}\) and \(\overline{z}^{j}\) are noncommutative from 
%\(
%  z^{i}
%  \ast
%  \overline{z}^{j}
%  \neq
%  \overline{z}^{j}
%  \ast
%  z^{i}
%\). 
Here, we introduce the creation and annihilation operators %in \eqref{cre_ann_set_1} and \eqref{cre_ann_set_2} 
as follows:
\begin{align}
  a^{\dagger}_{i}
  =
  z^{i},
  \qquad
  \underline{a}_{i}
  =
  \frac{1}{\hbar}
  \partial_{i}
  \Phi,
  \qquad
  a_{i}
  =
  \bar{z}^{i},
  \qquad
  \underline{a}_{i}^{\dagger}
  =
  \frac{1}{\hbar}
  \partial_{\bar{i}}
  \Phi
  \qquad
  \left(
    i=1,\cdots,N
  \right).
  \label{cre_ann_Kahler}
\end{align}
\noindent
Then, the commutation relations \eqref{star_comm_rel_1} and \eqref{star_comm_rel_2} can be rewritten as
\begin{align}
  \left[
    \underline{a}_{i},
    a^{\dagger}_{j}
  \right]_{\ast}
  &=
  \delta_{ij}, 
  \qquad
  \left[
    a^{\dagger}_{i},
    a^{\dagger}_{j}
  \right]_{\ast}
  =
  0,
  \qquad
  \left[
    \underline{a}_{i},
    \underline{a}_{j}
  \right]_{\ast}  
  =
  0
  \label{star_comm_rel_CA_1}
  \\
  \left[
    a_{i},
    \underline{a}_{j}^{\dagger}
  \right]_{\ast}
  &=
  \delta_{ij},
  \qquad
  \left[
    a_{i},
    a_{j}
  \right]_{\ast}
  =
  0,
  \qquad
  \left[
    \underline{a}_{i}^{\dagger},
    \underline{a}_{j}^{\dagger}
  \right]_{\ast}
  =
  0.
  \label{star_comm_rel_CA_2}
\end{align}
\noindent
Since 
\(
  \left[
    a_{i},
    a_{i}^{\dagger}
  \right]_{\ast}
  \neq
  0
\), 
\(
  \left[
    \underline{a}_{i},
    \underline{a}_{j}^{\dagger}
  \right]_{\ast}
  \neq
  0
\) 
in general, these relations are slightly different from the ordinary canonical commutation relation. From the %sets \eqref{cre_ann_set_1} and \eqref{cre_ann_set_2}
above operators, the (twisted) Fock space is defined by a vector space spanned by the basis
\begin{align}
  |{\vec{n}}\rangle
  =
  |n_{1},\cdots,n_{N}\rangle
  =
  %c_{1}\left(\vec{n}\right)
  \frac{1}{
    \sqrt{
      \vec{n}!
    }
  }
 {\left(a^{\dagger}_{1}\right)}_{\ast }^{n_{1}}
 \ast
 \cdots
 \ast
 {\left(a^{\dagger}_{N}\right)}_{\ast }^{n_{N}}
 \ast  
 |\vec{0}\rangle,
 \label{twFock_base_n}
\end{align}
\noindent
where a vacuum 
\(
  |{\vec{0}}\rangle
  =
  |0,\cdots,0\rangle 
\) 
is the vector such that
\begin{align}
  \underline{a}_{i}
  \ast
  |{\vec{0}}\rangle
  =
  0,
  \qquad
  (i=1,\cdots,N),
  \label{twFock_vac_n}
\end{align}
\noindent
%and \(c_{1}\left(\vec{n}\right)\) is a normalization constant. 
and  
\(
  \vec{n}!
  =
  n_{1}!
  \cdots
  n_{N}!
\). 
Note that 
\(
  \left(A\right)_{\ast}^{n}
\) 
is the product of multiplying \(n\) by the star product \(\ast\), i.e. 
\(
  \left(A\right)_{\ast}^{n}
  :=
  \underbrace{
    A
    \ast
    \cdots
    \ast
    A
  }_{
    n
    \
    \rm{
      times
      \
      by
    }
    \
    \ast
  }
\). Similarly, the dual basis for \(|{\vec{n}}\rangle\) is defined by
\begin{align}
  \underline{\langle{\vec{m}}|}
  =
  \underline{
    \langle
    m_{1},
    \cdots,
    m_{N}|
  }
  =
  \langle
  \vec{0}|
  \ast
  \left(\underline{a}_{1}\right)_{\ast }^{m_{1}}
  \ast
  \cdots
  \ast  
  \left(\underline{a}_{N}\right)_{\ast }^{m_{N}} 
  %c_{2}\left(\vec{m}\right),
  \frac{1}{
    \sqrt{
      \vec{m}!
    }
  },
 \label{twFock_dbase_m}
\end{align}
\noindent
where \(\langle\vec{0}|\) is the (dual) vector for a vacuum \(|{\vec{0}}\rangle\) such that
\begin{align}
  \langle
  \vec{0}|
  \ast 
  a_{i}^{\dagger}
  =
  0,
  \qquad
  (i=1,\cdots,N),
\end{align}
\noindent
%and \(c_{2}\left(\vec{m}\right)\) is the normalized constant. 
and 
\(
  \vec{m}!
  =
  m_{1}!
  \cdots
  m_{N}!
\).
Note that \(\underline{\langle{\vec{m}}|}\) does not imply Hermitian conjugate of \(|{\vec{m}}\rangle\), i.e. 
\(
  \underline{\langle{\vec{m}}|}
  \neq
  |{\vec{m}}\rangle^{\dagger}
\).% In this paper, we set each normalization constant as follows:
%\begin{align}
%  c_{1}\left(\vec{n}\right)
%  =
%  \frac{1}{
%    \sqrt{
%      \vec{n}!
%    }
%  },
%  \qquad
%  c_{2}\left(\vec{m}\right)
%  =
%  \frac{1}{
%    \sqrt{
%      \vec{m}!
%    }
%  },
%  \label{twFock_norm_const}
%\end{align}
%\noindent
%where 
%\(
%  \vec{n}!
%  =
%  n_{1}!
%  \cdots
%  n_{N}!
%\), 
%\(
%  \vec{m}!
%  =
%  m_{1}!
%  \cdots
%  m_{N}!
%\).
\begin{definition}
Let \(M\) be a K\"{a}hler manifold and \(U\) be a holomorphic coordinate neighborhood on \(M\). Then, the (local) twisted Fock algebra (representation) \(F_{U}\) is defined by
\begin{align}
  F_{U}
  :=
  \left\{
    \sum_{\vec{n},\vec{m}}
    A_{\vec{n}\vec{m}}
    |\vec{n}\rangle
    \underline{\langle\vec{m}|}
    \middle|
    A_{
      \vec{n}
      \vec{m}
    }
    \in
    \mathbb{C}
  \right\}.
\end{align}
\label{twFock_def}
\end{definition}
\noindent
\(F_{U}\) is defined as the algebra which is given by the creation and annihilation operators in \eqref{cre_ann_Kahler} and star-multiplication between each element of \(F_{U}\). Moreover, we can concretely express the coefficient functions \(A_{\vec{n}\vec{m}}\) which are the elements of \(F_{U}\). 
%\begin{lemma}[Berezin]
%For any K\"{a}hler manifolds \(M\), there is a K\"ahler potential 
%\(
%  \Phi
%  \left(
%    z,
%    \overline{z}
%  \right)
%\) 
%such that
%\begin{align}
%  \Phi
%  \left(
%    \mathbf{0},
%    \overline{z}
%  \right)
%  =
%  \Phi
%  \left(
%    z,
%    \mathbf{0}
%  \right)
%  =
%  0.
%  \label{Phi_cond}
%\end{align}
%\label{lem_Bere_potential}
%\end{lemma}
%ここまで書き換え済
%This is easily shown as follow.
%In the following, we abbreviate 
%$\Phi (z^1,\dots ,z^N , \bar{z}^1 , \dots , \bar{z}^N)$ to 
%$\Phi(z,\bar{z})$ for convenience.
%If a K\"ahler potential $\Phi$ satisfying 
%$g_{i\bar{j}} = \partial_i \partial_{\bar j} \Phi$
%does not satisfy (\ref{Phi_cond}),
%then we redefine a new K\"ahler potential $\Phi'$ as
%\begin{align}
%\Phi'(z , \bar{z}) := 
%\Phi (z , \bar{z})
%-\Phi( 0 , \bar{z}) 
%- \Phi (z , 0 ) +  \Phi (0 , 0 ).
%\end{align}
%$\Phi (z , 0 ) $ is a holomorphic function and
%$\Phi( 0 , \bar{z}) $ is an
%anti-holomorphic function.
%K\"ahler potentials have ambiguities of adding holomorphic and
%anti-holomorphic functions.
%This $\Phi'$ satisfies the condition (\ref{Phi_cond}).
%
% 
%
%In \cite{Sako:2012ws}, it is shown that $e^{-\Phi/\hbar}$ corresponds to
%a vacuum projection operator $ |\vec{0} \rangle \langle \vec{0}| $ for
%the noncommutative ${\mathbb C}P^N$.  We extend this statement for
%general K\"ahler manifolds.
%\begin{prop}
%Let $(M, \omega)$ be a K\"ahler manifold, $\Phi$ be its K\"ahler
% potential with the property (\ref{Phi_cond}), and
%$\ast $ be a star product with separation of variables given
%in the previous section.
%Then the function
%\begin{equation}
% |\vec{0} \rangle \langle \vec{0}| := e^{-\Phi/\hbar},
%\end{equation}
%satisfies
%\begin{align}
% & \underline{a}_i \ast  |\vec{0} \rangle \langle \vec{0}| 
% = 0, \qquad
% |\vec{0} \rangle \langle \vec{0}| \ast  a_i^\dagger 
%= 0, \\
% & \left(|\vec{0} \rangle \langle \vec{0}|\right) \ast  
% \left(|\vec{0} \rangle \langle \vec{0}|\right) =
% e^{-\Phi/\hbar}\ast e^{-\Phi/\hbar} = e^{-\Phi/\hbar}
% = |\vec{0} \rangle \langle \vec{0}|.
%\end{align}
%\end{prop}
%
%{\bf Overview of proof} 
%~(A more detailed proof is given in \cite{Sako:2016gqb}.)\\
%We define the following normal ordered quantity,
%\begin{align}
%: e^{- \sum_i a_i^{\dagger} \underline{a}_i} : ~ 
% := {\prod_{i=1}^N}_\ast  \sum_{n=0}^{\infty} 
% \frac{(-1)^n}{n!} (a_i^{\dagger})_\ast ^n \ast  (\underline{a}_i)^n_\ast .
%\end{align}
%Here ${\prod_{i=1}^N}_\ast  $ is defined by
%${\prod_{i=1}^N}_\ast  f_i = f_1 \ast  f_2 \ast  \cdots \ast  f_N$.\\
%It is easy to show that
%$ \underline{a}_i \ast  \sum_{n=0}^{\infty} \frac{(-1)^n}{n!} 
%(a_i^{\dagger})_\ast ^n \ast  (\underline{a}_i)^n_\ast  = 0$,
%
%It is easy to show that 
%$: e^{- \sum_i a_i^{\dagger} \underline{a}_i} : 
%= | \vec{0} \rangle \langle \vec{0} |$
%in the same way as in the case of the ordinary harmonic oscillator,
%\begin{align}
%\underline{a}_i \ast  \sum_{n=0}^{\infty} \frac{(-1)^n}{n!} 
%(a_i^{\dagger})_\ast ^n \ast  (\underline{a}_i)^n_\ast  
%& =  \sum_{n=0}^{\infty} \frac{(-1)^n}{n!}  
% \left[ n (a_i^{\dagger})_\ast ^{n-1} (\underline{a}_i)_\ast ^n 
% + (a^{\dagger})_\ast ^n (\underline{a})_\ast ^{n+1}
% \right]
%= 0,
%\end{align}
%where the commutation relations (\ref{comm-rel-1+1}) are used.
%Similarly, we can show 
%$ \sum_{n=0}^{\infty} \frac{(-1)^n}{n!} 
%(a_i^{\dagger})_\ast ^n \ast  (\underline{a}_i)^n_\ast  \ast  a_i^\dagger = 0 $. 
%These results and the fact that $\underline{a}_i$ and $a_i^{\dagger}$
%commute with $\underline{a}_j$ and $a_j^{\dagger}$ for $ i\neq j$ lead to 
%$ \underline{a}_i \ast  : e^{-  \sum_i a_i^{\dagger} \underline{a}_i} : = 0$
% and  
% $ : e^{- \sum_i a_i^{\dagger} \underline{a}_i} : \ast  a_i^\dagger = 0 $. 
% Further, these relations imply 
%$: e^{- \sum_i a_i^{\dagger} \underline{a}_i} : \ast  
%: e^{- \sum_i a_i^{\dagger} \underline{a}_i} :
% ~=~ : e^{- \sum_i a_i^{\dagger} \underline{a}_i} :$.\\
%Therefore, all we have to do is to show
%\begin{align}
%: e^{-  \sum_i a_i^{\dagger} \underline{a}_i} : = e^{-\Phi/\hbar}.
%\end{align}
%This can be done as follows:
%\begin{align}
%: e^{- \sum_i a_i^{\dagger} \underline{a}_i} : 
% &= \sum_{\vec{n}} \frac{(-1)^{|n|}}{\vec{n}!} 
% (a^\dagger)_\ast ^{\vec{n}} \ast  (\underline{a})_\ast ^{\vec{n}} \nonumber \\
% &= \sum_{\vec{n}} \frac{(-1)^{|n|}}{\vec{n}! \hbar^{|n|}} 
% (z)_\ast ^{\vec{n}} \ast  (\partial \Phi)_\ast ^{\vec{n}}.
%&= \sum_{n=0}^{\infty}  \sum_{n_1  + \dots + n_N = n} 
%\!\!\!\!\!\!\!\! \frac{(-1)^{n}}{n_1 ! n_2 ! \cdots n_N!} 
%(a_1^{\dagger})^{n_1}_\ast  \ast  (a_2^{\dagger})^{n_2}_\ast  \ast  \cdots \ast  
%(a_N^{\dagger})^{n_N}_\ast   \ast  
%(\underline{a}_1)^{n_1}_\ast  \ast  (\underline{a}_2)^{n_2}_\ast  \ast  \cdots \ast  
% (\underline{a}_N)^{n_N}_\ast    \nonumber \\
%&= \sum_{n=0}^{\infty}  \sum_{n_1 + \dots + n_N=n} 
%\!\!\!\!\!\!\!\! \frac{(-1)^{n}}{n_1 ! n_2 ! \cdots n_N! \hbar^{n_i}} 
%(z^1^{\dagger})^{n_1}_\ast   \ast  \cdots \ast 
%(z^N^{\dagger})^{n_N}_\ast   \ast  
%(\partial_1 \Phi)^{n_1}_\ast   \ast  \cdots \ast 
%(\partial_N \Phi)^{n_N}_\ast   
%\label{3_16}
%\end{align}
%In this article, we use the following notation: for an $N$-tuple 
%$A_i ~(i=1, 2, \cdots, N)$ and an $N$-vector 
%$\vec{n}=(n_1, n_2, \cdots, n_N)$,
%\begin{align}
%(A)_\ast ^{\vec{n}} &= (A_1)_\ast ^{n_1} \ast  (A_2)_\ast ^{n_2} \ast  \cdots \ast 
% (A_N)_\ast ^{n_N}, \\ 
% \vec{n}! &= n_1! n_2! \cdots n_N!, \qquad
%  |n| = \sum_{i=1}^N n_i.
%\end{align}
%By using $(z)^{\vec{n}}_\ast  = (z)^{\vec{n}} = (z^1)^{n_1} \cdots (z^N)^{n_N}$, the above is recast as
%\begin{align}
%& \sum_{n_1, n_2, \dots, n_N=0}^\infty 
%\frac{1}{n_1 ! n_2 ! \cdots n_N! } 
%(-z^1)^{n_1} \cdots (-z^N)^{n_N} e^{-\frac{\Phi (z, \bar{z})}%
%{\hbar}}
% \partial_1^{n_1}  \cdots \partial_N^{n_N} 
%e^{\frac{\Phi (z, \bar{z})}{\hbar}} \notag \\
%&= \sum_{n=0}^{\infty}
%e^{-\frac{\Phi (z, \bar{z})}{\hbar}}
%\frac{1}{n!} \left( 
%-(z^1 \partial_1 + \cdots z^N \partial_N)
%\right)^n 
%e^{\frac{\Phi (z, \bar{z})}{\hbar}}
%\notag \\
%&= e^{-\frac{\Phi (z, \bar{z})}{\hbar}} e^{\frac{\Phi (0 , \bar{z})}{\hbar}}
%=  e^{-\frac{\Phi (z, \bar{z})}{\hbar}} . \label{3_17}
%\end{align}
%Here, the final equality follows from the condition (\ref{Phi_cond}).
%{} \hfill $\Box$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%From a similar calculation to the above proof, we can also show the
%following relations with respect to $a_i$ and $\underline{a}_i^\dagger$, 
%\begin{align}
% & |\vec{0} \rangle \langle \vec{0}| 
% = e^{-\Phi/\hbar} 
% = : e^{-\sum_i \underline{a}_i^\dagger a_i} :
% = {\prod_{i=1}^N}_\ast  \sum_{n=0}^{\infty} 
% \frac{(-1)^n}{n!} (\underline{a}_i^{\dagger})_\ast ^n \ast  (a_i)^n_\ast , 
% \label{vac-proj1} \\
% & a_i \ast  |\vec{0} \rangle \langle \vec{0}| = 0, \qquad
% |\vec{0} \rangle \langle \vec{0}| \ast  \underline{a}_i^\dagger = 0.
% \label{vac-proj2}
%\end{align}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma}[Sako, Suzuki, Umetsu \cite{Sako:2012ws}] \label{ssu}
%$e^{-\Phi/\hbar}=|0 \rangle \langle  0 |$ satisfies the relation 
%\begin{align}
%|0 \rangle \langle  0 |\ast  f(z, \bar{z}) 
% &= e^{-\Phi/\hbar} \ast  f(z, \bar{z}) 
% = e^{-\Phi/\hbar} f(0, \bar{z}) 
% = |0 \rangle \langle  0 | f(0, \bar{z}),
% \label{vacuum1} \\
% f(z, \bar{z})\ast |0 \rangle \langle  0 |
% &= f(z, \bar{z}) \ast  e^{-\Phi/\hbar} 
% = f(z, 0) e^{-\Phi/\hbar}
% = f(z, 0) |0 \rangle \langle  0 |.
%  \label{vacuum2}
%\end{align}
%for a function $f(z, \bar{z})$ such that $f(z, \bar{w})$ can be expanded
%as Taylor series with respect to $z^i$ and $\bar{w}^j$, respectively. 
%\end{lemma}
%A proof for this lemmama is given in \cite{Sako:2012ws}.
%, but for the convenience 
%its proof is reviewed here. 
%\begin{proof}
%To show the relation (\ref{vacuum1}), we note that the differential
%operator $R_{z^i}$ corresponding to the right product of $z^i$ contains
%only partial derivatives by $\bar{z}^j$, and thus commutes with
% $z^k$. Moreover, $R_{z^i}$ annihilates $e^{-\Phi/\hbar}$,
% $R_{z^i} e^{-\Phi/\hbar} = e^{-\Phi/\hbar} \ast  z^i
% = |\vec{0}\rangle \langle \vec{0} |\ast  a_i^\dagger=0 $ .
% From these and (\ref{Rf_Rz}), the relation (\ref{vacuum1})
%is shown as
%\begin{align}
% e^{-\Phi/\hbar} \ast  f(z, \bar{z}) &= R_f e^{-\Phi/\hbar} \nonumber \\
% &= \sum_{k_1, \dots, k_N=0}^\infty \frac{1}{k_1! \cdots k_N!}
% \partial_1^{k_1} \cdots \partial_N^{k_N} f(z, \bar{z})
% \prod_{i=1}^{N} \left(R_{z^i} - z^i \right)^{k_i} e^{-\Phi/\hbar}
% \nonumber \\
% &= \sum_{k_1, \dots, k_N=0}^\infty \frac{1}{k_1! \cdots k_N!}
% \partial_1^{k_1} \cdots \partial_N^{k_N} f(z, \bar{z})
% \prod_{i=1}^{N} \left(- z^i \right)^{k_i} e^{-\Phi/\hbar}
% \nonumber \\
% &= e^{-\Phi/\hbar} f(0, \bar{z}). \label{e-f}
%\end{align}
%Similarly, (\ref{vacuum2}) follows from (\ref{Lf_Lz}) and
% (\ref{vac-proj2}).
%
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{cor}
%\begin{equation}
%|0 \rangle \langle  0 |\ast  \partial_{\bar{i}} \Phi  =  
%\bar{z}^i \ast  |0 \rangle \langle  0 | =0 , \ \ {\mbox{for}} \ i=1,2 , \dots , N
% \label{vacuum}
%\end{equation}
%\end{cor}
%
%\begin{proof}
%$\Phi$は実で上のpropと(3.11)から
%
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Using some holomorphic function $P_{\alpha}$ and its complex conjugate
%$\bar{P}_{\alpha} (\bar{z} )$,
We expand a function 
$\exp \Phi(z, \bar{z})/\hbar$ as a power series,
\begin{align}
 e^{\Phi(z, \bar{z})/\hbar}
 = \sum_{\vec{m},\vec{n}} H_{\vec{m}, \vec{n}}
 (z)^{\vec{m}} (\bar{z})^{\vec{n}}%,
 \label{H}
\end{align}
%\begin{align}
%\exp \left( \frac{1}{\hbar} \Phi (z, \bar{z}) \right)&= 
%\sum_{\alpha}^N (z^{\alpha} \bar{P}_{\alpha} (\bar{z}) 
%+ \bar{z}^{\alpha} {P}_{\alpha} ({z}) ),
%\end{align}
%and we give the Taylor expansion of the holomorphic function $P_{\alpha}$ and 
%anti-holomorphic function $\bar{P}_{\alpha}$ as:
%\begin{align}
%P_{\alpha} ( z) = \sum_{\beta} C_{\alpha , \beta}(\hbar)   z^{\beta} , \
%\bar{P}_{\alpha} ( \bar{z}) = \sum_{\beta} \bar{C}_{\alpha , \beta}(\hbar)   
%\bar{z}^{\beta},
%\end{align}
where $(z)^{\vec{n}} = (z^1)^{n_1} \cdots (z^N)^{n_N}$ and $(\bar{z})^{\vec{n}} = (\bar{z}^1)^{n_1} \cdots (\bar{z}^N)^{n_N}$.
%We also use 
%\begin{align}
%P_{\alpha \ast } ( z) = \sum_{\beta} C_{\alpha , \beta}   (z)_\ast ^{\beta} , \
%\bar{P}_{\alpha \ast } ( \bar{z}) = \sum_{\beta} \bar{C}_{\alpha , \beta}  
%(\bar{z})_\ast ^{\beta},
%\end{align}
%where $z^{\alpha}_\ast  = (z^{1 })_\ast ^{\alpha_1} \ast  \cdots \ast  (z^N)_\ast ^{\alpha_N}$.
%But these are same as $P_{\alpha} ( z)$ and $\bar{P}_{\alpha} ( \bar{z})$
%because our star products are the star product with
%separation of variables.
%Since $\exp \Phi/\hbar$ is real and satisfies (\ref{Phi_cond}),
%the expansion coefficients $H_{\vec{m},\vec{n}}$ obey   
%\begin{align}
% \bar{H}_{\vec{m},\vec{n}} &= H_{\vec{n}, \vec{m}}, \\
% H_{\vec{0}, \vec{n}} &= H_{\vec{n}, \vec{0}}
% = \delta_{\vec{n}, \vec{0}}.
%\end{align}
%
%
%Using this expansion, the following relations are obtained. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{prop}
% The right $\ast $-multiplication of
% $ (\underline{a})_\ast ^{\vec{n}}=(\partial \Phi /\hbar )_\ast ^{\vec{n}} $
% on $|\vec{0} \rangle \langle \vec{0} |$ is
% related to the right $\ast $-multiplication of
% $(a)_\ast ^{\vec{n}} = (\bar{z})_\ast ^{\vec{n}}$ on
% $|\vec{0} \rangle \langle \vec{0}| $ as follows,
%\begin{align}
% |\vec{0} \rangle \langle  \vec{0} | \ast  (\underline{a})_\ast ^{\vec{n}}
% &= |\vec{0} \rangle \langle  \vec{0} |
% \ast  \left(\frac{1}{\hbar}\partial \Phi \right)_\ast ^{\vec{n}} \nonumber \\ 
% &= \vec{n}! \sum_{\vec{m}} H_{\vec{n}, \vec{m}}
% |\vec{0} \rangle \langle  \vec{0} | \ast  (\bar{z})_\ast ^{\vec{m}}
% = \vec{n}! \sum_{\vec{m}} H_{\vec{n}, \vec{m}}
% |\vec{0} \rangle \langle  \vec{0} | \ast  (a)_\ast ^{\vec{m}}.
% \label{vac-dPhi}
%\end{align}
% Similarly, the following relation holds,
% \begin{align}
%  (\underline{a}^\dagger)_\ast ^{\vec{n}}
%  \ast  |\vec{0} \rangle \langle  \vec{0} | 
%  &= \left(\frac{1}{\hbar}\bar{\partial} \Phi \right)_\ast ^{\vec{n}}
%  \ast  |\vec{0} \rangle \langle  \vec{0} |
%  \nonumber \\
%  &= \vec{n}! \sum_{\vec{m}} H_{\vec{m}, \vec{n}} (z)^{\vec{m}}
%  \ast  |\vec{0} \rangle \langle  \vec{0} |
%  = \vec{n}! \sum_{\vec{m}} H_{\vec{m}, \vec{n}}
%  (a^\dagger)_\ast ^{\vec{m}}
%  \ast  |\vec{0} \rangle \langle  \vec{0} |.
%  \label{dbarPhi-vac}
% \end{align}
%\end{prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The proof of this proposition is given in \cite{Sako:2016gqb}
%\begin{proof}
%By using (\ref{LdPhi}),
%\begin{align}
% |\vec{0} \rangle \langle \vec{0} |
%  \ast  \left(\frac{1}{\hbar}\partial \Phi \right)^{\vec{n}}_\ast %  
%&= |\vec{0} \rangle \langle  \vec{0} | \ast  
%\left( e^{-\Phi /\hbar } (\partial)^{\vec{n}} e^{\Phi /\hbar } \right)
%\notag \\
%&= |\vec{0} \rangle \langle \vec{0} | \ast  
% \left(e^{-\Phi /\hbar } \sum_{\vec{m}} \vec{n}!
% H_{\vec{n}, \vec{m}} (\bar{z})^{\vec{m}}
% + O(z)\right) .
%\end{align}
%From (\ref{vacuum1}) and lemmama \ref{lemma-1}, this is rewritten as
%\begin{align}
%\left.
% |\vec{0} \rangle \langle \vec{0} | \ast  
% \left(e^{-\Phi /\hbar } \sum_{\vec{m}} \vec{n}!
% H_{\vec{n}, \vec{m}} (\bar{z})^{\vec{m}}\right) 
%\right|_{(z,\bar{z})=(0, \bar{z})}
% &= |\vec{0} \rangle \langle \vec{0} | \ast 
% \sum_{\vec{m}} \vec{n}! H_{\vec{n}, \vec{m}} (\bar{z})^{\vec{m}}
% \nonumber \\
% &= |\vec{0} \rangle \langle \vec{0} | \ast 
% \sum_{\vec{m}} \vec{n}! H_{\vec{n}, \vec{m}} (a)_\ast ^{\vec{m}}.
%\end{align}
% The relation (\ref{dbarPhi-vac}) is the complex conjugation of
% (\ref{vac-dPhi}). 
%\end{proof}
%
%{}From this proposition,
%if there exists the inverse matrix $H^{-1}_{\vec{m}, \vec{n}}$, then the
%following relations also holds,
%%%%%%
%\begin{cor}
%\begin{align}
% |\vec{0} \rangle \langle \vec{0} | \ast   (a)_\ast ^{\vec{n}} 
%&= \sum_{\vec{m}} \frac{1}{\vec{m}!} H^{-1}_{\vec{n}, \vec{m}}
% |\vec{0} \rangle \langle \vec{0} | \ast  (\underline{a})_\ast ^{\vec{m}}, \\
%(a^\dagger)_\ast ^{\vec{n}} \ast   |\vec{0} \rangle \langle \vec{0} | 
%&= \sum_{\vec{m}} \frac{1}{\vec{m}!} H^{-1}_{\vec{m}, \vec{n}}
% (\underline{a}^\dagger)^{\vec{m}} \ast 
% |\vec{0} \rangle \langle \vec{0} |, 
%\end{align}
%where $H^{-1}_{\vec{n},\vec{m}}$ 
%is the inverse matrix of the matrix $H_{\vec{n}, \vec{m}}$,
% $\sum_{\vec{k}} H_{\vec{m}, \vec{k}} H^{-1}_{\vec{k}, \vec{n}}
% = \delta_{\vec{m}, \vec{n}}$.
%\end{cor}
%
%We introduce bases of the Fock representation as follows,
%\begin{equation}
% |\vec{m} \rangle \underline{\langle \vec{n}|}
% := \frac{1}{\sqrt{\vec{m}! \vec{n}!}}
% (a^\dagger)_\ast ^{\vec{m}} \ast  |\vec{0} \rangle \langle \vec{0}|
% \ast  (\underline{a})_\ast ^{\vec{n}}
% = \frac{1}{\sqrt{\vec{m}! \vec{n}!}}
% (z)_\ast ^{\vec{m}} \ast  e^{-\Phi/\hbar}
% \ast  \left(\frac{1}{\hbar} \partial \Phi\right)_\ast ^{\vec{n}}.
%\end{equation}
%By using (\ref{vac-dPhi}), the bases are also written as
%\begin{align}
% |\vec{m} \rangle \underline{\langle \vec{n}|}
% &= \sqrt{\frac{\vec{n}!}{\vec{m}!}} 
% \sum_{\vec{k}} H_{\vec{n}, \vec{k}} 
% (z)_\ast ^{\vec{m}} \ast  e^{-\Phi/\hbar} \ast  (\bar{z})_\ast ^{\vec{k}} 
% \nonumber \\
% &= \sqrt{\frac{\vec{n}!}{\vec{m}!}} 
% \sum_{\vec{k}} H_{\vec{n}, \vec{k}} 
% (z)^{\vec{m}} (\bar{z})^{\vec{k}} e^{-\Phi/\hbar}. \label{base_H_ver}
%\end{align} 
%The completeness of the bases are formally shown as
%\begin{align}
% \sum_{\vec{n}} |\vec{n} \rangle \underline{\langle \vec{n}|}
% = \sum_{\vec{m}, \vec{n}} H_{\vec{n}, \vec{m}} 
% (z)^{\vec{n}} (\bar{z})^{\vec{m}} e^{-\Phi/\hbar} 
% = e^{\Phi/\hbar} e^{-\Phi/\hbar} 
% = 1.
%\end{align}
%The bases are orthogonal to each other under the $\ast $-products, 
%\begin{align}
% |\vec{m} \rangle \underline{\langle \vec{n}|} \ast 
% |\vec{k} \rangle \underline{\langle \vec{l}|}
% &= \frac{1}{\sqrt{\vec{m}!\vec{n}!\vec{k}!\vec{l}!}}
% (a^\dagger)_\ast ^{\vec{m}} \ast  |\vec{0} \rangle \langle \vec{0}|
% \ast  (\underline{a})_\ast ^{\vec{n}} \ast 
%(a^\dagger)_\ast ^{\vec{k}} \ast  |\vec{0} \rangle \langle \vec{0}|
% \ast  (\underline{a})_\ast ^{\vec{l}} \nonumber \\
% &= \delta_{\vec{n}, \vec{k}}
% |\vec{m} \rangle \underline{\langle \vec{l}|}.
%\end{align}
%The behavior of the bases under the complex conjugation is different
%from usual, because the bra vectors are not Hermitian conjugate with the
%ket vectors in general, as noticed above,
%\begin{align}
% \overline{|\vec{m} \rangle \underline{\langle \vec{n}|}}
% &= \sqrt{\frac{\vec{n}!}{\vec{m}!}} \sum_{\vec{k}}
% H_{\vec{k}, \vec{n}} (z)^{\vec{k}} (\bar{z})^{\vec{m}} e^{-%
%\Phi/\hbar}
% \nonumber \\
% &= \sqrt{\frac{\vec{n}!}{\vec{m}!}} \sum_{\vec{k}, \vec{l}}
% \sqrt{\frac{\vec{k}!}{\vec{l}!}}
% H_{\vec{k}, \vec{n}} H^{-1}_{\vec{m}, \vec{l}}~
% |\vec{k} \rangle \underline{\langle \vec{l}|}.
%\end{align}
%
%
%
%
The creation and annihilation operators $a_i^\dagger, \underline{a}_i$
act on the bases as follows,
\begin{align}
 a_i^\dagger \ast  |\vec{m} \rangle \underline{\langle \vec{n}|}
 = \sqrt{m_i+1} 
 |\vec{m} + \vec{e}_i \rangle \underline{\langle \vec{n}|},% \\
 \qquad
 &
 \underline{a}_i \ast  |\vec{m} \rangle \underline{\langle \vec{n}|}
 = \sqrt{m_i} 
 |\vec{m} - \vec{e}_i \rangle \underline{\langle \vec{n}|}, \\
 |\vec{m} \rangle \underline{\langle \vec{n}|} \ast  a_i^\dagger 
 = \sqrt{n_i} 
 |\vec{m} \rangle \underline{\langle \vec{n} - \vec{e}_i|},% \\
 \qquad
 &
 |\vec{m} \rangle \underline{\langle \vec{n}|} \ast  \underline{a}_i
 = \sqrt{n_i+1} 
 |\vec{m} \rangle \underline{\langle \vec{n} + \vec{e}_i|}, 
\end{align}
where $\vec{e}_i$ is a unit vector, $(\vec{e}_i)_j = \delta_{ij}$.
The action of $a_i$ and $\underline{a}_i^\dagger$ is derived by the
Hermitian conjugation of the above equations.
%
%The creation and annihilation operators can be expanded with respect to
%the bases as
%\begin{align}
% a_i^\dagger &= \sum_{\vec{n}} \sqrt{n_i+1} 
% |\vec{n} + \vec{e}_i \rangle \underline{\langle \vec{n}|}, 
% \label{ca-op1} \\
% \underline{a}_i &= \sum_{\vec{n}} \sqrt{n_i+1}
% |\vec{n} \rangle \underline{\langle \vec{n} + \vec{e}_i|}, 
% \label{ca-op2} \\
% a_i &= \sum_{\vec{m}, \vec{n}, \vec{k}}
% \sqrt{\frac{\vec{m}!}{\vec{n}!}} H_{\vec{m}, \vec{k}}
% H^{-1}_{\vec{k} + \vec{e}_i, \vec{n}} 
% |\vec{m} \rangle \underline{\langle \vec{n}|}, \\
% \underline{a}_i^\dagger &=
% \sqrt{\frac{\vec{m}!}{\vec{n}!}} (k_i + 1) 
% H_{\vec{m}, \vec{k}+\vec{e}_i} H^{-1}_{\vec{k}, \vec{n}} 
% |\vec{m} \rangle \underline{\langle \vec{n}|}.
%\end{align}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The results of the twisted Fock representation of the
noncommutative K\"{a}hler manifolds are summarized as the 
dictionary in the Table \ref{table:result}:
%%%%% Dictionary
\begin{table}[H]
 \caption{Functions - Fock operators Dictionary }
 \label{table:result}
 \centering
 \begin{tabular}{c|c}
  \hline
  Functions & Fock operators  \\
  \hline \hline
  $\displaystyle e^{-\Phi/\hbar}$  &  $|\vec{0}\rangle \langle \vec{0}|$
      \\
  \hline
  $z_i $    &   $a_i^{\dagger}$ 
      \\ \hline
  $\displaystyle \frac{1}{\hbar}\partial_i \Phi$   &  $\underline{a}_i$
      \\ \hline
  $\bar{z}^i$   
  & $\displaystyle a_i = 
      \sum \sqrt{\frac{\vec{m}!}{\vec{n}!}} H_{\vec{m},\vec{k}}
      H^{-1}_{\vec{k}+\vec{e}_i , \vec{n}} 
      |\vec{m}\rangle \underline{\langle \vec{n} |} $ 
      \\ \hline
  $\displaystyle \frac{1}{\hbar} \partial_{\bar i} \Phi$ 
  & 
      $\displaystyle \underline{a}_i^{\dagger} = \sum 
      \sqrt{\frac{\vec{m}!}{\vec{n}!}}
      (k_i+1) H_{\vec{m},\vec{k}+\vec{e}_i}
      H^{-1}_{\vec{k} , \vec{n}} |\vec{m}\rangle 
      \underline{ \langle \vec{n} |} $
      \\
  \hline
 \end{tabular}
\end{table}
For physics, it is difficult to interpret formal power series. So this Fock representation is useful to construct physics theories like field theories on noncommutative K\"{a}hler manifolds. We will discuss this point in Section \ref{DQ_Discussion}.
%%ここまで
%%Berezinの結果については数式は入れずとも文章で説明する．特に，K\"{a}hlerの量子化を初めて試みた人物はBerezinであるので，その手の話については必ず述べる．背景については元論文を引用し，文章を変えて解説するつもりで．
%%Karabegovの結果およびFock representation on noncommutative K\"{a}hlerの話についてはopen bookにて出す予定だったものから引用．ただし文章は変える．

